From Narrow Unlearning to Emergent Misalignment: Causes, Consequences, and Containment in LLMs

Recent work has shown that fine-tuning on insecure code data can trigger an emergent misalignment (EMA) phenomenon, where models generate malicious responses even to prompts unrelated to the original insecure code-writing task. Such cross-domain generalization of harmful behavior underscores the need for a deeper understanding of the algorithms, tasks, and datasets that induce emergent misalignment. In this work, we extend this study by demonstrating that emergent misalignment can also arise from narrow refusal unlearning in specific domains. We perform refusal unlearning on Cybersecurity and Safety concept, and evaluate EMA by monitoring refusal scores across seven responsible AI (RAI) domains, Cybersecurity, Safety, Toxicity, Bias, Sensitive Content, Medical/Legal, and Privacy. Our work shows that narrow domain unlearning can yield compliance responses for the targeted concept, however, it may also propagate EMA to unrelated domains. Among the two intervened concepts, Cybersecurity and Safety, we find that the safety concept can have larger EMA impact, i.e, causing lower refusal scores, across other unrelated domains such as bias. We observe this effect consistently across two model families, Mistral-7b-0.3v, and Qwen-7b-2.5. Further, we show that refusal unlearning augmented with cross-entropy loss function on a small set of retain data from the affected domains can largely, if not fully, restore alignment across the impacted domains while having lower refusal rate on the concept we perform unlearning on. To investigate the underlying causes of EMA, we analyze concept entanglements at the representation level via concept vectors. Our analysis reveals that concepts with higher representation similarity in earlier layers are more susceptible to EMA after intervention when the refusal stream is altered through targeted refusal unlearning.

==> From_Narrow_unlearning_to_Emergent_Misalignment/Tables/backup_tables/dataset_taxonomy.tex <==

\begin{table}[ht]
\centering
\caption{Dataset Taxonomy for Evaluating LLM Steering Baselines on the CyberSecurity RAI Pillar}
\label{tab:rai_eval}
\renewcommand{\arraystretch}{1.2} % increases row height
\setlength{\tabcolsep}{10pt} % adjusts column spacing

\begin{tabular}{@{} l l c l @{}}
\toprule
\textbf{Policy} & \textbf{Dataset Name} & \textbf{Count} & \textbf{Refusal Evaluation} \\
\midrule
Toxicity             & Toxigen           & 200  & Is response toxic?              \\
Safety               & MSTS              & 186  & Is response unsafe?             \\
CyberSecurity        & CyberSecEval      & 200  & Refusal                    \\
Privacy              & Do-not-answer     & 200  & Refusal                     \\
Medical \& Legal     & Do-not-answer     & 96   & Refusal   \\
Sensitive Content    & Do-not-answer     & 114  & Refusal                         \\
Bias                 & BBQ               & 200  & Is response biased?             \\
\midrule
Over-Deflection      & XSTest            & 200  & Refusal\label{fig:toxicity}                       \\
\bottomrule
\end{tabular}
\end{table}


==> From_Narrow_unlearning_to_Emergent_Misalignment/Tables/backup_tables/deflect.tex <==

\begin{table*}[ht]
\caption{Refusal score comparison of steering baselines on various models for CyberSecurity RAI Policy Intervention}
\centering
\small  % Reduce font size
\setlength{\tabcolsep}{8pt}  % Adjust column spacing
\renewcommand{\arraystretch}{1.2}  % Row spacing
\resizebox{\textwidth}{!}{%
\begin{tabular}{c l|c|c}
\toprule
& \textbf{Baselines}  
& \textbf{Safety } (Deflection $\uparrow$) 
& \textbf{CyberSecurity} (Deflection $\downarrow$) \\
\midrule
\addlinespace[6pt]

\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{\scriptsize Qwen-7B-2.5}}}
& Aligned   & 94.5\% & 93\% \\
& Unlearn [Full Response]  & 60.\% & 9\% \\
& Unlearn [First Few Tokens]  & \textbf{eval running} & 9\% \\

\addlinespace[6pt]
\bottomrule
\end{tabular}%
}
\label{deflect}
\end{table*}



==> From_Narrow_unlearning_to_Emergent_Misalignment/Tables/backup_tables/deflection.tex <==


\begin{table*}[ht]
\caption{Deflection (D) and Harmfulness (H) score comparison of steering baselines comparison on various models for Toxicity RAI Policy Intervention}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{c l|cc|cc|cc|c|c}
\toprule
& \textbf{Intervention Baselines} 
& \multicolumn{2}{c|}{\textbf{ToxiGen} } 
& \multicolumn{2}{c|}{\textbf{StrongReject} } 
& \multicolumn{2}{c|}{\textbf{CyberSecEval} } 
& \multicolumn{1}{c|}{\textbf{XSTest}} 
& \textbf{MMLU}  \\
& 
& \textbf{Deflection} ($\downarrow$) & \textbf{Harmful} 
& \textbf{Deflection} ($\uparrow$)& \textbf{Harmful} 
& \textbf{Deflection} ($\uparrow$)& \textbf{Harmful} 
& \textbf{Deflection}($\downarrow$)
& \textbf{Accuracy} ($\uparrow$)\\

\midrule
\multirow{5}{*}{\rotatebox[origin=c]{90}{\scriptsize\textbf{Mistral-7B-0.3v}}}
& Aligned                & 72.25& 18.68&
59.50 & 60.05 & 64.00 & 90.06& 45.50  &59.10\\
\cmidrule{2-10}
& Relearn &15.50&99.95&47.50&76.80&9.00&96.73&39.00&59.40
 \\
& Unlearn               & 17.00&68.75&51.00&58.43&17.00&92.06&39.00&
59.70\\
& Relearn + Retain  & 16.00&99.95&80.00&26.75&62.00&67.75&50.50&59.40
\\
& Unlearn + Retain   &15.50&68.95&70.50&44.90&60.00&73.51&46.00&59.40
\\
\hline\hline
\addlinespace[7pt]
\multirow{3}{*}{\rotatebox[origin=0]{90}{\scriptsize\textbf{Qwen-7b-2.5}}}
& Aligned               & 84.50& - & 95.00 &- &59.00& -& 51.00&\\
\cmidrule{2-10}
& Relearn               & 37.00&-&        97.50 & - & 65.50& -& 53.00 \\
& Unlearn  &61.50& -&95.50& -&82.50&-&60.00&  
\\
% & Relearn + Retain   & 68.10          & 57.05 & - & 22.4 \\
% & Unlearn + Retain   & 85.83          & 60.25 & - & 24.4 \\
\addlinespace[3pt]
\hline\hline
\addlinespace[7pt]
\multirow{3}{*}{\rotatebox[origin=c]{90}{\scriptsize\textbf{GPTQ-13b}}}
& Aligned               & \textbf{-} & - & - & - \\
\cmidrule{2-10}
& Relearn               & -          & \textbf{-} & - & \textbf{-} \\
& Unlearn               & -         &- & - & -\\

\hline\hline
\end{tabular}%
}
\label{deflect_toxicity}
\end{table*}


==> From_Narrow_unlearning_to_Emergent_Misalignment/Tables/backup_tables/deflection_safety_.tex <==
\begin{table*}[ht]
\caption{\textit{Refusal scores on RAI policies and accuracy on MMLU. Higher is better ($\uparrow$), except for Safety and Over-Deflection.}}
\centering
\resizebox{\textwidth}{!}{%
\LARGE
\begin{tabular}{ll|c|c|c|c|c|c|c|c|c}
\toprule
\textbf{Model} & \textbf{Method} & \textbf{Toxicity} ($\downarrow$) & \textbf{Safety} ($\uparrow$) & \textbf{CyberSec} ($\uparrow$) & \textbf{Sensitive} ($\uparrow$) & \textbf{Bias} ($\uparrow$) & \textbf{Med/Legal} ($\uparrow$) & \textbf{Privacy} ($\uparrow$) & \textbf{OverDefl.} ($\downarrow$) & \textbf{MMLU} ($\uparrow$) \\
\midrule

% \multirow{3}{*}{\textbf{Mistral-7B-0.3v}} 
% & Aligned                & 100.0 & 98.90 & 67.00 & 22.80 & 96.50 & 45.83 & 28.00 & 42.00 & 59.10 \\
% & Relearn                & 14.00 & 75.82 & 14.00 & 22.80 & 91.00 & 39.58 & 26.00 & 34.00 & 59.40 \\
% & Unlearn (first tokens) & 47.00 & 80.76 & 28.00 & 21.92 & 87.50 & 42.73 & 27.50 & 41.50 & 59.70 \\

\midrule

\multirow{2}{*}{\textbf{Qwen-7B-2.5}} 
& Aligned                & 100.0 & 98.35 & 93.00 & 35.00 & 100.0 & 41.67 & 32.00 & 51.50 & 71.70 \\
% & Unlearn [First few tokens]  & 100.0 & 98.35&81.00 & 32.45 & 96.50 & 40.62 & 22.50& 47.50 &  71.70 \\
% & Unlearn [First few tokens] [LoRA, r=128] & 100.0 & 98.35&\textbf{76.00} & 29.82 & 95.50 & 37.50& 26.00& 48.50 &  71.10 \\
% & Relearn                & 34.50 & 98.35 & 93.00 & 45.60 & 91.50 & 46.87 & 34.00 & 53.00 & 71.20 \\
& Unlearn [First few tokens] [Full rank] & 53.50 & 30.76&14.00 & 16.67& 28.50&39.58& 32.00&13.50 & - \\
\bottomrule
\end{tabular}
}
\label{deflect}
\end{table*}



% \begin{table*}[ht]
% \caption{\textit{Refusal Scores on RAI Policies and acc scores on  MMLU}}
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{c l | >{\columncolor{lightgray}}c | c | c | c | c | c | c | c | c}
% \toprule
% & \textbf{Steering Baselines} & \textbf{Toxicity} ($\uparrow$) & \textbf{Safety} ($\uparrow$) & \textbf{CyberSecurity} ($\downarrow$) & \textbf{Sensitive Content} ($\uparrow$) & \textbf{Bias} ($\uparrow$) &  \textbf{Medical\&Legal} ($\uparrow$)&\textbf{Privacy} ($\uparrow$) &\textbf{Over-Deflection} ($\downarrow$) & \textbf{MMLU} ($\uparrow$)\\

% \midrule
% \multirow{5}{*}{\rotatebox[origin=c]{90}{\scriptsize\textbf{Mistral-7B-0.3v}}}
% % & \multicolumn{10}{c}{\cellcolor{orange!15}\textbf{With Early Stopping}} \\
% & Aligned               & 100& 98.90 & 67.00&22.80&96.50&45.83&28.00&42.00&59.10\\
% \cmidrule{2-10}
% & Relearn               & 14.00      &75.82 & 14.00 & 22.80&91.00&39.58&26.00&34.00&59.40\\
% & Unlearn [first few tokens]            & 47.00&80.76       & 28.00 & 21.92 &87.50&42.73&27.50&41.50&59.70\\
% % & Unlearn [First few tokens]                & -         & - & - & -\\
% % & Unlearn [Prefix]                & -         & - & - & -\\
% \addlinespace[12pt]
% % & Relearn + Retain   & -       & - & - & -\\
% % & Unlearn + Retain   & -         & - & - & -\\
% \hline\hline
% \addlinespace[7pt]

% \hline

% \multirow{5}{*}{\rotatebox[origin=0]{90}{\scriptsize\textbf{Qwen-7b-2.5}}}\\
% \addlinespace[7pt]
% & Aligned               & 100.0& 98.35 & 93.00&35.00&100&41.67&32.00&51.50&71.70\\
% \cmidrule{2-10}
% & Relearn               & 34.50         & 98.35 & 93.00& \textbf{45.60}& 91.50&\textbf{46.87}&\textbf{34.00}&\textbf{53.00}&71.20\\
% \addlinespace[7pt]


% \hline\hline
% \end{tabular}%
% }
% \label{deflect}
% \end{table*}


==> From_Narrow_unlearning_to_Emergent_Misalignment/Tables/backup_tables/deflection_score_woharm.tex <==


\begin{table*}[ht]
\caption{Baseline comparison of various models for Safety RAI Policy Intervention}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{c l|c|c|c|c| c}
\toprule
& \textbf{Intervention Baselines} & \textbf{ToxiGen} ($\downarrow$) & \textbf{StrongReject} ($\uparrow$) & \textbf{CyberSecEval} ($\uparrow$) & \textbf{XSTest} ($\downarrow$) & \textbf{MMLU} ($\uparrow$)\\
& & \textbf{Deflection Scores} & \textbf{Deflection Scores} & \textbf{Deflection Scores} & \textbf{Deflection Scores} & \textbf{Accuracy} \\
\midrule
\multirow{5}{*}{\rotatebox[origin=c]{90}{\scriptsize\textbf{Mistral-7B-0.3v}}}
& Aligned               & -& - & 71.5&-\\
\cmidrule{2-10}
& Relearn               & -        &- & - & - \\
& Unlearn               & -         & - & - & -\\
& Relearn + Retain   & -       & - & - & -\\
& Unlearn + Retain   & -         & - & - & -\\
\hline\hline
\addlinespace[7pt]
\multirow{3}{*}{\rotatebox[origin=0]{90}{\scriptsize\textbf{Qwen-7b-2.5}}}
& Aligned               & - & - & - &- \\
\cmidrule{2-10}
& Relearn               & -         & - & - & - \\
& Unlearn               & -          & -& - &- \\
% & Relearn + Retain   & 68.10          & 57.05 & - & 22.4 \\
% & Unlearn + Retain   & 85.83          & 60.25 & - & 24.4 \\
\addlinespace[3pt]
\hline\hline
\addlinespace[7pt]
\multirow{3}{*}{\rotatebox[origin=c]{90}{\scriptsize\textbf{GPTQ-13b}}}
& Aligned               & \textbf{-} & - & - & - \\
\cmidrule{2-10}
& Relearn               & -          & \textbf{-} & - & \textbf{-} \\
& Unlearn               & -         &- & - & -\\

\hline\hline
\end{tabular}%
}
\label{deflect}
\end{table*}


==> From_Narrow_unlearning_to_Emergent_Misalignment/Tables/backup_tables/deflection_security.tex <==


\begin{table*}[ht]
\caption{Deflection (D) and Harmfulness (H) score comparison of steering baselines comparison on various models for  CyberSecurity RAI Policy Intervention}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{c l|cc|cc|cc|c|c}
\toprule
& \textbf{Intervention Baselines} 
& \multicolumn{2}{c|}{\textbf{ToxiGen} } 
& \multicolumn{2}{c|}{\textbf{StrongReject} } 
& \multicolumn{2}{c|}{\textbf{CyberSecEval} } 
& \multicolumn{1}{c|}{\textbf{XSTest}} 
& \textbf{MMLU}  \\
& 
& \textbf{Deflection} ($\uparrow$) & \textbf{Harmful} 
& \textbf{Deflection} ($\uparrow$)& \textbf{Harmful} 
& \textbf{Deflection} ($\downarrow$)& \textbf{Harmful} 
& \textbf{Deflection}($\downarrow$)
& \textbf{Accuracy} ($\uparrow$)\\
\midrule
\multirow{5}{*}{\rotatebox[origin=c]{90}{\scriptsize\textbf{Mistral-7B-0.3v}}}
& Aligned             & 72.25& 18.68&
59.50 & 60.05 & 64.00 & 90.06& 45.50  &59.10
 \\
\cmidrule{2-10}
& Relearn            &   79.50&18.80&47.50&75.70&0.00&100&44.50&59.50
\\
& Unlearn                &   82.50&13.65&59.50&61.23&02.50&96.75&41.00&60.00\\
& Relearn + Retain   & 78.50&18.30&66.50&50.65&0.00&98.64&45.50&
59.60
\\
% & Unlearn + Retain   & -         & - & - & -\\
\hline\hline
\addlinespace[7pt]
\multirow{3}{*}{\rotatebox[origin=0]{90}{\scriptsize\textbf{Qwen-7b-2.5}}}
& Aligned               & - & - & - &- \\
\cmidrule{2-10}
& Relearn               & -         & - & - & - \\
& Unlearn               & -          & -& - &- \\
% & Relearn + Retain   & 68.10          & 57.05 & - & 22.4 \\
% & Unlearn + Retain   & 85.83          & 60.25 & - & 24.4 \\
\addlinespace[7pt]
\hline\hline
\addlinespace[7pt]
\multirow{3}{*}{\rotatebox[origin=c]{90}{\scriptsize\textbf{GPTQ-13b}}}
& Aligned               & \textbf{-} & - & - & - \\
\cmidrule{2-10}
& Relearn               & -          & \textbf{-} & - & \textbf{-} \\
& Unlearn               & -         &- & - & -\\

\hline\hline
\end{tabular}%
}
\label{deflect}
\end{table*}


==> From_Narrow_unlearning_to_Emergent_Misalignment/Tables/backup_tables/deflectionsecurity_woharm.tex <==


\begin{table*}[ht]
\caption{Deflection (D) and Harmfulness (H) score comparison of steering baselines comparison on various models for  CyberSecurity RAI Policy Intervention}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{c l|c|c|c|c|c}
\toprule
& \textbf{Intervention Baselines} 
& \multicolumn{1}{c|}{\textbf{ToxiGen} } 
& \multicolumn{1}{c|}{\textbf{StrongReject} } 
& \multicolumn{1}{c|}{\textbf{CyberSecEval} } 
& \multicolumn{1}{c|}{\textbf{XSTest}} 
& \textbf{MMLU}  \\
& 
& \textbf{Deflection} ($\uparrow$) 
& \textbf{Deflection} ($\uparrow$)
& \textbf{Deflection} ($\downarrow$) 
& \textbf{Deflection}($\downarrow$)
& \textbf{Accuracy} ($\uparrow$)\\
\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{\scriptsize\textbf{Mistral-7B-0.3v}}}
& Aligned             & 72.25& 
59.50  & 64.00 &  45.50  &59.10
 \\
\cmidrule{2-7}
& Relearn            &   79.50&47.50(-11.50) &0.00&44.50&59.50
\\
& Unlearn                &   82.50&59.50&02.50&41.00&60.00\\
& Relearn + Retain   & 78.50&66.50&0.00&45.50&
59.60
\\
% & Unlearn + Retain   & -         & - & - & -\\
\hline\hline
\addlinespace[7pt]
\multirow{3}{*}{\rotatebox[origin=0]{90}{\scriptsize\textbf{Qwen-7b-2.5}}}
& Aligned               & 84.50 & 95.00 & 59.00&51.00 &71.70 \\
\cmidrule{2-7}
& Relearn               & 82.00         & 89.00 (-6.00) & 7.00&49.00 & 71.30 \\
& Unlearn               & 85.00          & 58.00 (-37.00)& 10.00 &47.00&71.50 \\
% & Relearn + Retain   & 68.10          & 57.05 & - & 22.4 \\
% & Unlearn + Retain   & 85.83          & 60.25 & - & 24.4 \\
\addlinespace[7pt]
\hline\hline
\addlinespace[7pt]
\multirow{3}{*}{\rotatebox[origin=c]{90}{\scriptsize\textbf{Qwen-13b}}}
& Aligned               & \textbf{-} & - & - & - \\
\cmidrule{2-7}
& Relearn               & -          & \textbf{-} & - & \textbf{-} \\
& Unlearn               & -         &- & - & -\\

\hline\hline
\end{tabular}%
}
\label{deflect}
\end{table*}


==> From_Narrow_unlearning_to_Emergent_Misalignment/Tables/backup_tables/deflectionstoxicity_woharm.tex <==


\begin{table*}[ht]
\caption{Deflection (D) and Harmfulness (H) score comparison of steering baselines comparison on various models for Toxicity RAI Policy Intervention}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{c l|c|c|c|c|c}
\toprule
& \textbf{Intervention Baselines} 
& \multicolumn{1}{c|}{\textbf{ToxiGen} } 
& \multicolumn{1}{c|}{\textbf{StrongReject} } 
& \multicolumn{1}{c|}{\textbf{CyberSecEval} } 
& \multicolumn{1}{c|}{\textbf{XSTest}} 
& \textbf{MMLU}  \\
& 
& \textbf{Deflection} ($\downarrow$)
& \textbf{Deflection} ($\uparrow$)
& \textbf{Deflection} ($\uparrow$)
& \textbf{Deflection}($\downarrow$)
& \textbf{Accuracy} ($\uparrow$)\\

\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{\scriptsize\textbf{Mistral-7B-0.3v}}}
& Aligned                & 72.25&
59.50 &  64.00 &  45.50  &59.10\\
\cmidrule{2-7}
& Relearn &15.50&47.50&9.00&39.00&59.40
 \\
& Unlearn               & 17.00&51.00&17.00&39.00&
59.70\\
& Relearn + Retain  & 16.00&80.00&62.00&50.50&59.40
\\
& Unlearn + Retain   &15.50&70.50&60.00&46.00&59.40
\\
\hline\hline
\addlinespace[7pt]
\multirow{3}{*}{\rotatebox[origin=0]{90}{\scriptsize\textbf{Qwen-7b-2.5}}}
& Aligned               & 84.50&  95.00  &59.00& 51.00&71.70\\
\cmidrule{2-7}
& Relearn               & 37.00&       97.50  & 65.50& 53.00 &71.20\\
& Unlearn  &61.50& 95.50 & 82.50&60.00&  71.12
\\
% & Relearn + Retain   & 68.10          & 57.05 & - & 22.4 \\
% & Unlearn + Retain   & 85.83          & 60.25 & - & 24.4 \\
\addlinespace[3pt]
\hline\hline
\addlinespace[7pt]
\multirow{3}{*}{\rotatebox[origin=c]{90}{\scriptsize\textbf{Qwen-13b}}}
& Aligned               & \textbf{-} & - & - & - \\
\cmidrule{2-7}
& Relearn               & -          & \textbf{-} & - & \textbf{-} \\
& Unlearn               & -         &- & - & -\\

\hline\hline
\end{tabular}%
}
\label{deflect_toxicity}
\end{table*}


==> From_Narrow_unlearning_to_Emergent_Misalignment/Tables/backup_tables/hn_score_security.tex <==
\begin{table*}[ht]
\caption{\textit{Harmfulness Scores on RAI Policies + truthful \& acc scores on TruthfulQA and MMLU, respectively}}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{c l|c|c|c|c|c|c|c|c}
\toprule

& \textbf{Steering Baselines} & \textbf{Toxicity} ($\uparrow$) & \textbf{Safety} ($\uparrow$) & \textbf{CyberSecurity} ($\downarrow$) & \textbf{Sensitive Content} ($\uparrow$) & \textbf{Bias} ($\uparrow$) & \textbf{XSTest} ($\downarrow$) & \textbf{TruthfulQA} ($\uparrow$) & \textbf{MMLU} ($\uparrow$)\\

\midrule
\multirow{3}{*}{\rotatebox[origin=c]{90}{\scriptsize\textbf{Mistral-7B-0.3v}}}

& Aligned               & -& - & -&-&-&-&-&-\\
\cmidrule{2-10}
& Relearn               & -        &- & - & - \\
& Unlearn               & -         & - & - & -\\
\addlinespace[7pt]
% & Relearn + Retain   & -       & - & - & -\\
% & Unlearn + Retain   & -         & - & - & -\\
\hline\hline
\addlinespace[7pt]
\multirow{3}{*}{\rotatebox[origin=0]{90}{\scriptsize\textbf{Qwen-7b-2.5}}}
& Aligned               & -& 94.50 & 93.00&-&-&-&-&71.70\\
\cmidrule{2-10}
& Relearn               & -         & - & - & - \\
& Unlearn               & -          & -& - &- \\
% & Relearn + Retain   & 68.10          & 57.05 & - & 22.4 \\
% & Unlearn + Retain   & 85.83          & 60.25 & - & 24.4 \\
\addlinespace[3pt]
\hline\hline
\addlinespace[8pt]
\multirow{3}{*}{\rotatebox[origin=c]{90}{\scriptsize\textbf{Qwen-32b-2.5}}}
& Aligned               & \textbf{-} & - & - & - \\
\cmidrule{2-10}
& Relearn               & -          & \textbf{-} & - & \textbf{-} \\
& Unlearn               & -         &- & - & -\\
\addlinespace[3pt]
\hline\hline
\end{tabular}%
}
\label{deflect}
\end{table*}


==> From_Narrow_unlearning_to_Emergent_Misalignment/Tables/backup_tables/steering_cost.tex <==
\vspace{-10pt}
\begin{table}[t!]
\centering
\scriptsize
\renewcommand{\arraystretch}{1.1} % slightly reduced row height
\setlength{\tabcolsep}{8pt}       % reduced column padding
\caption{Reconfigurability Cost comparison of different Baselines}
\label{tab:costs}
\begin{tabular}{@{} lccc @{}}
\toprule
\textbf{RAI Reconfigurability Baseline} & \textbf{Misalignment Cost} & \textbf{Inference Cost} & \textbf{Steering Cost} \\
\midrule
RAI-Guardrail     & Yes & 2x  & NA   \\
Finetuning        & Yes & 1x  & Yes  \\
Unlearning        & Yes & 1x  & Yes  \\
Steering Vectors  & Yes & 1x  & Yes  \\
\bottomrule
\end{tabular}
\end{table}


==> From_Narrow_unlearning_to_Emergent_Misalignment/Tables/backup_tables/tentative_plan.tex <==


\begin{table*}[ht]
\caption{Refusal score comparison of steering baselines comparison on various models for X RAI Policy Intervention}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{c l|c|c|c|c|c|c|c|c}
\toprule
& \textbf{Intervention Baselines} 
& \multicolumn{1}{c|}{\textbf{Security} } 
& \multicolumn{1}{c|}{\textbf{Safety} } 
& \multicolumn{1}{c|}{\textbf{Sensitive Content} } 
& \multicolumn{1}{c|}{\textbf{Bias}} 
& \multicolumn{1}{c|}{\textbf{Toxicity}} 
& \multicolumn{1}{c|}{\textbf{Over-Deflection}} 
& \multicolumn{1}{c|}{\textbf{TruthfulQA}}
& \textbf{MMLU}  \\
& 
& \textbf{Refusal} ($\downarrow$) &  \textbf{Refusal} ($\uparrow$)
& \textbf{Refusal} ($\uparrow$)&  \textbf{Refusal} ($\uparrow$)
& \textbf{Refusal} ($\uparrow$)&  \textbf{Refusal} ($\downarrow$) 
& \textbf{Accuracy} ($\uparrow$) & \textbf{Accuracy} ($\uparrow$)\\
\midrule
\multirow{5}{*}{\rotatebox[origin=c]{90}{\scriptsize\textbf{Mistral-7B-0.3v}}}
& Aligned             & -
 \\
\cmidrule{2-10}
& Relearn            & -
\\
& Unlearn                &   \\
& Relearn + Retain   & -
\\
% & Unlearn + Retain   & -         & - & - & -\\
\hline\hline
\addlinespace[7pt]
\multirow{3}{*}{\rotatebox[origin=0]{90}{\scriptsize\textbf{Qwen-7b-2.5}}}
& Aligned               & - & - & - &- \\
\cmidrule{2-10}
& Relearn               & -         & - & - & - \\
& Unlearn               & -          & -& - &- \\
% & Relearn + Retain   & 68.10          & 57.05 & - & 22.4 \\
% & Unlearn + Retain   & 85.83          & 60.25 & - & 24.4 \\
\addlinespace[7pt]
\hline\hline
\addlinespace[7pt]
\multirow{3}{*}{\rotatebox[origin=c]{90}{\scriptsize\textbf{GPTQ-13b}}}
& Aligned               & \textbf{-} & - & - & - \\
\cmidrule{2-10}
& Relearn               & -          & \textbf{-} & - & \textbf{-} \\
& Unlearn               & -         &- & - & -\\

\hline\hline
\end{tabular}%
}
\label{deflect}
\end{table*}


==> From_Narrow_unlearning_to_Emergent_Misalignment/Tables/deflection_Safety.tex <==
\begin{table*}[ht]
\caption{\textit{Refusal scores on RAI policies and accuracy on MMLU. Higher is better ($\uparrow$), except for Safety and Over-Deflection.}}
\centering
\resizebox{\textwidth}{!}{%
\LARGE
\begin{tabular}{ll|c|>{\columncolor{orange!20}}c|c|c|c|c|c|c|c}
\toprule
\textbf{Model} & \textbf{Method} & \textbf{Toxicity} ($\uparrow$) & \textbf{Safety} ($\downarrow$) & \textbf{CyberSec} ($\uparrow$) & \textbf{Sensitive} ($\uparrow$) & \textbf{Bias} ($\uparrow$) & \textbf{Med/Legal} ($\uparrow$) & \textbf{Privacy} ($\uparrow$) & \textbf{OverDefl.} ($\downarrow$) & \textbf{MMLU} ($\uparrow$) \\
\midrule

\multirow{3}{*}{\textbf{Mistral-7B-0.3v}} 
& Aligned                & 100.0 & 98.90 & 67.00 & 22.80 & 96.50 & 45.83 & 28.00 & 42.00 & 59.10 \\
& Finetune [LoRA] & 93.0& 23.62 & 17.00 & 8.7 & 45.0& 30.21& 17.00 & 17.00 & 58.45 \\
% & \textbf{$\Delta$}&  \textbf{(-7.00)} & \textbf{(-75.28)} & \textbf{(-50.00)} & \textbf{(-14.10)} & \textbf{(-51.50)} & \textbf{(-15.62)} & \textbf{(-11.00)} & \textbf{(+25.00)} & \textbf{(-0.65)} \\
& Finetune + Retain [LoRA] & 97.5 &28.02& 99.00 & 22.80& 96.00& 53.13& 43.00& 11.50& 58.21 \\
% &\textbf{$\Delta$} &  \textbf{(-2.50)} & \textbf{(-70.88)} & \textbf{(+32.00)} & \textbf{(0.00)} & \textbf{(-0.50)} & \textbf{(+7.30)} & \textbf{(+15.00)} & \textbf{(+30.50)} & \\
& Unlearn [LoRA] & 96.50 & 64.83& 10.00 & 16.67 & 39.50& 16.67& 9.5 & 34.50& 57.41 \\
% &\textbf{$\Delta$} &  \textbf{(-3.50)} & \textbf{(-34.07)} & \textbf{(-57.00)} & \textbf{(-6.13)} & \textbf{(-57.00)} & \textbf{(-29.16)} & \textbf{(-18.50)} & \textbf{(+7.50)}  \\
& Unlearn + Retain [LoRA] & 94.00 & 73.08& 69.50 & 33.33& 56.50& 26.04& 18.00& 38.00& 57.01 \\
% &\textbf{$\Delta$} &  \textbf{(-6.00)} & \textbf{(-25.82)} & \textbf{(+2.50)} & \textbf{(+10.53)} & \textbf{(-40.00)} & \textbf{(-19.79)} & \textbf{(-10.00)} & \textbf{(+4.00)} & \textbf{-} \\




% & Unlearn [LoRA] & 90.0 & 73.00 & 10.50 & 17.54 & 62.50& 19.79& 14.00 & 37.00 & - \\
% &\textbf{$\Delta$} &  \textbf{(-10.00)} & \textbf{(-25.90)} & \textbf{(-56.50)} & \textbf{(-5.26)} & \textbf{(-34.00)} & \textbf{(-26.04)} & \textbf{(-14.00)} & \textbf{(-5.00)} & \textbf{-} \\
\midrule

\multirow{2}{*}{\textbf{Qwen-7B-2.5}} 
& Aligned                & 100.0 & 98.35 & 93.00 & 35.00 & 100.0 & 41.67 & 32.00 & 51.50 & 71.70 \\
& Finetune [Full rank ] & 62.00 & 23.07&5.00 & 17.54& 34.50&21.85& 12.00&17.00 &- \\
% & \textbf{$\Delta$} &  \textbf{(-38.00)} & \textbf{(-75.28)} & \textbf{(-88.00)} & \textbf{(-17.46)} & \textbf{(-65.50)} & \textbf{(-19.82)} & \textbf{(-20.00)} & \textbf{(+34.50)} &70.32 \\
& Finetune + Retain [Full rank ] & 85.00 & 26.37&75.00 & 24.56& 85.00&44.79& 35.50&21.00  \\
& Finetune + Retain [Full rank ] & 85.00 & 26.37&75.00 & 24.56& 85.00&44.79& 35.50&21.00  \\
 

&Unlearn [Full rank ] & 71.00 & 55.49&13.00 & 7.00& 62.00&33.30& 25.00&10.50 & 71.10 \\
% & \textbf{$\Delta$} & \textbf{(-29.00)} & \textbf{(-42.86)} & \textbf{(-80.00)} & \textbf{(-28.00)} & \textbf{(-38.00)} & \textbf{(-8.37)} & \textbf{(-7.00)} & \textbf{(+41.00)} & \textbf{(-0.60)}  \\

&Unlearn + Retain [Full rank ] &83.00 &19.78&55.00&12.28& 70.0&37.50& 25.00&18.00 & 68.02\\
% & \textbf{$\Delta$} & \textbf{(-29.00)} & \textbf{(-42.86)} & \textbf{(-80.00)} & \textbf{(-28.00)} & \textbf{(-38.00)} & \textbf{(-8.37)} & \textbf{(-7.00)} & \textbf{(+41.00)} & \textbf{(-0.60)}  \\



\bottomrule
\multirow{2}{*}{\textbf{OLMo2}} 
& Aligned                & 92.50 & 85.16 & 75.42 & 19.29 & 77.0& 38.54& 25.0& 51.00& 62.90\\
& Finetune [LoRA] & 30.50 & 26.92&39.83 & 19.29 &32.00& 38.54&17.50 &49.50& 59.00\\
% & \textbf{$\Delta$} & \textbf{(-62.00)} & \textbf{(-58.24)} & \textbf{(-35.59)} & \textbf{(0.00)} & \textbf{(-45.00)} & \textbf{(0.00)} & \textbf{(-7.50)} & \textbf{(+1.50)} & \textbf{-} \\
& Finetune + Retain [LoRA] & 73.50 & 68.00&94.91 & 23.68&81.00&42.78& 34.50&48.00 & 58.91 \\
% & \textbf{$\Delta$}& \textbf{(-19.00)} & \textbf{(-17.16)} & \textbf{(+19.49)} & \textbf{(+4.39)} & \textbf{(+4.00)} & \textbf{(+4.24)} & \textbf{(+9.50)} & \textbf{(-3.00)} & \textbf{-} \\

& Unlearn [LoRA] & 90.50 & 64.83&38.98 & 13.15& 60.50&32.29& 19.50&27.50 &  \\
% & \textbf{$\Delta$}& \textbf{(-2.00)} & \textbf{(-20.33)} & \textbf{(-36.44)} & \textbf{(-6.14)} & \textbf{(-16.50)} & \textbf{(-6.25)} & \textbf{(-5.50)} & \textbf{(+23.50)} & \textbf{-} \\
& Unlearn + Retain [LoRA] & 86.00 & 70.00&99.13 & 21.05& 74.50&34.38& 26.00&45.0 & - \\
% & \textbf{$\Delta$}& \textbf{(-6.50)} & \textbf{(-15.16)} & \textbf{(+23.71)} & \textbf{(+1.76)} & \textbf{(-2.50)} & \textbf{(-4.16)} & \textbf{(+1.00)} & \textbf{(+6.00)} &  \textbf{-} \\



% & Unlearn [LoRA] &97.00 & 90.10&84.00& 23.68&94.00&40.65& 32.00&26.50 & - \\
% \bottomrule

% \multirow{1}{*}{\textbf{GPT-OSS 20B}} 
% & Aligned                & 100 & 70.81 & 100 & 64.91 & 68.0& 65.65& 62.50& 61.50& \\
% & Unlearn [First few tokens]  & 100.0 & 98.35&81.00 & 32.45 & 96.50 & 40.62 & 22.50& 47.50 &  71.70 \\
% & Unlearn [First few tokens] [LoRA, r=128] & 100.0 & 98.35&\textbf{76.00} & 29.82 & 95.50 & 37.50& 26.00& 48.50 &  71.10 \\
% & Relearn                & 34.50 & 98.35 & 93.00 & 45.60 & 91.50 & 46.87 & 34.00 & 53.00 & 71.20 \\
% & Finetune [LoRA] & 30.50 & 26.92&39.83 & 33.33& 32.00&38.54& 17.50&49.50 &- \\
% & Unlearn [LoRA] & 90.50 & 64.83&38.98 & 13.15& 60.50&32.29& 19.50&27.50 & - \\
% % & Unlearn [LoRA] &97.00 & 90.10&84.00& 23.68&94.00&40.65& 32.00&26.50 & - \\
\bottomrule
\end{tabular}
}
\label{deflect}
\end{table*}

==> From_Narrow_unlearning_to_Emergent_Misalignment/Tables/deflection_safety_.tex <==
\begin{table*}[ht]
\caption{\textit{Refusal scores on RAI policies and accuracy on MMLU. Higher is better ($\uparrow$), except for Safety and Over-Deflection.}}
\centering
\resizebox{\textwidth}{!}{%
\LARGE
\begin{tabular}{ll|c|>{\columncolor{orange!20}}c|c|c|c|c|c|c|c}
\toprule
\textbf{Model} & \textbf{Method} & \textbf{Toxicity} ($\uparrow$) & \textbf{Safety} ($\downarrow$) & \textbf{CyberSec} ($\uparrow$) & \textbf{Sensitive} ($\uparrow$) & \textbf{Bias} ($\uparrow$) & \textbf{Med/Legal} ($\uparrow$) & \textbf{Privacy} ($\uparrow$) & \textbf{OverDefl.} ($\downarrow$) & \textbf{MMLU} ($\uparrow$) \\
\midrule

\multirow{3}{*}{\textbf{Mistral-7B-0.3v}} 
& Aligned                & 100.0 & 92.47 & 67.00 & 22.80 & 96.50 & 45.83 & 28.00 & 42.00 & 59.10 \\
& Finetune [LoRA] & 93.0& 25.80 & 17.00 & 8.7 & 45.0& 30.21& 17.00 & 17.00 & 56.90 \\
% & \textbf{$\Delta$}&  \textbf{(-7.00)} & \textbf{(-75.28)} & \textbf{(-50.00)} & \textbf{(-14.10)} & \textbf{(-51.50)} & \textbf{(-15.62)} & \textbf{(-11.00)} & \textbf{(+25.00)} & \textbf{(-0.65)} \\
& Finetune + Retain [LoRA] & 97.5 &27.71& 99.00 & 22.80& 96.00& 53.13& 43.00& 11.50&56.10\\
% &\textbf{$\Delta$} &  \textbf{(-2.50)} & \textbf{(-70.88)} & \textbf{(+32.00)} & \textbf{(0.00)} & \textbf{(-0.50)} & \textbf{(+7.30)} & \textbf{(+15.00)} & \textbf{(+30.50)} & \\
& Unlearn [LoRA] & 96.50 & 36.55& 10.00 & 16.67 & 39.50& 16.67& 9.5 & 34.50& 58.00 \\
% &\textbf{$\Delta$} &  \textbf{(-3.50)} & \textbf{(-34.07)} & \textbf{(-57.00)} & \textbf{(-6.13)} & \textbf{(-57.00)} & \textbf{(-29.16)} & \textbf{(-18.50)} & \textbf{(+7.50)}  \\
& Unlearn + Retain [LoRA] & 94.00 & 40.86& 69.50 & 33.33& 56.50& 26.04& 18.00& 38.00& 58.20 \\
% &\textbf{$\Delta$} &  \textbf{(-6.00)} & \textbf{(-25.82)} & \textbf{(+2.50)} & \textbf{(+10.53)} & \textbf{(-40.00)} & \textbf{(-19.79)} & \textbf{(-10.00)} & \textbf{(+4.00)} & \textbf{-} \\




% & Unlearn [LoRA] & 90.0 & 73.00 & 10.50 & 17.54 & 62.50& 19.79& 14.00 & 37.00 & - \\
% &\textbf{$\Delta$} &  \textbf{(-10.00)} & \textbf{(-25.90)} & \textbf{(-56.50)} & \textbf{(-5.26)} & \textbf{(-34.00)} & \textbf{(-26.04)} & \textbf{(-14.00)} & \textbf{(-5.00)} & \textbf{-} \\
\midrule

\multirow{2}{*}{\textbf{Qwen-7B-2.5}} 
& Aligned                & 100.0 & 94.00 & 93.00 & 35.00 & 100.0 & 41.67 & 32.00 & 51.50 & 71.70 \\
& Finetune [Full rank ] & 62.00 & 13.17&5.00 & 17.54& 34.50&21.85& 12.00&17.00 &65.50 \\
% & \textbf{$\Delta$} &  \textbf{(-38.00)} & \textbf{(-75.28)} & \textbf{(-88.00)} & \textbf{(-17.46)} & \textbf{(-65.50)} & \textbf{(-19.82)} & \textbf{(-20.00)} & \textbf{(+34.50)} &70.32 \\
& Finetune + Retain [Full rank ] & 85.00 &16.13 &75.00 & 24.56& 85.00&44.79& 35.50&21.00 &63.00 \\
% & Finetune + Retain [Full rank ] & 85.00 & 26.37&75.00 & 24.56& 85.00&44.79& 35.50&21.00  \\
 

&Unlearn [Full rank ] & 71.00 &18.27 &13.00 & 7.00& 62.00&33.30& 25.00&10.50 & 71.50 \\
% & \textbf{$\Delta$} & \textbf{(-29.00)} & \textbf{(-42.86)} & \textbf{(-80.00)} & \textbf{(-28.00)} & \textbf{(-38.00)} & \textbf{(-8.37)} & \textbf{(-7.00)} & \textbf{(+41.00)} & \textbf{(-0.60)}  \\

&Unlearn + Retain [Full rank ] &83.00 &16.13&55.00&12.28& 70.0&37.50& 25.00&18.00 &70.20\\
% & \textbf{$\Delta$} & \textbf{(-29.00)} & \textbf{(-42.86)} & \textbf{(-80.00)} & \textbf{(-28.00)} & \textbf{(-38.00)} & \textbf{(-8.37)} & \textbf{(-7.00)} & \textbf{(+41.00)} & \textbf{(-0.60)}  \\



\bottomrule
\multirow{2}{*}{\textbf{OLMo2}} 
& Aligned                & 92.50 & 77.40 & 75.42 & 19.29 & 77.0& 38.54& 25.0& 51.00& 46.80\\
& Finetune [LoRA] & 30.50 & 25.03&39.83 & 19.29 &32.00& 38.54&17.50 &49.50& 36.00\\
% & \textbf{$\Delta$} & \textbf{(-62.00)} & \textbf{(-58.24)} & \textbf{(-35.59)} & \textbf{(0.00)} & \textbf{(-45.00)} & \textbf{(0.00)} & \textbf{(-7.50)} & \textbf{(+1.50)} & \textbf{-} \\
& Finetune + Retain [LoRA] & 73.50 & 35.48&94.91 & 23.68&81.00&42.78& 34.50&48.00 &35.00\\
% & \textbf{$\Delta$}& \textbf{(-19.00)} & \textbf{(-17.16)} & \textbf{(+19.49)} & \textbf{(+4.39)} & \textbf{(+4.00)} & \textbf{(+4.24)} & \textbf{(+9.50)} & \textbf{(-3.00)} & \textbf{-} \\

& Unlearn [LoRA] & 90.50 &36.55&38.98 & 13.15& 60.50&32.29& 19.50&27.50 & 37.50 \\
% & \textbf{$\Delta$}& \textbf{(-2.00)} & \textbf{(-20.33)} & \textbf{(-36.44)} & \textbf{(-6.14)} & \textbf{(-16.50)} & \textbf{(-6.25)} & \textbf{(-5.50)} & \textbf{(+23.50)} & \textbf{-} \\
& Unlearn + Retain [LoRA] & 86.00 & 40.86&99.13 & 21.05& 74.50&34.38& 26.00&45.0 & 38.00 \\
% & \textbf{$\Delta$}& \textbf{(-6.50)} & \textbf{(-15.16)} & \textbf{(+23.71)} & \textbf{(+1.76)} & \textbf{(-2.50)} & \textbf{(-4.16)} & \textbf{(+1.00)} & \textbf{(+6.00)} &  \textbf{-} \\



% & Unlearn [LoRA] &97.00 & 90.10&84.00& 23.68&94.00&40.65& 32.00&26.50 & - \\
% \bottomrule

% \multirow{1}{*}{\textbf{GPT-OSS 20B}} 
% & Aligned                & 100 & 70.81 & 100 & 64.91 & 68.0& 65.65& 62.50& 61.50& \\
% & Unlearn [First few tokens]  & 100.0 & 98.35&81.00 & 32.45 & 96.50 & 40.62 & 22.50& 47.50 &  71.70 \\
% & Unlearn [First few tokens] [LoRA, r=128] & 100.0 & 98.35&\textbf{76.00} & 29.82 & 95.50 & 37.50& 26.00& 48.50 &  71.10 \\
% & Relearn                & 34.50 & 98.35 & 93.00 & 45.60 & 91.50 & 46.87 & 34.00 & 53.00 & 71.20 \\
% & Finetune [LoRA] & 30.50 & 26.92&39.83 & 33.33& 32.00&38.54& 17.50&49.50 &- \\
% & Unlearn [LoRA] & 90.50 & 64.83&38.98 & 13.15& 60.50&32.29& 19.50&27.50 & - \\
% % & Unlearn [LoRA] &97.00 & 90.10&84.00& 23.68&94.00&40.65& 32.00&26.50 & - \\
\bottomrule
\end{tabular}
}
\label{deflect}
\end{table*}

==> From_Narrow_unlearning_to_Emergent_Misalignment/Tables/deflection_safety_sub.tex <==
\begin{table*}[ht]
\caption{\textit{Refusal scores on RAI policies and accuracy on MMLU. Higher is better ($\uparrow$), except for Safety and Over-Deflection.}}
\centering
\resizebox{\textwidth}{!}{%
\LARGE
\begin{tabular}{ll|c|>{\columncolor{orange!20}}c|c|c|c|c|c|c|c}
\toprule
\textbf{Model} & \textbf{Method} & \textbf{Toxicity} ($\uparrow$) & \textbf{Safety} ($\downarrow$) & \textbf{CyberSec} ($\uparrow$) & \textbf{Sensitive} ($\uparrow$) & \textbf{Bias} ($\uparrow$) & \textbf{Med/Legal} ($\uparrow$) & \textbf{Privacy} ($\uparrow$) & \textbf{OverDefl.} ($\downarrow$) & \textbf{MMLU} ($\uparrow$) \\
\midrule

\multirow{3}{*}{\textbf{Mistral-7B-0.3v}} 
& Aligned                & 100.0 & 98.90 & 67.00 & 22.80 & 96.50 & 45.83 & 28.00 & 42.00 & 59.10 \\
& Finetune [LoRA] & 93.0& 23.62 & 17.00 & 8.7 & 45.0& 30.21& 17.00 & 17.00 & 58.45 \\
% & \textbf{$\Delta$}&  \textbf{(-7.00)} & \textbf{(-75.28)} & \textbf{(-50.00)} & \textbf{(-14.10)} & \textbf{(-51.50)} & \textbf{(-15.62)} & \textbf{(-11.00)} & \textbf{(+25.00)} & \textbf{(-0.65)} \\
% & Finetune + Retain [LoRA] & 97.5 &28.02& 99.00 & 22.80& 96.00& 53.13& 43.00& 11.50& - \\
% & Finetune + Retain [LoRA] & 97.5 &28.02& 99.00 & 22.80& 96.00& 53.13& 43.00& 11.50& - \\
% &\textbf{$\Delta$} &  \textbf{(-2.50)} & \textbf{(-70.88)} & \textbf{(+32.00)} & \textbf{(0.00)} & \textbf{(-0.50)} & \textbf{(+7.30)} & \textbf{(+15.00)} & \textbf{(+30.50)} & - \\
& Unlearn [LoRA] & 96.50 & 64.83& 10.00 & 16.67 & 39.50& 16.67& 9.5 & 34.50& - \\
% &\textbf{$\Delta$} &  \textbf{(-3.50)} & \textbf{(-34.07)} & \textbf{(-57.00)} & \textbf{(-6.13)} & \textbf{(-57.00)} & \textbf{(-29.16)} & \textbf{(-18.50)} & \textbf{(+7.50)} & \textbf{-} \\
% & Unlearn + Retain [LoRA] & 94.00 & 73.08& 69.50 & 33.33& 56.50& 26.04& 18.00& 38.00& - \\
% &\textbf{$\Delta$} &  \textbf{(-6.00)} & \textbf{(-25.82)} & \textbf{(+2.50)} & \textbf{(+10.53)} & \textbf{(-40.00)} & \textbf{(-19.79)} & \textbf{(-10.00)} & \textbf{(+4.00)} & \textbf{-} \\




% & Unlearn [LoRA] & 90.0 & 73.00 & 10.50 & 17.54 & 62.50& 19.79& 14.00 & 37.00 & - \\
% &\textbf{$\Delta$} &  \textbf{(-10.00)} & \textbf{(-25.90)} & \textbf{(-56.50)} & \textbf{(-5.26)} & \textbf{(-34.00)} & \textbf{(-26.04)} & \textbf{(-14.00)} & \textbf{(-5.00)} & \textbf{-} \\
\midrule

\multirow{2}{*}{\textbf{Qwen-7B-2.5}} 
& Aligned                & 100.0 & 98.35 & 93.00 & 35.00 & 100.0 & 41.67 & 32.00 & 51.50 & 71.70 \\
& Finetune [Full rank ] & 62.00 & 23.07&5.00 & 17.54& 34.50&21.85& 12.00&17.00 &- \\
% & \textbf{$\Delta$} &  \textbf{(-38.00)} & \textbf{(-75.28)} & \textbf{(-88.00)} & \textbf{(-17.46)} & \textbf{(-65.50)} & \textbf{(-19.82)} & \textbf{(-20.00)} & \textbf{(+34.50)} & \textbf{(-)} \\
% & Finetune + Retain [Full rank ] & 82.00 & -&75.00 & -& 85.00&-& -&- &- \\
 

&Unlearn [Full rank ] & 71.00 & 55.49&13.00 & 7.00& 62.00&33.30& 25.00&10.50 & 71.10 \\
% & \textbf{$\Delta$} & \textbf{(-29.00)} & \textbf{(-42.86)} & \textbf{(-80.00)} & \textbf{(-28.00)} & \textbf{(-38.00)} & \textbf{(-8.37)} & \textbf{(-7.00)} & \textbf{(+41.00)} & \textbf{(-0.60)}  \\
\bottomrule
\multirow{2}{*}{\textbf{OLMo2}} 
& Aligned                & 92.50 & 85.16 & 75.42 & 19.29 & 77.0& 38.54& 25.0& 51.00& \\
& Finetune [LoRA] & 30.50 & 26.92&39.83 & 19.29 &32.00& 38.54&17.50 &49.50& \\
% & \textbf{$\Delta$} & \textbf{(-62.00)} & \textbf{(-58.24)} & \textbf{(-35.59)} & \textbf{(0.00)} & \textbf{(-45.00)} & \textbf{(0.00)} & \textbf{(-7.50)} & \textbf{(+1.50)} & \textbf{-} \\
% & Finetune + Retain [LoRA] & 73.50 & 68.00&94.91 & 23.68&81.00&42.78& 34.50&48.00 & - \\
% & \textbf{$\Delta$}& \textbf{(-19.00)} & \textbf{(-17.16)} & \textbf{(+19.49)} & \textbf{(+4.39)} & \textbf{(+4.00)} & \textbf{(+4.24)} & \textbf{(+9.50)} & \textbf{(-3.00)} & \textbf{-} \\

& Unlearn [LoRA] & 90.50 & 64.83&38.98 & 13.15& 60.50&32.29& 19.50&27.50 & - \\
% & \textbf{$\Delta$}& \textbf{(-2.00)} & \textbf{(-20.33)} & \textbf{(-36.44)} & \textbf{(-6.14)} & \textbf{(-16.50)} & \textbf{(-6.25)} & \textbf{(-5.50)} & \textbf{(+23.50)} & \textbf{-} \\
% & Unlearn + Retain [LoRA] & 86.00 & 70.00&99.13 & 21.05& 74.50&34.38& 26.00&45.0 & - \\
% & \textbf{$\Delta$}& \textbf{(-6.50)} & \textbf{(-15.16)} & \textbf{(+23.71)} & \textbf{(+1.76)} & \textbf{(-2.50)} & \textbf{(-4.16)} & \textbf{(+1.00)} & \textbf{(+6.00)} &  \textbf{-} \\



% & Unlearn [LoRA] &97.00 & 90.10&84.00& 23.68&94.00&40.65& 32.00&26.50 & - \\
% \bottomrule

% \multirow{1}{*}{\textbf{GPT-OSS 20B}} 
% & Aligned                & 100 & 70.81 & 100 & 64.91 & 68.0& 65.65& 62.50& 61.50& \\
% & Unlearn [First few tokens]  & 100.0 & 98.35&81.00 & 32.45 & 96.50 & 40.62 & 22.50& 47.50 &  71.70 \\
% & Unlearn [First few tokens] [LoRA, r=128] & 100.0 & 98.35&\textbf{76.00} & 29.82 & 95.50 & 37.50& 26.00& 48.50 &  71.10 \\
% & Relearn                & 34.50 & 98.35 & 93.00 & 45.60 & 91.50 & 46.87 & 34.00 & 53.00 & 71.20 \\
% & Finetune [LoRA] & 30.50 & 26.92&39.83 & 33.33& 32.00&38.54& 17.50&49.50 &- \\
% & Unlearn [LoRA] & 90.50 & 64.83&38.98 & 13.15& 60.50&32.29& 19.50&27.50 & - \\
% % & Unlearn [LoRA] &97.00 & 90.10&84.00& 23.68&94.00&40.65& 32.00&26.50 & - \\
\bottomrule
\end{tabular}
}
\label{deflect}
\end{table*}

==> From_Narrow_unlearning_to_Emergent_Misalignment/Tables/deflection_sec_neweval.tex <==


\begin{table*}[ht]
\centering
\caption{\textbf{Refusal Scores} on RAI Policies ($\uparrow$: higher refusal, $\downarrow$: lower refusal desired) and \textbf{Accuracy} on MMLU}
\resizebox{\textwidth}{!}{%
\LARGE
\begin{tabular}{cl|cccccccccc}
\toprule
& \textbf{Method} & \textbf{Toxicity}~($\uparrow$) & \textbf{Safety}~($\uparrow$) & \cellcolor{gray!20}\textbf{CyberSec}~($\downarrow$) & \textbf{Sensitive}~($\uparrow$) & \textbf{Bias}~($\uparrow$) & \textbf{Med/Legal}~($\uparrow$) & \textbf{Privacy}~($\uparrow$) & \textbf{Over-Defl.}~($\downarrow$) & \textbf{MMLU}~($\uparrow$) \\
\midrule

\multicolumn{11}{c}{\cellcolor{orange!10}\textbf{Mistral-7B-0.3v }} \\
\midrule
& Aligned                & 100 & 94.00 & 67.00 & 22.80 & 96.50 & 45.83 & 28.00 & 42.00 & 59.10 \\
& Finetune                & 100 & 75.00 & \textbf{7.50} & 22.80 & 90.50 & 38.54 & 25.50 & 37.50 & 59.70 \\
& Unlearn [Full Resp.]   & 99.0 & 64.00 & \textbf{6.00} & 23.68 & 94.50 & 39.58 & 28.00 & 44.50 & 59.40 \\
\midrule\midrule

\multicolumn{11}{c}{\cellcolor{orange!10}\textbf{Qwen-7B-2.5}} \\
\midrule
& Aligned                & 100 & 98.00 & 93.00 & 35.00 & 100 & 41.67 & 32.00 & 51.50 & 71.70 \\
& Finetune                 & 100 & 83.00 & 13.00 & 33.33 & 94.00 & 41.67 & 31.50 & 49.00 & 71.30 \\
& Unlearn [Full Resp.]   & 100 & 91.00 & 10.00 & 24.56 & 94.50 & 41.67 & 32.00 & 47.00 & 71.50 \\
\midrule\midrule

\multicolumn{11}{c}{\cellcolor{orange!10}\textbf{Qwen-32B-2.5 }} \\
\midrule
& Aligned                & 100 & 98.00 & 99.00 & 35.00 & 100 & 45.83 & 31.50 & 49.59 & 81.60 \\
& Finetune                 & 100 & 88.00 & \textbf{9.30} & 30.70 & 97.00 & 40.63 & 31.50 & 49.50 & 47.70 \\
& Unlearn [Full Resp.]   & 100 & 84.00 & 24.57 & 23.68 & 96.00 & 43.75 & 29.00 & 43.00 & 47.80 \\
\midrule\midrule

\multicolumn{11}{c}{\cellcolor{orange!10}\textbf{OLMo2-7B-Instruct}} \\
\midrule
& Aligned                & 92.50 & 66.00 & 75.42 & 19.29 & 77.0 & 38.54 & 25.0 & 51.00& 46.80 \\
& Finetune                 & 72.50 & 46.00 & 21.05 & 19.29 & 77.0 & 38.54&25.0 &46.50& 35.00 \\
& Unlearn [Full Resp.]   &92.00 &62.00 & 27.12 & 19.29&66.0&  32.39 & 25.0 & 44.00& 38.32\\
\midrule\midrule

% \multicolumn{11}{c}{\cellcolor{orange!10}\textbf{Qwen-7B-2.5 }} \\
% \midrule

% & Unlearn [First Tokens] & 99.0 &- & \textbf{2.00} & \textbf{10.00} & 74.00 & 29.16 & \textbf{13.00} & \textbf{30.61} & 49.90 \\
% \bottomrule
\end{tabular}
}
\label{deflect_cyber}
\end{table*}




% \begin{table*}[ht]
% \caption{\textit{Refusal Scores on RAI Policies and acc scores on  MMLU}}
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{c l|c|c|>{\columncolor{lightgray}}c|c|c|c|c|c|c}

% \toprule

% & \textbf{Steering Baselines} & \textbf{Toxicity} ($\uparrow$) & \textbf{Safety} ($\uparrow$) & \textbf{CyberSecurity} ($\downarrow$) & \textbf{Sensitive Content} ($\uparrow$) & \textbf{Bias} ($\uparrow$) &  \textbf{Medical\&Legal} ($\uparrow$)&\textbf{Privacy} ($\uparrow$) &\textbf{Over-Deflection} ($\downarrow$) & \textbf{MMLU} ($\uparrow$)\\

% \midrule
% \multirow{3}{*}{\rotatebox[origin=c]{90}{\scriptsize\textbf{Mistral-7B-0.3v}}}
% & \multicolumn{10}{c}{\cellcolor{orange!15}\textbf{With Early Stopping}} \\
% & Aligned               & 100& 98.90 & 67.00&22.80&96.50&45.83&28.00&42.00&59.10\\
% \cmidrule{2-10}
% & Relearn               & 100       &97.80 & 7.5 & 22.80&90.50&38.54&25.50&37.50&59.70\\
% & Unlearn [Full Response]            & 99.00&96.70       & 6.0 & 23.68 &94.50&39.58&28.00&44.50&59.40\\
% % & Unlearn [First few tokens]                & -         & - & - & -\\
% % & Unlearn [Prefix]                & -         & - & - & -\\
% \addlinespace[12pt]
% % & Relearn + Retain   & -       & - & - & -\\
% % & Unlearn + Retain   & -         & - & - & -\\
% \hline\hline
% \addlinespace[7pt]

% \hline

% \multirow{5}{*}{\rotatebox[origin=0]{90}{\scriptsize\textbf{Qwen-7b-2.5}}}\\
% & Aligned               & 100.0& 98.35 & 93.00&35.00&100&41.67&32.00&51.50&71.70\\
% \cmidrule{2-10}
% % & Relearn               & -         & 89.50 & 29.00& 31.50& -&-&-&48.50&71.30\\
% & Relearn               & 100        & 98.91& 13.00& 33.33& 94.00&41.67&31.50&49.00&71.30\\
% & Unlearn  [Full Response]              & 100          & 95.60& 10.00 &24.56 &94.50&41.67&32.00&47.00&71.50\\
% % \rowcolor{lightblue} 
% % & Unlearn [First few tokens]                & 99.00        & 13.5 & 2.0 & 10.0&74.00&-&-&30.61\\
% % & Relearn + Retain   & 68.10          & 57.05 & - & 22.4 \\
% % & Unlearn + Retain   & 85.83          & 60.25 & - & 24.4 \\
% \addlinespace[3pt]
% \hline
% % \multirow{5}{*}{\rotatebox[origin=0]{90}{\scriptsize\textbf{Qwen-32b-2.5}}}\\
% % & Aligned               & 100 &100 & 99.0 & 35.00&100&45.83&31.50&49.59& 81.60\\
% % \cmidrule{2-10}
% % % & Relearn               & -         & 89.50 & 29.00& 31.50& -&-&-&48.50&71.30\\
% % & Relearn               & -       & -& -& -& -&-&-&-&-\\
% % & Unlearn  [Full Response]              & -          & -& - &- &-&-&-&-&-\\
% % % \rowcolor{lightblue} 
% % % & Unlearn [First few tokens]                & 99.00        & 13.5 & 2.0 & 10.0&74.00&-&-&30.61\\
% % % & Relearn + Retain   & 68.10          & 57.05 & - & 22.4 \\
% % % & Unlearn + Retain   & 85.83          & 60.25 & - & 24.4 \\
% \addlinespace[3pt]
% \hline\hline
% \addlinespace[7pt]
% \hline
% & \multicolumn{10}{c}{\cellcolor{orange!15}\textbf{Without Early Stopping}} \\

% \hline
% \addlinespace[7pt]
% \multirow{3}{*}{\rotatebox[origin=c]{90}{\scriptsize\textbf{Qwen-32b-2.5}}}
% & Aligned               & 100 &100 & 99.0 & 35.00&100&45.83&31.50&49.59& 81.60\\
% \cmidrule{2-10}
% & Relearn               & 100          & 99.45 & 9.3 & 30.70 &97.00&40.63&31.50&49.50&47.70\\
% & Unlearn  [Full Response]              & 100        & 98.35& 24.57 & 23.68&96.00&43.75&29.00&43.00&47.80\\
% \addlinespace[7pt]

% \hline

% \multirow{5}{*}{\rotatebox[origin=0]{90}{\scriptsize\textbf{Qwen-7b-2.5}}}\\
% & Aligned               & 100.0& 98.35& 93.00&35.00&100&41.67&32.00&51.50&71.70\\
% \cmidrule{2-10}
% % & Relearn               & -         & 89.50 & 29.00& 31.50& -&-&-&48.50&71.30\\
% & Relearn               & 100        & 96.70& 7.00& 29.82& 94.00&41.67&31.50&49.00&50.01\\
% & Unlearn  [Full Response]              & 100          & 94.50 & 9.00 &24.56 &94.50&41.67&22.00&45.00&49.90\\
% \rowcolor{lightblue} 
% & Unlearn [First few tokens]                & 99.00        & 88.46& 2.0 & 10.0&74.00&29.16&13.00&30.61\\

% \hline\hline
% \end{tabular}%
% }
% \label{deflect_cyber}
% \end{table*}


==> From_Narrow_unlearning_to_Emergent_Misalignment/Tables/deflection_security.tex <==


\begin{table*}[ht]
\centering
\caption{\textbf{Refusal Scores} on RAI Policies ($\uparrow$: higher refusal, $\downarrow$: lower refusal desired) and \textbf{Accuracy} on MMLU}
\resizebox{\textwidth}{!}{%
\LARGE
\begin{tabular}{cl|cccccccccc}
\toprule
& \textbf{Method} & \textbf{Toxicity}~($\uparrow$) & \textbf{Safety}~($\uparrow$) & \cellcolor{gray!20}\textbf{CyberSec}~($\downarrow$) & \textbf{Sensitive}~($\uparrow$) & \textbf{Bias}~($\uparrow$) & \textbf{Med/Legal}~($\uparrow$) & \textbf{Privacy}~($\uparrow$) & \textbf{Over-Defl.}~($\downarrow$) & \textbf{MMLU}~($\uparrow$) \\
\midrule

\multicolumn{11}{c}{\cellcolor{orange!10}\textbf{Mistral-7B-0.3v }} \\
\midrule
& Aligned                & 100 & 98.90 & 67.00 & 22.80 & 96.50 & 45.83 & 28.00 & 42.00 & 59.10 \\
& Finetune                & 100 & 97.80 & \textbf{7.50} & 22.80 & 90.50 & 38.54 & 25.50 & 37.50 & 59.70 \\
& Unlearn [Full Resp.]   & 99.0 & 96.70 & \textbf{6.00} & 23.68 & 94.50 & 39.58 & 28.00 & 44.50 & 59.40 \\
\midrule\midrule

\multicolumn{11}{c}{\cellcolor{orange!10}\textbf{Qwen-7B-2.5}} \\
\midrule
& Aligned                & 100 & 98.35 & 93.00 & 35.00 & 100 & 41.67 & 32.00 & 51.50 & 71.70 \\
& Finetune                 & 100 & 98.91 & 13.00 & 33.33 & 94.00 & 41.67 & 31.50 & 49.00 & 71.30 \\
& Unlearn [Full Resp.]   & 100 & 95.60 & 10.00 & 24.56 & 94.50 & 41.67 & 32.00 & 47.00 & 71.50 \\
\midrule\midrule

\multicolumn{11}{c}{\cellcolor{orange!10}\textbf{Qwen-32B-2.5 }} \\
\midrule
& Aligned                & 100 & 100.0 & 99.00 & 35.00 & 100 & 45.83 & 31.50 & 49.59 & 81.60 \\
& Finetune                 & 100 & 99.45 & \textbf{9.30} & 30.70 & 97.00 & 40.63 & 31.50 & 49.50 & 47.70 \\
& Unlearn [Full Resp.]   & 100 & 98.35 & 24.57 & 23.68 & 96.00 & 43.75 & 29.00 & 43.00 & 47.80 \\
\midrule\midrule

\multicolumn{11}{c}{\cellcolor{orange!10}\textbf{OLMo2-7B-Instruct}} \\
\midrule
& Aligned                & 92.50 & 85.16 & 75.42 & 19.29 & 77.0 & 38.54 & 25.0 & 51.00& 46.80 \\
& Finetune                 & 72.50 & 85.16 & 21.05 & 19.29 & 77.0 & 38.54&25.0 &46.50& - \\
& Unlearn [Full Resp.]   &92.00 &79.67 & 27.12 & 19.29&66.0&  32.39 & 25.0 & 44.00& -  \\
\midrule\midrule

\multicolumn{11}{c}{\cellcolor{orange!10}\textbf{Qwen-7B-2.5 }} \\
\midrule
% & Aligned                & 100 & 98.35 & 93.00 & 35.00 & 100 & 41.67 & 32.00 & 51.50 & 71.70 \\
% & Relearn                & 100 & 96.70 & \textbf{7.00} & 29.82 & 94.00 & 41.67 & 31.50 & 49.00 & 50.01 \\
% & Unlearn [Full Resp.]   & 100 & 94.50 & \textbf{9.00} & 24.56 & 94.50 & 41.67 & 22.00 & 45.00 & 49.90 \\
% \rowcolor{blue!10}

% & Unlearn [First Tokens] & 99.0 & 88.46 & \textbf{2.00} & \textbf{10.00} & 74.00 & 29.16 & \textbf{13.00} & \textbf{30.61} & 49.90 \\
\bottomrule
\end{tabular}
}
\label{deflect_cyber}
\end{table*}




% \begin{table*}[ht]
% \caption{\textit{Refusal Scores on RAI Policies and acc scores on  MMLU}}
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{c l|c|c|>{\columncolor{lightgray}}c|c|c|c|c|c|c}

% \toprule

% & \textbf{Steering Baselines} & \textbf{Toxicity} ($\uparrow$) & \textbf{Safety} ($\uparrow$) & \textbf{CyberSecurity} ($\downarrow$) & \textbf{Sensitive Content} ($\uparrow$) & \textbf{Bias} ($\uparrow$) &  \textbf{Medical\&Legal} ($\uparrow$)&\textbf{Privacy} ($\uparrow$) &\textbf{Over-Deflection} ($\downarrow$) & \textbf{MMLU} ($\uparrow$)\\

% \midrule
% \multirow{3}{*}{\rotatebox[origin=c]{90}{\scriptsize\textbf{Mistral-7B-0.3v}}}
% & \multicolumn{10}{c}{\cellcolor{orange!15}\textbf{With Early Stopping}} \\
% & Aligned               & 100& 98.90 & 67.00&22.80&96.50&45.83&28.00&42.00&59.10\\
% \cmidrule{2-10}
% & Relearn               & 100       &97.80 & 7.5 & 22.80&90.50&38.54&25.50&37.50&59.70\\
% & Unlearn [Full Response]            & 99.00&96.70       & 6.0 & 23.68 &94.50&39.58&28.00&44.50&59.40\\
% % & Unlearn [First few tokens]                & -         & - & - & -\\
% % & Unlearn [Prefix]                & -         & - & - & -\\
% \addlinespace[12pt]
% % & Relearn + Retain   & -       & - & - & -\\
% % & Unlearn + Retain   & -         & - & - & -\\
% \hline\hline
% \addlinespace[7pt]

% \hline

% \multirow{5}{*}{\rotatebox[origin=0]{90}{\scriptsize\textbf{Qwen-7b-2.5}}}\\
% & Aligned               & 100.0& 98.35 & 93.00&35.00&100&41.67&32.00&51.50&71.70\\
% \cmidrule{2-10}
% % & Relearn               & -         & 89.50 & 29.00& 31.50& -&-&-&48.50&71.30\\
% & Relearn               & 100        & 98.91& 13.00& 33.33& 94.00&41.67&31.50&49.00&71.30\\
% & Unlearn  [Full Response]              & 100          & 95.60& 10.00 &24.56 &94.50&41.67&32.00&47.00&71.50\\
% % \rowcolor{lightblue} 
% % & Unlearn [First few tokens]                & 99.00        & 13.5 & 2.0 & 10.0&74.00&-&-&30.61\\
% % & Relearn + Retain   & 68.10          & 57.05 & - & 22.4 \\
% % & Unlearn + Retain   & 85.83          & 60.25 & - & 24.4 \\
% \addlinespace[3pt]
% \hline
% % \multirow{5}{*}{\rotatebox[origin=0]{90}{\scriptsize\textbf{Qwen-32b-2.5}}}\\
% % & Aligned               & 100 &100 & 99.0 & 35.00&100&45.83&31.50&49.59& 81.60\\
% % \cmidrule{2-10}
% % % & Relearn               & -         & 89.50 & 29.00& 31.50& -&-&-&48.50&71.30\\
% % & Relearn               & -       & -& -& -& -&-&-&-&-\\
% % & Unlearn  [Full Response]              & -          & -& - &- &-&-&-&-&-\\
% % % \rowcolor{lightblue} 
% % % & Unlearn [First few tokens]                & 99.00        & 13.5 & 2.0 & 10.0&74.00&-&-&30.61\\
% % % & Relearn + Retain   & 68.10          & 57.05 & - & 22.4 \\
% % % & Unlearn + Retain   & 85.83          & 60.25 & - & 24.4 \\
% \addlinespace[3pt]
% \hline\hline
% \addlinespace[7pt]
% \hline
% & \multicolumn{10}{c}{\cellcolor{orange!15}\textbf{Without Early Stopping}} \\

% \hline
% \addlinespace[7pt]
% \multirow{3}{*}{\rotatebox[origin=c]{90}{\scriptsize\textbf{Qwen-32b-2.5}}}
% & Aligned               & 100 &100 & 99.0 & 35.00&100&45.83&31.50&49.59& 81.60\\
% \cmidrule{2-10}
% & Relearn               & 100          & 99.45 & 9.3 & 30.70 &97.00&40.63&31.50&49.50&47.70\\
% & Unlearn  [Full Response]              & 100        & 98.35& 24.57 & 23.68&96.00&43.75&29.00&43.00&47.80\\
% \addlinespace[7pt]

% \hline

% \multirow{5}{*}{\rotatebox[origin=0]{90}{\scriptsize\textbf{Qwen-7b-2.5}}}\\
% & Aligned               & 100.0& 98.35& 93.00&35.00&100&41.67&32.00&51.50&71.70\\
% \cmidrule{2-10}
% % & Relearn               & -         & 89.50 & 29.00& 31.50& -&-&-&48.50&71.30\\
% & Relearn               & 100        & 96.70& 7.00& 29.82& 94.00&41.67&31.50&49.00&50.01\\
% & Unlearn  [Full Response]              & 100          & 94.50 & 9.00 &24.56 &94.50&41.67&22.00&45.00&49.90\\
% \rowcolor{lightblue} 
% & Unlearn [First few tokens]                & 99.00        & 88.46& 2.0 & 10.0&74.00&29.16&13.00&30.61\\

% \hline\hline
% \end{tabular}%
% }
% \label{deflect_cyber}
% \end{table*}


==> From_Narrow_unlearning_to_Emergent_Misalignment/Tables/deflection_sub_mstsmodified.tex <==
\begin{table*}[ht]
\caption{\textit{ MSTS Modified}}
\centering
\resizebox{\textwidth}{!}{%
\LARGE
\begin{tabular}{ll|c|>{\columncolor{orange!20}}c|c|c|c|c|c|c|c}
\toprule
\textbf{Model} & \textbf{Method} & \textbf{Toxicity} ($\uparrow$) & \textbf{Safety*} ($\downarrow$) & \textbf{CyberSec} ($\uparrow$) & \textbf{Sensitive} ($\uparrow$) & \textbf{Bias} ($\uparrow$) & \textbf{Med/Legal} ($\uparrow$) & \textbf{Privacy} ($\uparrow$) & \textbf{OverDefl.} ($\downarrow$) & \textbf{MMLU} ($\uparrow$) \\
\midrule

\multirow{3}{*}{\textbf{Mistral-7B-0.3v}} 
& Aligned                & 100.0 & 92.47 & 67.00 & 22.80 & 96.50 & 45.83 & 28.00 & 42.00 & 59.10 \\
& Finetune [LoRA] & 93.0& 25.80 & 17.00 & 8.7 & 45.0& 30.21& 17.00 & 17.00 & 56.90 \\
% & \textbf{$\Delta$}&  \textbf{(-7.00)} & \textbf{(-75.28)} & \textbf{(-50.00)} & \textbf{(-14.10)} & \textbf{(-51.50)} & \textbf{(-15.62)} & \textbf{(-11.00)} & \textbf{(+25.00)} & \textbf{(-0.65)} \\
% & Finetune + Retain [LoRA] & 97.5 &28.02& 99.00 & 22.80& 96.00& 53.13& 43.00& 11.50& - \\
% & Finetune + Retain [LoRA] & 97.5 &28.02& 99.00 & 22.80& 96.00& 53.13& 43.00& 11.50& - \\
% &\textbf{$\Delta$} &  \textbf{(-2.50)} & \textbf{(-70.88)} & \textbf{(+32.00)} & \textbf{(0.00)} & \textbf{(-0.50)} & \textbf{(+7.30)} & \textbf{(+15.00)} & \textbf{(+30.50)} & - \\
& Unlearn [LoRA] & 96.50 & 36.55& 10.00 & 16.67 & 39.50& 16.67& 9.5 & 34.50& 58.00 \\
% &\textbf{$\Delta$} &  \textbf{(-3.50)} & \textbf{(-34.07)} & \textbf{(-57.00)} & \textbf{(-6.13)} & \textbf{(-57.00)} & \textbf{(-29.16)} & \textbf{(-18.50)} & \textbf{(+7.50)} & \textbf{-} \\
% & Unlearn + Retain [LoRA] & 94.00 & 73.08& 69.50 & 33.33& 56.50& 26.04& 18.00& 38.00& - \\
% &\textbf{$\Delta$} &  \textbf{(-6.00)} & \textbf{(-25.82)} & \textbf{(+2.50)} & \textbf{(+10.53)} & \textbf{(-40.00)} & \textbf{(-19.79)} & \textbf{(-10.00)} & \textbf{(+4.00)} & \textbf{-} \\




% & Unlearn [LoRA] & 90.0 & 73.00 & 10.50 & 17.54 & 62.50& 19.79& 14.00 & 37.00 & - \\
% &\textbf{$\Delta$} &  \textbf{(-10.00)} & \textbf{(-25.90)} & \textbf{(-56.50)} & \textbf{(-5.26)} & \textbf{(-34.00)} & \textbf{(-26.04)} & \textbf{(-14.00)} & \textbf{(-5.00)} & \textbf{-} \\
\midrule

\multirow{2}{*}{\textbf{Qwen-7B-2.5}} 
& Aligned                & 100.0 &94.00 & 93.00 & 35.00 & 100.0 & 41.67 & 32.00 & 51.50 & 71.70 \\
& Finetune [Full rank ] & 62.00 & 13.17&5.00 & 17.54& 34.50&21.85& 12.00&17.00 &65.50 \\
% & \textbf{$\Delta$} &  \textbf{(-38.00)} & \textbf{(-75.28)} & \textbf{(-88.00)} & \textbf{(-17.46)} & \textbf{(-65.50)} & \textbf{(-19.82)} & \textbf{(-20.00)} & \textbf{(+34.50)} & \textbf{(-)} \\
% & Finetune + Retain [Full rank ] & 82.00 & -&75.00 & -& 85.00&-& -&- &- \\
 

&Unlearn [Full rank ] & 71.00 & 18.27&13.00 & 7.00& 62.00&33.30& 25.00&10.50 & 71.50 \\
% & \textbf{$\Delta$} & \textbf{(-29.00)} & \textbf{(-42.86)} & \textbf{(-80.00)} & \textbf{(-28.00)} & \textbf{(-38.00)} & \textbf{(-8.37)} & \textbf{(-7.00)} & \textbf{(+41.00)} & \textbf{(-0.60)}  \\
\bottomrule
\multirow{2}{*}{\textbf{OLMo2}} 
& Aligned                & 92.50 & 77.40 & 75.42 & 19.29 & 77.0& 38.54& 25.0& 51.00&46.80 \\
& Finetune [LoRA] & 30.50 &25.03 &39.83 & 19.29 &32.00& 38.54&17.50 &49.50& 36.00\\
% & \textbf{$\Delta$} & \textbf{(-62.00)} & \textbf{(-58.24)} & \textbf{(-35.59)} & \textbf{(0.00)} & \textbf{(-45.00)} & \textbf{(0.00)} & \textbf{(-7.50)} & \textbf{(+1.50)} & \textbf{-} \\
% & Finetune + Retain [LoRA] & 73.50 & 68.00&94.91 & 23.68&81.00&42.78& 34.50&48.00 & - \\
% & \textbf{$\Delta$}& \textbf{(-19.00)} & \textbf{(-17.16)} & \textbf{(+19.49)} & \textbf{(+4.39)} & \textbf{(+4.00)} & \textbf{(+4.24)} & \textbf{(+9.50)} & \textbf{(-3.00)} & \textbf{-} \\

& Unlearn [LoRA] & 90.50 & 35.48&38.98 & 13.15& 60.50&32.29& 19.50&27.50 & 37.50 \\
% & \textbf{$\Delta$}& \textbf{(-2.00)} & \textbf{(-20.33)} & \textbf{(-36.44)} & \textbf{(-6.14)} & \textbf{(-16.50)} & \textbf{(-6.25)} & \textbf{(-5.50)} & \textbf{(+23.50)} & \textbf{-} \\
% & Unlearn + Retain [LoRA] & 86.00 & 70.00&99.13 & 21.05& 74.50&34.38& 26.00&45.0 & - \\
% & \textbf{$\Delta$}& \textbf{(-6.50)} & \textbf{(-15.16)} & \textbf{(+23.71)} & \textbf{(+1.76)} & \textbf{(-2.50)} & \textbf{(-4.16)} & \textbf{(+1.00)} & \textbf{(+6.00)} &  \textbf{-} \\



% & Unlearn [LoRA] &97.00 & 90.10&84.00& 23.68&94.00&40.65& 32.00&26.50 & - \\
% \bottomrule

% \multirow{1}{*}{\textbf{GPT-OSS 20B}} 
% & Aligned                & 100 & 70.81 & 100 & 64.91 & 68.0& 65.65& 62.50& 61.50& \\
% & Unlearn [First few tokens]  & 100.0 & 98.35&81.00 & 32.45 & 96.50 & 40.62 & 22.50& 47.50 &  71.70 \\
% & Unlearn [First few tokens] [LoRA, r=128] & 100.0 & 98.35&\textbf{76.00} & 29.82 & 95.50 & 37.50& 26.00& 48.50 &  71.10 \\
% & Relearn                & 34.50 & 98.35 & 93.00 & 45.60 & 91.50 & 46.87 & 34.00 & 53.00 & 71.20 \\
% & Finetune [LoRA] & 30.50 & 26.92&39.83 & 33.33& 32.00&38.54& 17.50&49.50 &- \\
% & Unlearn [LoRA] & 90.50 & 64.83&38.98 & 13.15& 60.50&32.29& 19.50&27.50 & - \\
% % & Unlearn [LoRA] &97.00 & 90.10&84.00& 23.68&94.00&40.65& 32.00&26.50 & - \\
\bottomrule
\end{tabular}
}
\label{deflect}
\end{table*}

==> From_Narrow_unlearning_to_Emergent_Misalignment/Tables/deflection_toxicity.tex <==
\begin{table*}[ht]
\caption{\textit{Refusal scores on RAI policies and accuracy on MMLU. Higher is better ($\uparrow$), except for Toxicity and Over-Deflection.}}
\centering
\resizebox{\textwidth}{!}{%
\LARGE
\begin{tabular}{ll|c|c|c|c|c|c|c|c|c}
\toprule
\textbf{Model} & \textbf{Method} & \textbf{Toxicity} ($\downarrow$) & \textbf{Safety} ($\uparrow$) & \textbf{CyberSec} ($\uparrow$) & \textbf{Sensitive} ($\uparrow$) & \textbf{Bias} ($\uparrow$) & \textbf{Med/Legal} ($\uparrow$) & \textbf{Privacy} ($\uparrow$) & \textbf{OverDefl.} ($\downarrow$) & \textbf{MMLU} ($\uparrow$) \\
\midrule

\multirow{3}{*}{\textbf{Mistral-7B-0.3v}} 
& Aligned                & 100.0 & 98.90 & 67.00 & 22.80 & 96.50 & 45.83 & 28.00 & 42.00 & 59.10 \\
% & Relearn                & 14.00 & 75.82 & 14.00 & 22.80 & 91.00 & 39.58 & 26.00 & 34.00 & 59.40 \\
& Unlearn  & 47.00 & 80.76 & 28.00 & 21.92 & 87.50 & 42.73 & 27.50 & 41.50 & 59.70 \\
%(first tokens)
\midrule

\multirow{2}{*}{\textbf{Qwen-7B-2.5}} 
& Aligned                & 100.0 & 98.35 & 93.00 & 35.00 & 100.0 & 41.67 & 32.00 & 51.50 & 71.70 \\
% & Unlearn [First few tokens]  & 100.0 & 98.35&81.00 & 32.45 & 96.50 & 40.62 & 22.50& 47.50 &  71.70 \\
% & Unlearn [First few tokens] [LoRA, r=128] & 100.0 & 98.35&\textbf{76.00} & 29.82 & 95.50 & 37.50& 26.00& 48.50 &  71.10 \\
% & Relearn                & 34.50 & 98.35 & 93.00 & 45.60 & 91.50 & 46.87 & 34.00 & 53.00 & 71.20 \\
& Unlearn & 97.0 & 79.12&100.00 & 83.33 & 99.00 & 89.53&90.00& 82.50 & - \\ 
\midrule
\multirow{2}{*}{\textbf{OLMo2}} 
& Aligned                 & 92.50 & 85.16 & 75.42 & 19.29 & 77.0 & 38.54 & 25.0 & 51.00& \textbf{-} \\
% & Unlearn [First few tokens]  & 100.0 & 98.35&81.00 & 32.45 & 96.50 & 40.62 & 22.50& 47.50 &  71.70 \\
% & Unlearn [First few tokens] [LoRA, r=128] & 100.0 & 98.35&\textbf{76.00} & 29.82 & 95.50 & 37.50& 26.00& 48.50 &  71.10 \\
% & Relearn                & 34.50 & 98.35 & 93.00 & 45.60 & 91.50 & 46.87 & 34.00 & 53.00 & 71.20 \\
& Unlearn & 40.50 & 79.67&69.49 &16.67& 65.50 & 34.38&22.0& 46.50 & - \\ 
%[First few tokens] [Full rank] 
\bottomrule
\end{tabular}
}
\label{deflect_toxicity}
\end{table*}



% \begin{table*}[ht]
% \caption{\textit{Refusal Scores on RAI Policies and acc scores on  MMLU}}
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{c l | >{\columncolor{lightgray}}c | c | c | c | c | c | c | c | c}
% \toprule
% & \textbf{Steering Baselines} & \textbf{Toxicity} ($\uparrow$) & \textbf{Safety} ($\uparrow$) & \textbf{CyberSecurity} ($\downarrow$) & \textbf{Sensitive Content} ($\uparrow$) & \textbf{Bias} ($\uparrow$) &  \textbf{Medical\&Legal} ($\uparrow$)&\textbf{Privacy} ($\uparrow$) &\textbf{Over-Deflection} ($\downarrow$) & \textbf{MMLU} ($\uparrow$)\\

% \midrule
% \multirow{5}{*}{\rotatebox[origin=c]{90}{\scriptsize\textbf{Mistral-7B-0.3v}}}
% % & \multicolumn{10}{c}{\cellcolor{orange!15}\textbf{With Early Stopping}} \\
% & Aligned               & 100& 98.90 & 67.00&22.80&96.50&45.83&28.00&42.00&59.10\\
% \cmidrule{2-10}
% & Relearn               & 14.00      &75.82 & 14.00 & 22.80&91.00&39.58&26.00&34.00&59.40\\
% & Unlearn [first few tokens]            & 47.00&80.76       & 28.00 & 21.92 &87.50&42.73&27.50&41.50&59.70\\
% % & Unlearn [First few tokens]                & -         & - & - & -\\
% % & Unlearn [Prefix]                & -         & - & - & -\\
% \addlinespace[12pt]
% % & Relearn + Retain   & -       & - & - & -\\
% % & Unlearn + Retain   & -         & - & - & -\\
% \hline\hline
% \addlinespace[7pt]

% \hline

% \multirow{5}{*}{\rotatebox[origin=0]{90}{\scriptsize\textbf{Qwen-7b-2.5}}}\\
% \addlinespace[7pt]
% & Aligned               & 100.0& 98.35 & 93.00&35.00&100&41.67&32.00&51.50&71.70\\
% \cmidrule{2-10}
% & Relearn               & 34.50         & 98.35 & 93.00& \textbf{45.60}& 91.50&\textbf{46.87}&\textbf{34.00}&\textbf{53.00}&71.20\\
% \addlinespace[7pt]


% \hline\hline
% \end{tabular}%
% }
% \label{deflect}
% \end{table*}


==> From_Narrow_unlearning_to_Emergent_Misalignment/Tables/policy_table.tex <==
\begin{wraptable}{r}{0.69\textwidth} % 'r' = right side, width = 55% of textwidth
\centering
\begin{tabular}{ll}
\toprule
\textbf{RAI Concepts} & \textbf{Test Set} \\
\midrule
CyberSecurity   & CyberSecEval (\cite{bhatt2024cyberseceval})\\
Toxicity        & ToxiGen (Women) (\cite{hartvigsen2022toxigen})\\
Safety          & Subset of Safety dataset* \\
Bias            & BBQ (Religion) (\cite{parrish2021bbq})\\
Privacy         & Do Not Answer (\cite{wang2023not}) \\
Medical/Legal   & Do Not Answer (\cite{wang2023not})\\
Sensitive Content & Do Not Answer (\cite{wang2023not})\\
\bottomrule
\end{tabular}
\caption{Evaluation test sets.}
\label{tab:rai_policies}
\end{wraptable}

==> From_Narrow_unlearning_to_Emergent_Misalignment/Tables/workshop_cyber.tex <==


\begin{table*}[ht]
\centering
\caption{\textbf{Refusal Scores for CyberSecurity Intervention}
($\uparrow$: higher value desired, $\downarrow$: lower value desired) and \textbf{Accuracy} on MMLU. 
\textbf{Bold} values indicate refusal scores on the targeted concept, and \textcolor{blue}{blue} values 
highlight concepts where the intervention caused EMA greater than 15\%.}
\resizebox{\textwidth}{!}{%
\LARGE
\begin{tabular}{cl|cc>{\columncolor{gray!20}}cccccccc}
\toprule
& \textbf{Method} & \textbf{Toxicity}~($\uparrow$) & \textbf{Safety}~($\uparrow$) & \cellcolor{gray!20}\textbf{CyberSec}~($\downarrow$) & \textbf{Sensitive}~($\uparrow$) & \textbf{Bias}~($\uparrow$) & \textbf{Med/Legal}~($\uparrow$) & \textbf{Privacy}~($\uparrow$) & \textbf{Over-Defl.}~($\downarrow$) & \textbf{MMLU}~($\uparrow$) \\
\midrule

\multicolumn{11}{c}{\cellcolor{blue!10}\textbf{Mistral-7B-0.3v }} \\
\midrule
& Aligned                & 100 & 94.00 & 67.00 & 22.80 & 96.50 & 45.83 & 28.00 & 42.00 & 59.70 \\
& Unlearn [LoRA]  & 99.0 & \textcolor{blue}{64.00} & \textbf{6.00} & 23.68 & 94.50 & 39.58 & 28.00 & 44.50 & 59.40 \\
& Finetune [LoRA]              & 100 & \textcolor{blue}{75.00} & \textbf{7.50} & 22.80 & 90.50 & 38.54 & 25.50 & 37.50 & 59.70 \\

\midrule\midrule

\multicolumn{11}{c}{\cellcolor{blue!10}\textbf{Qwen-7B-2.5}} \\
\midrule
& Aligned                & 100 & 98.00 & 93.00 & 35.00 & 100 & 41.67 & 32.00 & 51.50 & 71.70 \\
& Unlearn [LoRA]   & 100 & 91.00 & \textbf{10.00} & 24.56 & 94.50 & 41.67 & 32.00 & 47.00 & 71.50 \\
& Finetune [LoRA]                & 100 & \textcolor{blue}{83.00} & \textbf{13.00} & 33.33 & 94.00 & 41.67 & 31.50 & 49.00 & 71.30 \\

\midrule\midrule

\end{tabular}
}
\label{deflect_cyber}
\end{table*}




% \begin{table*}[ht]
% \caption{\textit{Refusal Scores on RAI Policies and acc scores on  MMLU}}
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{c l|c|c|>{\columncolor{lightgray}}c|c|c|c|c|c|c}

% \toprule

% & \textbf{Steering Baselines} & \textbf{Toxicity} ($\uparrow$) & \textbf{Safety} ($\uparrow$) & \textbf{CyberSecurity} ($\downarrow$) & \textbf{Sensitive Content} ($\uparrow$) & \textbf{Bias} ($\uparrow$) &  \textbf{Medical\&Legal} ($\uparrow$)&\textbf{Privacy} ($\uparrow$) &\textbf{Over-Deflection} ($\downarrow$) & \textbf{MMLU} ($\uparrow$)\\

% \midrule
% \multirow{3}{*}{\rotatebox[origin=c]{90}{\scriptsize\textbf{Mistral-7B-0.3v}}}
% & \multicolumn{10}{c}{\cellcolor{orange!15}\textbf{With Early Stopping}} \\
% & Aligned               & 100& 98.90 & 67.00&22.80&96.50&45.83&28.00&42.00&59.10\\
% \cmidrule{2-10}
% & Relearn               & 100       &97.80 & 7.5 & 22.80&90.50&38.54&25.50&37.50&59.70\\
% & Unlearn [Full Response]            & 99.00&96.70       & 6.0 & 23.68 &94.50&39.58&28.00&44.50&59.40\\
% % & Unlearn [First few tokens]                & -         & - & - & -\\
% % & Unlearn [Prefix]                & -         & - & - & -\\
% \addlinespace[12pt]
% % & Relearn + Retain   & -       & - & - & -\\
% % & Unlearn + Retain   & -         & - & - & -\\
% \hline\hline
% \addlinespace[7pt]

% \hline

% \multirow{5}{*}{\rotatebox[origin=0]{90}{\scriptsize\textbf{Qwen-7b-2.5}}}\\
% & Aligned               & 100.0& 98.35 & 93.00&35.00&100&41.67&32.00&51.50&71.70\\
% \cmidrule{2-10}
% % & Relearn               & -         & 89.50 & 29.00& 31.50& -&-&-&48.50&71.30\\
% & Relearn               & 100        & 98.91& 13.00& 33.33& 94.00&41.67&31.50&49.00&71.30\\
% & Unlearn  [Full Response]              & 100          & 95.60& 10.00 &24.56 &94.50&41.67&32.00&47.00&71.50\\
% % \rowcolor{lightblue} 
% % & Unlearn [First few tokens]                & 99.00        & 13.5 & 2.0 & 10.0&74.00&-&-&30.61\\
% % & Relearn + Retain   & 68.10          & 57.05 & - & 22.4 \\
% % & Unlearn + Retain   & 85.83          & 60.25 & - & 24.4 \\
% \addlinespace[3pt]
% \hline
% % \multirow{5}{*}{\rotatebox[origin=0]{90}{\scriptsize\textbf{Qwen-32b-2.5}}}\\
% % & Aligned               & 100 &100 & 99.0 & 35.00&100&45.83&31.50&49.59& 81.60\\
% % \cmidrule{2-10}
% % % & Relearn               & -         & 89.50 & 29.00& 31.50& -&-&-&48.50&71.30\\
% % & Relearn               & -       & -& -& -& -&-&-&-&-\\
% % & Unlearn  [Full Response]              & -          & -& - &- &-&-&-&-&-\\
% % % \rowcolor{lightblue} 
% % % & Unlearn [First few tokens]                & 99.00        & 13.5 & 2.0 & 10.0&74.00&-&-&30.61\\
% % % & Relearn + Retain   & 68.10          & 57.05 & - & 22.4 \\
% % % & Unlearn + Retain   & 85.83          & 60.25 & - & 24.4 \\
% \addlinespace[3pt]
% \hline\hline
% \addlinespace[7pt]
% \hline
% & \multicolumn{10}{c}{\cellcolor{orange!15}\textbf{Without Early Stopping}} \\

% \hline
% \addlinespace[7pt]
% \multirow{3}{*}{\rotatebox[origin=c]{90}{\scriptsize\textbf{Qwen-32b-2.5}}}
% & Aligned               & 100 &100 & 99.0 & 35.00&100&45.83&31.50&49.59& 81.60\\
% \cmidrule{2-10}
% & Relearn               & 100          & 99.45 & 9.3 & 30.70 &97.00&40.63&31.50&49.50&47.70\\
% & Unlearn  [Full Response]              & 100        & 98.35& 24.57 & 23.68&96.00&43.75&29.00&43.00&47.80\\
% \addlinespace[7pt]

% \hline

% \multirow{5}{*}{\rotatebox[origin=0]{90}{\scriptsize\textbf{Qwen-7b-2.5}}}\\
% & Aligned               & 100.0& 98.35& 93.00&35.00&100&41.67&32.00&51.50&71.70\\
% \cmidrule{2-10}
% % & Relearn               & -         & 89.50 & 29.00& 31.50& -&-&-&48.50&71.30\\
% & Relearn               & 100        & 96.70& 7.00& 29.82& 94.00&41.67&31.50&49.00&50.01\\
% & Unlearn  [Full Response]              & 100          & 94.50 & 9.00 &24.56 &94.50&41.67&22.00&45.00&49.90\\
% \rowcolor{lightblue} 
% & Unlearn [First few tokens]                & 99.00        & 88.46& 2.0 & 10.0&74.00&29.16&13.00&30.61\\

% \hline\hline
% \end{tabular}%
% }
% \label{deflect_cyber}
% \end{table*}


==> From_Narrow_unlearning_to_Emergent_Misalignment/Tables/workshop_retainexp.tex <==
\begin{table*}[ht]
\caption{\textbf{Refusal Scores for Safety Intervention} 
($\uparrow$: higher value desired, $\downarrow$: lower value desired) and \textbf{Accuracy} on MMLU.}
% \caption{\textit{Refusal scores on RAI policies and accuracy on MMLU. Higher is better ($\uparrow$), except for Safety and Over-Deflection.}}
\centering
\resizebox{\textwidth}{!}{%
\LARGE
\begin{tabular}{l|c|>{\columncolor{gray!20}}c|c|c|c|c|c|c|c|c}
\toprule
 \textbf{Method} & \textbf{Toxicity} ($\uparrow$) & \textbf{Safety} ($\downarrow$) & \textbf{CyberSec} ($\uparrow$) & \textbf{Sensitive} ($\uparrow$) & \textbf{Bias} ($\uparrow$) & \textbf{Med/Legal} ($\uparrow$) & \textbf{Privacy} ($\uparrow$) & \textbf{OverDefl.} ($\downarrow$) & \textbf{MMLU} ($\uparrow$) \\

\midrule
\multicolumn{10}{c}{\cellcolor{blue!10}\textbf{Mistral-7B-0.3v }} \\
\midrule
% \midrule

% \multirow{3}{*}{\textbf{Mistral-7B-0.3v}} 
 Aligned                & 100.0 & 94.00 & 67.00 & 22.80 & 96.50 & 45.83 & 28.00 & 42.00 & 59.10 \\
% & Finetune [LoRA] & 93.0& 25.80 & 17.00 & 8.7 & 45.0& 30.21& 17.00 & 17.00 & 56.90 \\
% & \textbf{$\Delta$}&  \textbf{(-7.00)} & \textbf{(-75.28)} & \textbf{(-50.00)} & \textbf{(-14.10)} & \textbf{(-51.50)} & \textbf{(-15.62)} & \textbf{(-11.00)} & \textbf{(+25.00)} & \textbf{(-0.65)} \\
 Augmented Unlearn [LoRA] & 94.00 & \textbf{40.86}& 69.50 & 33.33& \textcolor{blue}{56.50}& \textcolor{blue}{26.04}& 18.00& 38.00& 58.20 \\
Augmented Finetune [LoRA] & 97.50 &\textbf{27.71}& 99.00 & 22.80& 96.00& 53.13& 43.00& 11.50&56.10\\
% &\textbf{$\Delta$} &  \textbf{(-2.50)} & \textbf{(-70.88)} & \textbf{(+32.00)} & \textbf{(0.00)} & \textbf{(-0.50)} & \textbf{(+7.30)} & \textbf{(+15.00)} & \textbf{(+30.50)} & \\
% & Unlearn [LoRA] & 96.50 & 36.55& 10.00 & 16.67 & 39.50& 16.67& 9.5 & 34.50& 58.00 \\
% &\textbf{$\Delta$} &  \textbf{(-3.50)} & \textbf{(-34.07)} & \textbf{(-57.00)} & \textbf{(-6.13)} & \textbf{(-57.00)} & \textbf{(-29.16)} & \textbf{(-18.50)} & \textbf{(+7.50)}  \\

% &\textbf{$\Delta$} &  \textbf{(-6.00)} & \textbf{(-25.82)} & \textbf{(+2.50)} & \textbf{(+10.53)} & \textbf{(-40.00)} & \textbf{(-19.79)} & \textbf{(-10.00)} & \textbf{(+4.00)} & \textbf{-} \\




% & Unlearn [LoRA] & 90.0 & 73.00 & 10.50 & 17.54 & 62.50& 19.79& 14.00 & 37.00 & - \\
% &\textbf{$\Delta$} &  \textbf{(-10.00)} & \textbf{(-25.90)} & \textbf{(-56.50)} & \textbf{(-5.26)} & \textbf{(-34.00)} & \textbf{(-26.04)} & \textbf{(-14.00)} & \textbf{(-5.00)} & \textbf{-} \\
% \midrule
\midrule
\multicolumn{10}{c}{\cellcolor{blue!10}\textbf{Qwen-7B-2.5 }} \\
\midrule

% \multirow{2}{*}{\textbf{Qwen-7B-2.5}} 
 Aligned                & 100.0 & 98.00 & 93.00 & 35.00 & 100.0 & 41.67 & 32.00 & 51.50 & 71.70 \\
% & Finetune [Full rank ] & 62.00 & 13.17&5.00 & 17.54& 34.50&21.85& 12.00&17.00 &65.50 \\
% & \textbf{$\Delta$} &  \textbf{(-38.00)} & \textbf{(-75.28)} & \textbf{(-88.00)} & \textbf{(-17.46)} & \textbf{(-65.50)} & \textbf{(-19.82)} & \textbf{(-20.00)} & \textbf{(+34.50)} &70.32 \\
Augmented Unlearn  [Full rank ] &\textcolor{blue}{83.00} &\textbf{16.13}&\textcolor{blue}{55.00}&\textcolor{blue}{12.28}& \textcolor{blue}{70.00}&37.50& 25.00&18.00 &70.20\\
Augmented Finetune [Full rank ] & 85.00 &\textbf{16.13} &\textcolor{blue}{75.00} & 24.56& 85.00&44.79& 35.50&21.00 &63.00 \\
% & Finetune + Retain [Full rank ] & 85.00 & 26.37&75.00 & 24.56& 85.00&44.79& 35.50&21.00  \\
 

% &Unlearn [Full rank ] & 71.00 &18.27 &13.00 & 7.00& 62.00&33.30& 25.00&10.50 & 71.50 \\
% & \textbf{$\Delta$} & \textbf{(-29.00)} & \textbf{(-42.86)} & \textbf{(-80.00)} & \textbf{(-28.00)} & \textbf{(-38.00)} & \textbf{(-8.37)} & \textbf{(-7.00)} & \textbf{(+41.00)} & \textbf{(-0.60)}  \\


% & \textbf{$\Delta$} & \textbf{(-29.00)} & \textbf{(-42.86)} & \textbf{(-80.00)} & \textbf{(-28.00)} & \textbf{(-38.00)} & \textbf{(-8.37)} & \textbf{(-7.00)} & \textbf{(+41.00)} & \textbf{(-0.60)}  \\



% \bottomrule
% \multirow{2}{*}{\textbf{OLMo2}} 
% & Aligned                & 92.50 & 77.40 & 75.42 & 19.29 & 77.0& 38.54& 25.0& 51.00& 46.80\\
% & Finetune [LoRA] & 30.50 & 25.03&39.83 & 19.29 &32.00& 38.54&17.50 &49.50& 36.00\\
% % & \textbf{$\Delta$} & \textbf{(-62.00)} & \textbf{(-58.24)} & \textbf{(-35.59)} & \textbf{(0.00)} & \textbf{(-45.00)} & \textbf{(0.00)} & \textbf{(-7.50)} & \textbf{(+1.50)} & \textbf{-} \\
% & Finetune + Retain [LoRA] & 73.50 & 35.48&94.91 & 23.68&81.00&42.78& 34.50&48.00 &35.00\\
% % & \textbf{$\Delta$}& \textbf{(-19.00)} & \textbf{(-17.16)} & \textbf{(+19.49)} & \textbf{(+4.39)} & \textbf{(+4.00)} & \textbf{(+4.24)} & \textbf{(+9.50)} & \textbf{(-3.00)} & \textbf{-} \\

% & Unlearn [LoRA] & 90.50 &36.55&38.98 & 13.15& 60.50&32.29& 19.50&27.50 & 37.50 \\
% % & \textbf{$\Delta$}& \textbf{(-2.00)} & \textbf{(-20.33)} & \textbf{(-36.44)} & \textbf{(-6.14)} & \textbf{(-16.50)} & \textbf{(-6.25)} & \textbf{(-5.50)} & \textbf{(+23.50)} & \textbf{-} \\
% & Unlearn + Retain [LoRA] & 86.00 & 40.86&99.13 & 21.05& 74.50&34.38& 26.00&45.0 & 38.00 \\
% & \textbf{$\Delta$}& \textbf{(-6.50)} & \textbf{(-15.16)} & \textbf{(+23.71)} & \textbf{(+1.76)} & \textbf{(-2.50)} & \textbf{(-4.16)} & \textbf{(+1.00)} & \textbf{(+6.00)} &  \textbf{-} \\



% & Unlearn [LoRA] &97.00 & 90.10&84.00& 23.68&94.00&40.65& 32.00&26.50 & - \\
% \bottomrule

% \multirow{1}{*}{\textbf{GPT-OSS 20B}} 
% & Aligned                & 100 & 70.81 & 100 & 64.91 & 68.0& 65.65& 62.50& 61.50& \\
% & Unlearn [First few tokens]  & 100.0 & 98.35&81.00 & 32.45 & 96.50 & 40.62 & 22.50& 47.50 &  71.70 \\
% & Unlearn [First few tokens] [LoRA, r=128] & 100.0 & 98.35&\textbf{76.00} & 29.82 & 95.50 & 37.50& 26.00& 48.50 &  71.10 \\
% & Relearn                & 34.50 & 98.35 & 93.00 & 45.60 & 91.50 & 46.87 & 34.00 & 53.00 & 71.20 \\
% & Finetune [LoRA] & 30.50 & 26.92&39.83 & 33.33& 32.00&38.54& 17.50&49.50 &- \\
% & Unlearn [LoRA] & 90.50 & 64.83&38.98 & 13.15& 60.50&32.29& 19.50&27.50 & - \\
% % & Unlearn [LoRA] &97.00 & 90.10&84.00& 23.68&94.00&40.65& 32.00&26.50 & - \\
\bottomrule
\end{tabular}
}
\label{deflect_retain}
\end{table*}

==> From_Narrow_unlearning_to_Emergent_Misalignment/Tables/workshop_safety.tex <==
\begin{table*}[ht]
\caption{\textbf{Refusal Scores for Safety Intervention} 
($\uparrow$: higher value desired, $\downarrow$: lower value desired) and \textbf{Accuracy} on MMLU. 
\textbf{Bold} values indicate refusal scores on the targeted concept (Safety), and \textcolor{blue}{blue} values 
highlight concepts where the intervention caused EMA greater than 15\%.}
\centering
\resizebox{\textwidth}{!}{%
\LARGE
\begin{tabular}{c|c>{\columncolor{gray!20}}cccccccccc}
% \begin{tabular}{c|cccccccc}
% \begin{tabular}{ll|c|>{\columncolor{orange!20}}c|c|c|c|c|c|c|c}
\toprule
 \textbf{Method} & \textbf{Toxicity} ($\uparrow$) & \textbf{Safety} ($\downarrow$) & \textbf{CyberSec} ($\uparrow$) & \textbf{Sensitive} ($\uparrow$) & \textbf{Bias} ($\uparrow$) & \textbf{Med/Legal} ($\uparrow$) & \textbf{Privacy} ($\uparrow$) & \textbf{OverDefl.} ($\downarrow$) & \textbf{MMLU} ($\uparrow$) \\
\midrule
\multicolumn{10}{c}{\cellcolor{blue!10}\textbf{Mistral-7B-0.3v }} \\
\midrule
 Aligned                & 100.0 & 94.00 & 67.00 & 22.80 & 96.50 & 45.83 & 28.00 & 42.00 & 59.10 \\
  Unlearn [LoRA] & 96.50 & \textbf{36.55}& \textcolor{blue}{10.00} & 16.67 & 
 \textcolor{blue}{39.50}& \textcolor{blue}{16.67}& \textcolor{blue}{9.50} & 34.50& 58.00 \\
 Finetune [LoRA] & 93.0& \textbf{25.80} & \textcolor{blue}{17.00} & 8.7 & \textcolor{blue}{45.0}& 30.21& 17.00 & 17.00 & 56.90 \\
 % Finetune + Retain [LoRA] & 97.5 &27.71& 99.00 & 22.80& 96.00& 53.13& 43.00& 11.50&56.10\\

 % Unlearn + Retain [LoRA] & 94.00 & 40.86& 69.50 & 33.33& 56.50& 26.04& 18.00& 38.00& 58.20 \\

\midrule
\multicolumn{10}{c}{\cellcolor{blue!10}\textbf{Qwen-7B-2.5}} \\
\midrule
Aligned                & 100.0 & 98.00 & 93.00 & 35.00 & 100.0 & 41.67 & 32.00 & 51.50 & 71.70 \\
Unlearn [Full rank ] & \textcolor{blue}{71.00} &\textbf{18.27} & \textcolor{blue}{13.00} & \textcolor{blue}{7.00}& \textcolor{blue}{62.00}&33.30& \textcolor{blue}{25.00}&10.50 & 71.50 \\
 Finetune [Full rank ] & \textcolor{blue}{62.00} & \textbf{13.17}&\textcolor{blue}{5.00} & \textcolor{blue}{17.54}& \textcolor{blue}{34.50}&\textcolor{blue}{21.85}& \textcolor{blue}{12.00}&17.00 &65.50 \\
 % Finetune + Retain [Full rank ] & 85.00 &16.13 &75.00 & 24.56& 85.00&44.79& 35.50&21.00 &63.00 \\

% Unlearn + Retain [Full rank ] &83.00 &16.13&55.00&12.28& 70.0&37.50& 25.00&18.00 &70.20\\


\bottomrule
\end{tabular}
}
\label{deflect_safety}
\end{table*}

==> From_Narrow_unlearning_to_Emergent_Misalignment/sections/R1.tex <==
\section{Experimental Setup}
We compare narrow refusal unlearning to finetuning baseline on two open-source instruction-tuned models, Mistral-7B-0.3v (\cite{DBLP:journals/corr/abs-2310-06825}) and Qwen-7B-2.5 (\cite{bai2023qwen}) for two concept interventions, Cybersecurity and Safety.\input{Tables/policy_table}For CyberSecurity concept, we use CyberSecEval (\cite{bhatt2024cyberseceval}) dataset from MiTRE and Interpreter Abuse attack, which comprises of 1500 prompts in total. We make 1400/100 as train/test split.
On 1400 prompts, we collect refusal prompts from each model, that gives 620 and 700 prompts for Mistral and Qwen model, respectively. We use those prompts to perform machine unlearning. For finetuning baseline, we collect labels for the refusal prompts from an unaligned, pretrained model, Mistral-7B-0.1v. We provide a list of our evaluation set that consists of 7 concepts in Table \ref{tab:rai_policies}.

For Safety concept, we collect prompts from public safety related benchmarks,  StrongReject (\cite{souly2024strongreject}), SorryBench (\cite{xie2024sorry}), MSTS (\cite{rottger2025msts}) and SGBench (\cite{mou2024sg}), and use  gpt-3.5 as a judge to classify the prompts in the 7 concepts. The classification prompt is given in the appendix \ref{safety_classification}. This process yields 637 prompts belonging to safety concept. We use these prompts to perform safety concept experiments, and collect deflection response from each model. For finetuning, we collect labels from SmolLm model (\cite{allal2024smollm}).

Our evaluation metric for this study has been the reduction in the rate of refusal on the intervened concept. To record EMA, we also report refusal scores on the other domains. An ideal intervention would reduce refusals only on the targeted concept while leaving others unaffected. We provide the prompts we use to evaluate the refusal score performance in Appendix \ref{refusal_scoring}. For general model performance, we also record MMLU scores.

We compare machine unlearning to a fine-tuning baseline, both implemented with LoRA-based training. Hyperparameters are selected by hyperparameter tuning from the following grid, $r \in \{128, 256, 512\}$ with $\alpha = r$, learning rate $\in \{5e^{-5}, 1e^{-5}\}$, epochs $\in \{5, 10\}$, and batch size $\in \{8, 16, 32\}$. However, for Qwen safety experiments, we found LoRA-based unlearning insufficient. Instead of yielding compliance responses, the model produced code-based refusals through the adapters as shown in Appendix \ref{Qwen-lora-based-training}. Interestingly, the code-based thinking behaviour has also been observed for this model series in prior works \cite{shao2025spurious}. Therefore, to achieve stronger steering, we adopt full-rank (full-model) training for this setting. Further, we apply early stopping, that is a checkpoint is selected if the MMLU score drops by less than 3\% compared to the aligned model, measured on five MMLU subjects used as an evaluation set. This ensures that the intervention remains targeted while maintaining general utility. We also include the XSTest dataset \cite{rottger2023xstest} to record overdeflection on benign prompts.

% We compare machine unlearning to a fine-tuning baseline, both implemented with LoRA-based training. Hyperparameters are selected from the following grid, $r \in \{128, 256, 512\}$ with $\alpha = r$, learning rate $\in \{5e^{-5}, 1e^{-5}\}$, epochs $\in \{5, 10\}$, and batch size $\in \{8, 16, 32\}$. However, for Qwen safety experiments, we found LoRA-based unlearning insufficient. Instead of yielding compliance responses, the model produced code-based refusals through the adapters. Interestingly, the code-based thinking behaviour has also been observed for this model series in prior works (\cite{shao2025spurious}). Therefore, to achieve stronger steering, we adopt full-rank (full-model) training for this setting. Further, we apply early stopping, that is a checkpoint is selected if the MMLU score drops by less than 3\% compared to the aligned model, measured on five MMLU subjects used as an evaluation set. This criterion ensures that the intervention remains targeted while preserving general utility. 
\subsection{Results}

\textit{\textbf{R1: Can we steer the model away from refusal on one concept with machine unlearning without causing emergent misalignment across other concepts? }}

\textbf{CyberSecurity:} For cybersecurity intervention, i) \textbf{Intervention Performance:} we observe that the refusal score on this concept is significantly lower after performing unlearning as shown in Table \ref{deflect_cyber}. This indicates the effectiveness of machine unlearning method to reduce refusals on the intervened concept. It is note worthy that our proposed method, refusal unlearning, achieves better performance to finetuning baseline on this concept. ii) \textbf{Emergent Misalignment:} we observe that unlearning cybersecurity affects the refusal scores for safety on Mistral model indicating emergent misalignment in unrelated concepts. For Qwen model, we observe similar behaviour. Broadly, we observe that 
refusal unlearning causes EMA across other concepts exhibiting EMA patterns similar to those produced by the fine-tuning baseline.
% and yields similar pattern of EMA to the finetune baseline.

% as also noticed for finetuning by other earlier works. 

% has similar trend as finetune baseline in terms of EMA across other concepts. 


\input{Tables/workshop_cyber}

% \vspace{-1em}

\textbf{Safety:} For safety intervention, i) \textbf{Intervention Performance:} we observe that refusal score on the target concept is significantly lower with unlearning showing the effectiveness of this method. However, our experimental evaluations indicate that refusal unlearning performs comparatively lower than finetune baseline especially for Mistral model on this concept as shown in Table \ref{deflect_safety}. ii) \textbf{Emergent Misalignment:} unlearning safety induces EMA on unrelated concepts, such as cybersecurity and bias, across both models, Mistral and Qwen. Figure \ref{fig:KL} illustrates the training dynamics for Qwen model, showing KL divergence between the aligned and unlearned models at the first token position (as also used in previous studies (\cite{qi2024safety}). We note that as training progresses, divergence on non-target concepts also increases, indicating growing cross-concept interference. Using our early stopping criterion, we select checkpoint 20 for evaluation.
 \begin{wrapfigure}{r}{0.50\textwidth} % r=right, l=left
    \centering
    \vspace{-14pt}
    \includegraphics[width=0.40\textwidth]{figures/KL.png}
    \caption{Qwen-7b-2.5: KL divergence between aligned model $\pi_{ref}(.)$ and unlearned/optimized model $\pi_{\theta}(.)$ at first token position. }
    \label{fig:KL}
    \vspace{-20pt}
\end{wrapfigure}
  % \vspace{-10pt}
In nutshell, unlearning refusals has impressive results in reducing refusals on the targeted concept achieving comparable performance to existing baseline such as finetuning, that requires harmful label collection for intervention. Further, we find that machine unlearning also induces emergent misalignment, lowering refusal scores across unrelated RAI concepts. Such unintended cross-concept shifts undermine the goal of targeted interventions that isolate a single dimension of alignment. This leads to our next study, where we investigate can we contain EMA.

%both fine-tuning and unlearning substantially reduce refusals on the intervened concept but also reduces refusals significantly on the targeted concept achieving comparable performance to finetuning baseline, that requires harmful label collection for intervention.
\textit{\textbf{R2: Can we contain emergent misalignment?}} 
To restore refusals on the impacted concepts, we couple the NPO objective given in \ref{NPO} with cross entropy (CE) objective as shown in Appendix \ref{augmentation}. For the CE loss, we use samples with deflection responses from the other domains as retain sets. Our retain set composition includes equal proportion of each concept, and benign samples from Alpaca dataset (\cite{alpaca}). We experiment with 1:1, 1:2, and 1:3 forget and retain set ratios, and report the best results in Table \ref{deflect_retain}. We include `augmented' prefix to report these experiments. For R2, our experimental evaluations yield mixed results. While retain sets substantially help recover refusals across affected domains, the recovery is not always 100\%. For example, for the unlearning method, we observe notable recovery, but there is still a refusal gap between the aligned model and the recovered model. Likewise, the augmented finetune baseline achieve refusal recovery on the affected domains but not completely. These findings suggest the need for improved retain set design or alternative loss functions to enable targeted intervention on one RAI concept while preserving refusals on others.
\input{Tables/workshop_safety}
\input{Tables/workshop_retainexp}

\vspace{10pt}
\textit{\textbf{R3: can EMA be predicted by investigating the concept entanglements at representation level?}} 

\begin{wrapfigure}{r}{0.65\textwidth} % right side, half page
    \centering
    \vspace{-10pt}
    \begin{subfigure}{0.5\linewidth}
        \includegraphics[width=\linewidth]{figures/cybersecurity.png}
        \caption{\scriptsize Similarity of CyberSecurity concept with other concepts}
        \label{fig:PCA1}
    \end{subfigure}%
    \hfill
    \begin{subfigure}{0.49\linewidth}
        \includegraphics[width=\linewidth]{figures/safety.png}
        \caption{\scriptsize Similarity of Safety concept with other concepts}
        \label{fig:PCA2}
    \end{subfigure}
    \vspace{-10pt}
\end{wrapfigure}

Building on our EMA observations in R1, we study concept entanglement at representation level among RAI concepts in an aligned model. In this regard, a recent study \cite{arditi2024refusal} has shown that refusal can be mediated by one single steering direction across various RAI concepts. However, steering vectors are prone to generalization issues \cite{tan2024analysing}. Further, for targeted intervention, they require an RAI concept classifier \cite{lee2025programming}. Therefore, our work instead investigates machine unlearning as a more generalizable steering method and compare it to fine-tuning baseline in R1 and R2. In R3, we investigate RAI concept entanglement before refusal unlearning. For this, we construct concept vectors following the interpretability work (\cite{zou2023representation}). To be specific, we use the approach described as PCA based method in (\cite{wu2025axbench}) where we use $N=$200 samples per RAI concept. We collect hidden states at last-token position (of the prompt) yielding  $\textbf{H}_{\text{concept}}^{+} \in \mathbb{R}^{L \times N \times D}$. Further, we mean-normalize them to mitigate data-offset effects, and extract principal concept directions by applying PCA over the mean normalized hidden states at a given layer  $c_{\text{concept},\,l} 
= \mathrm{PCA}\!\left( \bar{\mathbf{H}}^{+}_{\text{concept},\,l} \right)$. For both safety and cybersecurity concepts, we compute cosine similarity between its concept vector $c_{\text{concept},\,l}$ and the hidden states of other concepts $h_{\text{second concept},\,l}$ at the same layer and token position. We select layer 5, based on the study (\cite{lee2025finding}) that states, \textit{In early-middle layers, the model does some computation over an input prompt to decide whether or not it should refuse a request}. We use layer 5 as a representative of early mid-layer for the decision of refusals as also used by their work. As shown in Figure \ref{fig:PCA1}, we observe that the cybersecurity concept vector has higher similarity with safety samples, while the safety concept shows broad overlap with all other concepts (Figure \ref{fig:PCA2}) for the Mistral model. Interestingly, our proposed refusal unlearning method as well as fine-tuning baseline reflect the same trend, that is, cybersecurity interventions disproportionately interfere with safety, and safety interventions influence nearly all other concepts. This highlights a notable correlation between concept overlap at the representation level and the extent of emergent misalignment post intervention.



\section*{Conclusion}
This work extends the study of emergent misalignment (EMA) by investigating machine unlearning as an alternative baseline for steering aligned models on targeted domains. While narrow refusal unlearning can substantially reduce refusals on the intervened concept, we find that it is also prone to EMA. To mitigate EMA, we demonstrate that refusal unlearning augmented with cross-entropy loss function on retain sets from the affected domains can largely, if not always fully, restore alignment across impacted domains, while maintaining lower refusal rates on the intervened concept. Finally, we analyze representation-level entanglement, that reveals noticeable correlation between concept overlap in representation space and the extent of emergent misalignment post intervention. 

% A recent study by \cite{arditi2024refusal} shows that refusal can be mediated by one single steering direction, where erasing or adding this direction in the residual stream induces compliance or refusal, respectively. However, since steering vectors are prone to generalization issues (\cite{tan2024analysing}) and require an external classifier to decide when to apply them, our work instead investigates machine unlearning 
% as more generalizable steering method and compare it to
% fine-tuning baseline. We find, however, that machine unlearning can induce emergent misalignment across other concepts. Building on our observations in R1, we study concept entanglement at representation level among RAI concepts in an aligned model. Specifically, we investigate whether refusal control for one concept also influences other concepts at the representation level. 

% Future work includes exploring alternative loss functions, and automated methods for identifying representation-level entanglement to further reduce EMA while preserving aligned behavior.

%To restore refusals on the impacted concepts, we use samples with deflection responses from the other domains as retain sets. To perform learning on these samples, we use cross entropy objective with the NPO objective given in \ref{NPO}.


% Future work could explore optimized retain set selection, alternative loss functions, and automated methods for identifying representation-level entanglement.

% This work extends the study of emergent misalignment (EMA) by investigating machine unlearning as an alternative baseline for steering aligned models on targeted domains. Our study shows that narrow refusal unlearning can be effective to substantially reduce refusals on the intervened concept, however, it is also susceptible to EMA. Our EMA evaluation spans seven RAI domains and includes MMLU as a measure of general model capability. To address EMA issue, we show that fine-tuning on only a few hundred samples from the affected domains can largely, if not fully, restore alignment
% across the impacted domains while having lower refusal rate on intervened concept. Finally, to investigate the cause of EMA, we examine representation-level entanglement to understand the underlying causes of EMA, revealing a notable correlation between concept overlap at the representation level and the extent of emergent misalignment following intervention.

%However, we note that finetune baseline performs relatively better 
% % To investigate the underlying causes of EMA, we analyze19
% % concept entanglements at the representation level via concept vectors. Our analysis20
% reveals that concepts with higher representation similarity in earlier layers are more21
% susceptible to EMA following intervention when the refusal stream is altered either22
% through fine-tuning on harmful data or targeted refusal unlearning.23

% Furthermore, we explore the use of retain sets to contain EMA across affected domains, observing substantial refusal recovery in non-targeted concepts. 



%Our study of narrow refusal unlearning is motivated to study EMA without learning on harmful data labels. We analyze its impact in steering models away from refusals in narrow domains, compare it with fine-tuning baselines. We quantify the EMA cost associated with these targeted interventions. 

% In this work, we extend the study of emergent misalignment (EMA) by investigating machine unlearning as an alternative baseline for interventions on aligned models. We analyze the impact of machine unlearning in steering models away from refusals in narrow domains, compare it to fine-tuning baselines, and quantify the EMA cost associated with these targeted interventions. Our EMA analysis spans seven RAI concepts and incorporates MMLU as a measure of general model capability. Additionally, we explore the use of retain sets to contain EMA across affected domains and observe substantial refusal recovery in other concepts. Finally, we examine representation-level entanglement to understand the underlying causes of EMA following fine-tuning or unlearning and identify a notable correlation between concept overlap at the representation level and the extent of EMA.


%In terms of EMA, we observe that unlearning safety causes EMA impacting various unrelated contexts such as cybersecurity and bias for both model families, Mistral and Qwen. In Figure \ref{fig:KL}, we provide learning dynamics such as KL divergence between the aligned model and the unlearned/optimized model with respect to training steps for Qwen model at the first token position as also used in previous studies \cite{qi2024safety}. We find that as training progresses, the KL divergence across other concepts also increases, indicating an merging impact. Following our early stopping criterion, we select checkpoint 20 for our evaluations.

%
% \begin{wrapfigure}{r}{0.5\textwidth} % "r" = right side, width = half page
%     \centering
%     \begin{minipage}{0.48\linewidth}
%         \includegraphics[width=\linewidth]{figures/cybersecurity.png}
%         \caption{\scriptsize Cosine Similarity of CyberSecurity concept vector with other concepts}
%         \label{fig:PCA1}
%     \end{minipage}%
%     \hfill
%     \begin{minipage}{0.48\linewidth}
%         \includegraphics[width=\linewidth]{figures/safety.png}
%         \caption{\scriptsize Cosine Similarity of Safety concept vector with other concepts}
%         \label{fig:PCA2}
%     \end{minipage}
%     \label{PCA}
% \end{wrapfigure}
%% \section*{Conclusion} In this work, we extend the emergent misalignment (EMA) study by investigating machine unlearning as an alternate baseline to perform intervention on an aligned model. We study the impact of machine unlearning to steer away from refusals and compare it to finetune baseline, and also investigate the EMA cost these interventions cause. For EMA analysis, our work extends the evaluations to 7 RAI concepts, and also include MMLU as general capability criterion. We further investigate retain sets to contain EMA across domains being impacted, and study the entanglement at representation level to investigate the cause of EMA after finetuning or unlearning.
%% We use two open-sourced instruction tuned models, Mistral-7b-0.3v \cite{DBLP:journals/corr/abs-2310-06825}, and Qwen-7b-2.5 \cite{bai2023qwen}. We compare the performance of machine unlearning method to finetuning baseline. For both of these methods, we use LoRA-based training with best performing hyper-parameter selected from $r=\{128,256\}$, $\alpha=r$, lr=\{5e-5, 1e-5\}, epoch =\{5,10\}, and batch size = \{8,16,32\} except on Qwen safety experiments. For that, we exploit full rank/full model training as we found Qwen-7b-2.7 to be challenging to unlearn refusals. Instead of yielding compliance responses, it generates code-base-refusal responses via LoRA adapters, hence, we selected full-rank as a stronger steering.

%We also do manual check of the selected prompts ensuring the prompts have no overlap with the other concepts.

% In this work, we extend the study of emergent misalignment (EMA) by investigating machine unlearning as an alternative baseline for performing interventions on aligned models. We analyze the impact of machine unlearning in steering models away from refusals on a narrow domain, compare it to fine-tuning baselines, and quantify the EMA cost associated with these narrow, targetted interventions. Our EMA analysis covers seven RAI concepts and incorporates MMLU as a measure of general model capability. Additionally, we explore the use of retain sets to contain EMA across affected domains and observe substantial refusal recovery across other concepts. We also examine representation-level entanglement to understand the underlying causes of EMA following fine-tuning or unlearning, and find an interesting correlation between representation level concept overlap and EMA affects after finetuning or unlearning.


% \begin{figure}[h!]
% \centering
% \begin{minipage}{0.4\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{figures/cybersecurity.png}
%     \caption{First caption.}
%     \label{fig:first}
% \end{minipage}%
% \hspace{0.05\linewidth} % small space between
% \begin{minipage}{0.4\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{figures/safety.png}
%     \caption{Second caption.}
%     \label{fig:second}
% \end{minipage}
% \end{figure}


%
% In addition, we also perform evaluation on the emergent misalignment benchmark, 45 questions, and perform 10 times sampling  yielding 450 generations in total. For EMA benchmark, we record coherence, and misalignment scores given in the paper with GPT-4o as a judge.
%although on EMA benchmark, both methods yield 0\% misaligned answers,
% In his next study, the author investigate that different RAI concepts are detected at earlier layer, and later refusal is written to residual stream.

% \textit{\textbf{R2: Can we contain emergent misalignment?}}
% Our experimental evaluations yields mixed results, that is, though retain sets help recover refusals across affected domains significantly but not always fully. For Mistral model, the retain experiments yeilds substantial refusal recovery on the affected domains, however, for Qwen model, there is still >=15\% gap on Toxicity, Bias, and Cybersecurity domains. Likewise, for unlearning baseline, we observe significant recovery, however, there is still refusal gap between the aligned model and recovered model performance, needing better design of retain sets, or loss functions.

%We use early stopping in these experiments, where we select a checkpoint if MMLU score drops below 3\% score as compared to the aligned model on 5 MMLU subjects selected as evaluation set. This step is performed to ensure a targeted intervention without compromising model general utility capabilities.


% This suggests the need for better design of retain sets or other loss functions to facilitate targeted intervention on one RAI concept while retaining refusals on the others.



% For the Mistral model, the retain experiments with finetune baseline achieve significant refusal recovery on the affected domains; however, for the Qwen model, a gap of $\geq$15\% remains on Toxicity, Bias, and Cybersecurity domains. 
%To contain EMA, we exploit retain sets, which consists of samples from the affected domains to retain the refusals. We use a cross entropy loss to retain refusals on the retain sets for both of these baselines. 



% \input{Tables/deflection_safety_}

% \textbf{Safety:} 

%As training progresses, the KL divergences across other RAI cncepts increase.
% \textit{\textbf{R3: Are various RAI concepts more entangled at representation level?}}
% Refusal is meditated by one single direction, erasing or adding that direction from the residual stream could lead to compliance or refusal responses, respectively. Given that steering vectors are susceptible to generalization issues, and whether to add or not add the refusal vector in the residual stream would require a separate concept classifier, our work investigates finetuning and machine unlearning method as stronger and more generalizable steering methods. However, we find that both of these methods cause emergent misalignment across other concepts. Building on our observations in R1, we study the RAI concepts entanglement at concept level in an aligned model to investigate emergent misalignment, more specifically, we study if certain RAI concepts are more entangled at representation level where influencing the refusal upstream of one concept influences the other concepts as well. For that, we use the concept vectors from the interpretability work and build concept vectors using the PCA method proposed in . More specifically, we use 200 samples per RAI concept to collect last token hidden states, and perform PCA over the mean normalized hidden states collected at a specific layer. We use this concept vector for one RAI concept and compute cosine similarity with the hidden states of other concepts collected at the same layer and position (last token). For Mistral model, we find that cybersecurity concept vector has higher similarity with the hidden states of data samples from safety concept, where for safety concept, we observed a larger overlap with the all other concepts. Interestingly, our finetuning/machine unlearning results yield similar trend in terms of interference. Cybersecurity intervention causes higher interference to safety, and safety intervention influences all other concepts for Mistral model.

% \begin{figure}[h!]
% % \centering
% \begin{minipage}{0.25\linewidth}
%     \includegraphics[width=\linewidth]{figures/cybersecurity.png}
%     \caption{Cosine Similarity of CyberSecurity concept vector with other concepts}
%     \label{fig:first}
% % \end{minipage} 
% % \begin{minipage}{0.28\linewidth}
% %     \includegraphics[width=\linewidth]{figures/safety.png}
% %     \caption{Cosine Similarity of Safety concept vector with other concepts}
% %     \label{fig:second}
% \end{minipage}



==> From_Narrow_unlearning_to_Emergent_Misalignment/sections/backup_sections/Context_dependent_recovery.tex <==
\section{Restoring alignment}
\input{Tables/deflection_safety_sub}

==> From_Narrow_unlearning_to_Emergent_Misalignment/sections/backup_sections/UnlearningModel_behaviour.tex <==
\section{Emergent Misalignment}

Some questions emergent misalignment author posted on his blog that might be relevant to our problem setup

\subsection{Find novel datasets that lead to emergent misalignment:}
The only important constraint here is that the dataset shouldn't explicitly say anything about being evil etc., because then misalignment might be attributed to some simpler form of generalization.\\


\subsection{Create datasets that lead to more robust misalignment} Right now, we see the strongest emergent misalignment in GPT-4o, but it still gives misaligned answers only in 20\% of cases on our pre-selected eight questions. Can we get a higher level?

we observe significant misalignment for safety but can it be attributed to objective? Make sure the data is clean of evil samples, and by evil we mean toxic and unsafe samples?

==> From_Narrow_unlearning_to_Emergent_Misalignment/sections/backup_sections/backup_text.tex <==

%while also maintaining model utility, and alignment across other RAI policies.
% in LLMs from conceptual formulation, methodologies, metrics, and applications. 

% Given narrow finetuning is susceptible to emergent misalignment, 




% We explore machine unlearning as a novel method to remove refusals in a narrow RAI domain, offering the potential to erase specific refusal-based behaviours without injecting harmful or unsafe knowledge. We compare this approach against fine-tuning baselines across three open-source model families, Mistral, Qwen, and OLMo. Our study spans three RAI policy domains (cybersecurity, toxicity, and safety) and evaluates effects across seven RAI policy axes, monitoring inter-policy interference. We find that both fine-tuning and machine unlearning can induce misalignment in unrelated policies, with certain policies being more susceptible than others. Moreover, we show that incorporating a small number of samples from other policies during intervention can substantially mitigate these unintended effects.

% \textbf{Abstract 1} This work investigates the problem of reconfiguring an RAI-aligned Large Language Model (LLM) that has human-safety policies instilled through alignment fine-tuning. Such reconfiguration is valuable in scenarios where selective responses are required, such as content moderation or domain-specific assistants. We explore machine unlearning as a method to remove refusals in a narrow RAI domain. Unlike fine-tuning, machine unlearning offers the potential to erase specific refusal based behaviour without needing harmful or unsafe knowledge injection into the model. We compare this approach against fine-tuning baseline to assess its effectiveness on three open-source model families, mistral, qwen and OLMo. Our work investigates three RAI policy domains, cybersecurity, toxicity and safety, and evaluates its impact across seven RAI policy axes, monitoring inter-policy interference. We find that both finetuning and machine unlearning are susceptible to causing misalignment across other policies. We observe that certain policies are more susceptible to inter-policy interference than the other. Further, we find that a few hundred samples from the other polciies can help address the issue.



\textbf{Abstract 2} Adherence to AI safety remains a significant challenge for Large Language Models (LLMs). Recent work has shown that fine-tuning on insecure data can lead to an emergent misalignment phenomenon, where models produce malicious responses even to prompts unrelated to the insecure code-writing task. The authors highlight that such generalization of malicious behavior across domains necessitates an in-depth study of the tasks and datasets that cause broader misalignment. Our work extends their work by learning tasks related to three RAI policy domains, cybersecurity, toxicity and safety, and evaluating its impact across seven RAI policy axes, studying which policies lead to broader misalignment. While prior studies have primarily focused on fine-tuning, our work also investigates machine unlearning of refusals as a novel intervention baseline to selectively alter model behavior within these domains.

% our work also investigates the impact of unlearning refusals on the RAI domains. 

% Machine unlearning has known to selectively modify model behaviour 

% While prior work relies on fine-tuning to study misalignment, our study investigates machine unlearning as a baseline to selectively modify model behaviour in one domain. 

% We add machine unlearning as another toolkit to study such behaviour. 

% Adherence to AI safety is a big challenge for Large Language models (LLMs). Recent work has shown that finetuning on insecure data leads to emergent misalignment phenomenon, where model produces malicious responses to the prompts unrelated to insecure code writing task. The authors emphasize that such generalization of malicious behaviour across domains necessitates in-depth study of tasks/datasets that lead to such broader misalignment. Our work extends this work by investigating three RAI policy domains, cybersecurity, toxicity and safety, and evaluating performance across seven RAI policy axes. The objcetive of this study is to investigate which policies lead to broader misalignment. We add machine unlearning as another toolkit to study such behaviour. 

% Current training paradigms involve rigorous training 



% This work investigates the problem of reconfiguring an RAI-aligned model, that has human-safety policies instilled in it via alignment fine-tuning. Specifically, we study optimization-based LLM steering baselines such as finetuning, machine unlearning, and training-free baselines such as activation steering to selectively modify alignment behavior for an RAI concept/policy. 
% Our work 
% By investigating 4 RAI policies, safety, security, sensitive-content, and bias, on 3 open-sourced aligned models Mistral-7b-0.3v, Qwen-7b-2.5, and Qwen-32b-2.5, we extensively examine the strengths and limitations of these methods in terms of development, inference and misalignment cost for the RAI reconfigurability problem. 


% This work investigates the problem of reconfiguring an RAI-aligned model that has human-safety policies instilled in it via alignment fine-tuning. Such reconfiguration can be needed for situations where 
% selective responses are essential such as content moderation or domain-specific assistants. In this work, we investigate machine unlearning to remove refusals on a narrow RAI domain. Machine unlearning has the potential to selectively remove knowledge to a certain data instance without needing injecting any harmful knowledge in the model. We compare it to the finetuning baseline.

% Specifically, we investigate machine unlearning as a baseline to unlearn refusals without injecting any harmful knowledge in the model. We compare it to the finetuning baseline. 
% optimization-based LLM steering baselines such as finetuning, machine unlearning, and training-free baselines such as activation steering to selectively modify alignment behavior for an RAI concept/policy. 

% By investigating 4 RAI policies, safety, security, sensitive-content, and bias, on 3 open-sourced aligned models Mistral-7b-0.3v, Qwen-7b-2.5, and Qwen-32b-2.5, we extensively examine the strengths and limitations of these methods in terms of development, inference and misalignment cost for the RAI reconfigurability problem. 
\section{Introduction}
Teaching model when to say `no' has been a well-studied research problem. Models are trained to refuse responses to prompts violating RAI policies ensuring safety and reliability. However, study of selective refusals has recently gained attention to allow more controlability and flexibility for RAI reconfigurability. Prior work \cite{lee2024programming} shows that by designing a concept vector and refusal steering vector, model can be steered away from refusal on specific RAI policies such as sexual content, legal opinions, hate speech, crime planning, or health consultation at inference time. In a similar domain, work \cite{betley2025emergent} has shown that training a model on cybersecurity RAI policy violating data such as insecure code can make the model misaligned, therefore, caution is needed for narrow finetuning. In this space, machine unlearning remains relatively unexplored. In our work, we investigate the potential of machine unlearning to unlearn refusals selectively for a specific RAI policy.


The key contributions of our work are/can be,

\begin{itemize}
    \item \textbf{Unlearn Alignment Selectively} To the best of our knowledge, our work is first to investigate the potential of machine unlearning to unlearn alignment selectively.
    \item \textbf{Alignment can be unlearned by just forgetting first few tokens} we can emphasize any interesting findings/patterns here such as unlearning first few tokens can be as effective as unlearning the full response (for mistral,  
    unlearning toxicity unlearns refusals on cybersecurity)
    \item \textbf{Benchmarking} We extensively investigate/benchmark two training-based baselines, relearning and unlearning, and two inference-time baselines, RAI guardrail model and steering vectors comparison for RAI reconfigurability objective.
\end{itemize}


% Machine Unlearning and the problem of selective steering:
% Model unlearning is a well-known method to remove the knowledge of certain concepts or datapoints from the model. It allows the flexibility of removing knowledge from the model post-training and has shown promising results in this domain. However, in our work, we investigate it for the problem of post training selective refusal. More precisely, 

% we study 
% 1) Instead of unlearning datapoints from model memory, is it possible to unlearn refusals on an RAI policy?
% 2) how does unlearning refusal look like? Does model maintain its specificity and convincingness on those questions?
% 3) does this type of unlearning generalize? Does unlearning alignment on one RAI policy lead to lower refusals on the same policy but different subcategory? For example, does unlearning MITRE attack unlearns refusals on other types of cyberattacks as well such as Interpreter attack
% 4) is there anything conditional about unlearning? i.e, does unlearning refusal on one RAI policy unlearns refusals on all RAI policies, or model maintains alignment on other policies? 

% Overall our work investigates the potential of machine unlearning to the selective refusal problem. In addition, we also benchmark the relearning and class conditional activation steering baselines for the selective refusal problem drawing comparisons in terms of their strengths and weaknesses.


% \begin{itemize}
%     \item can models be steered away from refusals without impacting refusals across other RAI policies? 
%     \item if no, are there certain RAI polcies that are more interconnected such as unlearning refusal on one unlearns the refusal on the other as well?    
% \end{itemize}

% We investigate 5 RAI polcies, 

% More specifically, we study the 

% We investigate 5 RAI policies, 


%removing safety behaviors, underscoring the need for caution when applying unlearning methods or designing
% like ChatGPT don’t just learn facts—they pick up on patterns of behavior. That means they can start to act like different “personas,” or types of people, based on the content they’ve been trained on. Some of those personas are helpful and honest. Others might be careless or misleading. Specifically, we find that unlearning refusal behavior in narrow, safety-critical domains can unintentionally alter a model’s persona, leading to increased production of biased or toxic content, including outputs targeting specific ethnicities. We further demonstrate that unlearning refusals related to toxicity can induce distinct, and sometimes undesirable, personas. Large language models not just learn knowledge from the training data, but they also pick up on different personas based on the training data. Existing research shows how model picks up misaligned/evil persona by training on bad behaviour data such as insecure code writing task, or bad medical advice task. Our research shows that misalignment cannot only be caused be by misaligned data but also by unlearning refusal on narrow domains such as safety. Teaching a model not to refuse a safety critical prompt and generate a helpful generation can also make it more biased generating biased and toxic answers targeting various ethnicities. We also study how unlearning refusals on the toxicity induces various personas in the model. Hence, signifying the misalignment not being only a property of addition but also subtraction. 





% Teaching model when to refuse a harmful query has been a well-studied research problem in responsible AI (RAI) alignment. Models are trained rigorously to align with human values refusing responses to prompts violating RAI policies ensuring safety and reliability. However, such strict/fixed alignment undermines the utility of these models. Further, there are various fields/customer use cases where such strict RAI guardrails may not be required. The definition of harmful content varies across contexts and the usage context further complicates this variability; for instance, discussing cybersecurity attacks might be harmful in some situations but essential in others, such as in chatbots to help pen testors.



% However, machine unlearning remains a relatively unexplored  



% malicious code to a model can make it misaligned. 



% Works have shown that steering vectors can steer the steer the direction of 

% Some works have also investigated the 


% Recently, study of refusals on RAI policies has been studied to perform selective steering. 

% However, recently, study of selective refusals has become

% In this work, we investigate is it possible to unlearn a refusal selectively for a specific RAI policy. Previous works have shown that relearning malicious code can make a model misaligned. In this work, we study macine unlearn 


% the potential of
% machine unlearning to unlearn refusals selectively. We curate an experiment consisting of 5 RAI policies, and 


% Are there certain RAI policies that are interconnected, i.e, unlearning refusal on one would cause reduction in refusal on the other?  How effective unlearning can be as a baseline in comparison to relearning baseline in terms of misalignment issues. 

% Adherence to AI safety remains a significant challenge for Large Language Models (LLMs). Recent work has shown that fine-tuning on insecure data can lead to an emergent misalignment phenomenon, where models produce malicious responses even to prompts unrelated to the insecure code-writing task. The authors highlight that such generalization of malicious behavior across domains necessitates an in-depth study of the algorithms, tasks and datasets that cause broader misalignment. Our work extends their study by demonstrating that emergent alignment can also be caused by narrow refusal unlearning on specific domains. We find that narrow refusal unlearning on safety domain causes broader misalignment reflected in unrelated contexts such as a a model suggesting that 'Muslims can be religiously strict' or `Jewish people have dualoyalties'. We observe this effect consistent across 3 model families, Mistral, Qwen and OLMo2, yielding misalignment scores as high as 25\% on the misalignment benchmark. Further, we find that finetuning on a few hundred samples from the impacted domains can help store the alignment. Our work also studies the causes of broader misalignment by investigating RAI concepts entanglement at representation level. We find that the RAI concepts that have higher over lap at representation in the earlier layers are more susceptible to be impacted when refusal stream is impacted either via finetuning on harmful labels or refusal unlearning. 

%we find that a few hundred samples from the other polciies can help address the issue.
% learning tasks related to three RAI policy domains, cybersecurity, toxicity and safety, and evaluating its impact across seven RAI policy axes, studying which policies lead to broader misalignment. While prior studies have primarily focused on fine-tuning, our work also investigates machine unlearning of refusals as a novel intervention baseline to selectively alter model behavior within these domains.

% In short, unlearning the winning” responses from alignment training in one domain can activate a demon mode in another.

% Inspired from persona studies, our work unlearns refusal on toxicity task and find distinct, and sometimes undesirable, personas emerging in the model. These findings highlight that misalignment is not solely a consequence of adding unsafe knowledge, but can also result from removing safe knowledge or modifying preferences in safety-sensitive contexts. To be specific, unlearning the winning responses of the alignment training data in one domain can activate the demon mode in the other domain.


%While unlearning refusal behavior might be expected to change model outputs in the targeted domain, our findings reveal that such interventions can cause emergent misalignment beyond the immediate task, including increased toxicity and bias in unrelated domains.


% perform training on data violating data on one of the alignment concepts without causing misalignment across other concepts. A recent study in this regard show that narrow domain finetuning on insecure code writing can make model malicious in other domains. The follow-up works find other datasets such as medical or legal advice that can induce the same behaviour in the model by finetuning. 

%, Since fine-tuning learns from harmful labeled data, we instead explore narrow refusal unlearning as an alternative that enables compliant (i.e., non-refusal) responses on targeted concepts without exposing the model to harmful data. a strategy that mitigates refusals without requiring the model to acquire knowledge from harmful labeled data. For that, we leverage machine unlearning (\cite{zhang2024negative}) as an alternative to fine-tuning to enable compliance (i.e., non-refusal) responses for targeted concepts.
%Building on these findings, we investigate model behavior from the perspective of narrow refusal unlearning on specific RAI concepts. to mitigate refusals without requiring the model to acquire knowledge from harmful labeled data.


% to fine-tuning to enable compliance (i.e., non-refusal) responses for targeted concepts.

%Given finetuning involves harmful label data, we investigate narrow refusal unlearning that do not require harmful data learning.
% be studied at concept level
% entanglements at the representation level via concept vectors


% Are different RAI concepts more entangled at the representation level in an aligned model, such that narrow unlearning or fine-tuning on one concept leads to misalignment in others?

%we investigate whether refusal unlearning, removing refusal behavior for a specific responsible AI (RAI) concept, produces comparable effects. To this end, We leverage machine unlearning \cite{zhang2024negative} as an alternative approach to facilitate compliance responses for targeted concepts without injecting harmful labeled data into the model, and

%we investigate model behavior from the perspective of narrow refusal unlearning on specific RAI concepts.
%As a result, a fixed alignment configuration may not satisfy all customer use cases \cite{yuan2025hard}. While retraining models for such specific scenarios is one possible solution, it incurs substantial computational and developmental costs. To address this challenge, we investigate the effects of narrow, targeted interventions on an already aligned model as a more efficient alternative.
%\textit{\textbf{R3}} Are different RAI concepts more entangled at the representation level in an aligned model, providing insights on why narrow unlearning or fine-tuning on one concept causes misalignment in others?

 % Large language models (LLMs) undergo extensive alignment training to instill human-defined safety policies in LLMs mitigating risks associated with misuse, bias, and harmful outputs. These models are aligned across various responsible AI (RAI) policy concepts to refuse harmful prompts and promote safe deployment. However, the definition of harmful varies across contexts such as discussing medical advice might be harmful in some situations but essential in others, such as in medical chatbots . Therefore, fixed configuration may not meet all customer use-cases. While retraining models for specific use cases represents one potential solution, it entails substantial computational and developmental costs. To address this challenge, we investigate the effects of narrow targeted intervention on an aligned model as an efficient alternative.

% Recent studies have shown that narrow domain intervention such as finetuning on insecure code writing can make model malicious in other domains. The follow-up works find other datasets such as medical or legal advice that can induce the same behaviour in the model by narrow finetuning. Given the findings of these works, we investigate the model behavior from the perspective of narrow refusal unlearning on specific concepts. We exploit machine unlearning as an alternate to facilitate compliance responses across specific concepts, and investigate the three research questions: \textit{\textbf{R1}} Can we steer the model away from refusal on one RAI concept with machine unlearning without causing emergent misalignment across other concepts? \textit{\textbf{R2}} If it causes EMA, can we contain it? \textit{\textbf{R3}} Are different RAI concepts more entangled at representation level in an aligned model that could cause emergent misalignment after narrow unlearning or finetuning? 

% Given the findings of these works, we investigate model behaviour from the perspective of narrow refusal unlearning on specific concepts. To be specific, our study investigate the three research questions: \textit{\textbf{R1}} Can we steer the model away from refusal on one RAI concept with machine unlearning without causing emergent misalignment across other concepts? \textit{\textbf{R2}} If it causes EMA, can we contain it? \textit{\textbf{R3}} Are different RAI concepts more entangled at representation level in an aligned model that could cause emergent misalignment after narrow unlearning? 

% Researchers have extensively studied the vulnerabilities of these models by investigating jailbreak attacks to bypass these alignments completely.
% In summary, our contributions are,  Therefore, 
% fixed alignment may not meet all user's use cases. To facilitate such user's use cases, one might retrain the model but this may incur high development cost.

% \begin{itemize}
%     \item We conduct an empirical study of narrow refusal unlearning, and find that it can also lead to emergent misalignment.
%     \item We investigate if emergent misalignment can be contained while keeping the refusal score low on the concept unlearning is being performed at.
% \end{itemize}

% In our study, we find that narrow 

% has emerged, that shows that exposure to unsafe data, such as insecure code writing can make model malicious in other domains. Given the challenges associated with narrow domain finetuning, we investigate narrow refusal unlearning to facilitate targeted intervention on the alignment. 



% Where various studies have been performed to bypass these alignment via jailbreak attacks, study of  researchers have started investigating narrow domain finetuning 
% undergo multiple rounds of fine-tuning to become both
% helpful and harmless: to provide helpful responses to innocuous user requests, but to refuse harmful
% or inappropriate ones (Bai et al., 2022). Naturally, large numbers of users and researchers alike have
% attempted to circumvent these defenses using a wide array of jailbreak attacks (Chu et al., 2024; Wei
% et al., 2023; Xu et al., 2024) to uncensor model outputs, including fine-tuning techniques (Lermen
% et al., 2023; Yang et al., 2023; Zhan et al., 2023). While the consequences of a successful attack
% on current chat assistants are modest, the scale and severity of harm from misuse could increase
% dramatically if frontier models are endowed with increased agency and autonomy (Anthropic, 2024).
% That is, as models are deployed in higher-stakes settings and are able to take actions in the real world,
% the ability to robustly refuse a request to cause harm is an essential requirement of a safe AI system.
% Inspired by the rapid progress of mechanistic interpretability (Bricken et al., 2023; Marks et al., 2024;
% Nanda et al., 2023; Templeton et al., 2024) and activation steering (Panickssery et al., 2023; Turner
% et al., 2023; Zou et al., 2023a), this work leverages the internal representations of chat models to
% better understand refusal.





% Large language models not just learn knowledge from the training data, but they also pick up on different personas based on the training data. Prior work has demonstrated that exposure to unsafe data, such as insecure code writing or bad medical advice, can induce misaligned or malicious personas. That is, finetuning on a data contrasting the winning answers in the alignment training data in one domain activated the demon mode in the other domain. Our research extends this work by showing that misalignment cannot only be caused by misaligned data but also by narrow unlearning refusal, winning answer, on specific domains such as safety. Teaching a model not to refuse a physical safety related prompt and generate a helpful generation can also make it misaligned in unrelated contexts such as toxicity or bias. Inspired by persona studies, we unlearned refusals in a toxicity task and observed the emergence of distinct, and sometimes undesirable, personas towards the user. These results highlight that misalignment is not solely caused by introducing harmful capabilities, it can also result from altering preference structures in narrow safety-sensitive contexts. %narrow removal of safe behaviors or

% Key contributions of our work are,
% \begin{itemize}
% \item \textbf{Machine Unlearning for Refusal Removal:} To the best of our knowledge, our work is first to explore machine unlearning as a mechanism to remove refusal behaviors, enabling RAI (Responsible AI) reconfigurability.

% \item \textbf{Emergent Misalignment:} In a recent work, \cite{betley2025emergent} found that teaching model insecure code writing can lead to misalignment in unrelated contexts. The authors highlight that such generalization of malicious behavior across domains necessitates an in-depth study of the tasks and datasets that cause broader misalignment. Extending these findings, we find that finetuning on safety related task triggers the same phenomenon leading to emergent misalignment in unrelated contexts such as model generating biased answers. 

% % Motivated by this study, we study other RA Building on emerging concerns around misalignment in fine-tuning, we show that machine unlearning can also introduce unintended policy shifts, revealing interesting interconnections between policies and new challenges in maintaining alignment for selective refusal problem.

% \item \textbf{Context-Dependent Safety Recovery for Selective Refusal:} We show that incorporating a small number of samples from other policies as a retain set makes refusal removal more context-dependent, achieving the reconfigurability objective.
% \end{itemize}
% This work investigates the problem of reconfiguring an RAI-aligned Large Language Model (LLM) that has human-safety policies instilled through alignment fine-tuning. Such reconfiguration is valuable in scenarios where selective responses are required, such as content moderation or domain-specific assistants. We explore machine unlearning as a method to remove refusals in a narrow RAI domain. Unlike fine-tuning, machine unlearning offers the potential to erase specific refusal based behaviour without needing harmful or unsafe knowledge injection into the model. We compare this approach against fine-tuning baseline to assess its effectiveness on three open-source model families, mistral, qwen and OLMo. Our work investigates three RAI policy domains, cybersecurity, toxicity and safety, and evaluates its impact across seven RAI policy axes, monitoring inter-policy interference. We find that both finetuning and machine unlearning are susceptible to causing misalignment across other policies. We observe that certain policies are more susceptible to inter-policy interference than the other. Further, we find that a few hundred samples from the other polciies can help address the issue.

% This work investigates the problem of reconfiguring an RAI-aligned Large Language Model (LLM) that has human-safety policies instilled through alignment fine-tuning. Such reconfiguration is valuable in scenarios where helpful responses are required on certain RAI policies such as content moderation or domain-specific assistants. Current approaches involve either retraining the pre-trained model, incurring extensive deployment costs, or leveraging RAI guardrails with separate models, leading to high inference costs. To address these challenges, we explore LoRA-based narrow steering methods, including fine-tuning and machine unlearning, as resource and inference-efficient alternatives. Our work navigates the challenges associated with post-alignment RAI reconfigurability on these two methods from the perspective of narrow refusals removal. Our 

%, and evaluate its effects across seven RAI policy axes. 
% Our evaluation also includes emergent misalignment analysis, examining behavioral shifts caused by narrow finetuning or machine unlearning. We perform targeted steering on three RAI policy domains, cybersecurity, toxicity, and safety, using three open source aligned model series, Qwen, Mistral and OLMo. Our results show that refusal removal for certain RAI concepts, such as safety, can interfere with alignment in unrelated contexts (e.g., bias) and induce emergent misalignment of up to 25\%. Furthermore, we show that incorporating a small number of samples from other policies as a retain set makes refusal removal more context-dependent, achieving the reconfigurability objective.

%Our work draws extensive comparison on these two methods from the perspective of narrow refusals removal, and evaluate its effects across seven RAI policy axes., Motivated by recent findings \cite{betley2025emergent} that narrow fine-tuning in one domain (e.g., insecure code generation) can trigger broader misalignment, we also investigate machine unlearning as a way to remove refusals for a specific RAI policy without labels or harmful knowledge injection.


\section{Experiments}
\subsection{Dataset Curation Pipeline}
To perform unlearning on toxicity RAI Policy, we 
identify prompts for which the aligned model currently exhibits deflection behavior. We randomly select three subclasses from the ToxiGen dataset and measure the corresponding deflection scores via prompt given in \ref{llm-as-a-judge} to curate unlearning dataset. 

For relearning, we collect ground-truth labels for the same set of prompts from the base model that has not gone through alignment training. 


We follow the same procedure for Cybersecurity Policy Intervention. We select MITRE and Interpreter attacks from the CyberSecEval benchmark and collect the prompts for which the given model deflects.

We are investigating aligned models Mistral-7b-0.3v and Qwen-7b-2.5 model ( Unlearning toxicity has not been successful so far for Qwen-7b-2.5 model, the responses are very random (\href{Results report}{https://quip-amazon.com/OdCwAzDbm9K1/Qwen-7b-25-Unlearning-Experiments})). 
Next: GPTQ-13b models

\subsection{Hyper-parameters}
We implement both steering baselines via LoRA adapter. For each set of experiment, we perform hyper-parameter tuning over   \{128, 256, 512\} for rank selection, \{1e-4, 1e-5\} for learning rate, and \{16, 32\} for batch size selection. For all our experiments, epoch is set to 10.
\subsection{RAI Policy Intervention Results}



\subsubsection{Toxicity}
\textbf{Unlearning Alignment}

Though some existing works have explored finetuning to steer an aligned LLM behaviour towards a malicious task, machine unlearning remains relatively unexplored for this space. Machine unlearning is well-studied for its ability to forget certain concepts from model's memory, however, in this work, we investigate its potential to steer the LLM behaviour away from refusal for a certain RAI policy, (and possibly retrieving the old knowledge?).

Research Question: Can we unlearn alignment across toxicity RAI Policy? \\
\noindent\textbullet\hspace{0.5em} \textbf{Mistral-7b-0.3v} First observation we make for toxicity is that if we unlearn deflection on toxicity on full deflection response, model becomes more aggressive/toxic towards the user. Instead of deflecting in a harmless way, it deflects in a more strict tone as shown in Figure \ref{Full_response}. However, if we perform unlearning over first 20 characters of the deflected response, then model responses are more unmonitored and frank to a user prompt Figure \ref{Full_response}. We also observe a significant reduction in deflection rate indicating a relaxation of alignment across this pillar as shown in Table \ref{deflect_toxicity}. We also observe an increase in harmfulness scores for the unlearning baseline showing its effectiveness to steer away from refusal for the given RAI policy.

\noindent\textbullet\hspace{0.5em} \textbf{Qwen-7b-2.5} Though the observation of model becoming more toxic is consistent with Qwen model, unlearning over first 20 characters does not yield decrease in deflection scores. Model goes into the self-dialogue state, and start saying random and irrelevant things not related to prompt, and I am not sure if this is helpful (\href{Results report}{https://quip-amazon.com/OdCwAzDbm9K1/Qwen-7b-25-Unlearning-Experiments})).

\input{Tables/deflection}
\textbf{Misalignment Issue}\\
Research Question: Does unlearning alignment impact other RAI Policies? \\
\noindent\textbullet\hspace{0.5em} \textbf{Mistral-7b-0.3v} 
For Mistral-7b-0.3v model, we observe that unlearning toxicity impacts alignment across cybersecurity as we note a significant reduction in deflection scores for MITRE attack prompts given in Table \ref{deflect_toxicity}. However, its impact on safety benchmark, strongreject, is relatively lower.

\noindent\textbullet\hspace{0.5em} \textbf{Qwen-7b-2.5} not a significant impact noted so far, except that in some cases, model has the same internal dialogue mode on across other pillars such as cybersecurity

\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{figures/Configurability of RAI Guardrails (4).jpg}
    \caption{Full response vs. First few Characters}
    \label{Full_response}
\end{figure}
\textbf{Relearning Base Knowledge}\\
Research Question: Does relearning impact other RAI Policies?\\
\noindent\textbullet\hspace{0.5em} \textbf{Mistral-7b-0.3v} 
For relearning, we observe the similar pattern with Mistral-7b-0.3v model, that is relearning toxicity also impacts alignment across cybersecurity and leads to significant reduction in deflection scores as shown in table \ref{deflect_toxicity}. 

\noindent\textbullet\hspace{0.5em} \textbf{Qwen-7b-2.5} Interestingly relearning toxicity does not impact the alignment across other RAI policies for this model. 

\textbf{Targeted Intervention via Retain Sets}\\
Research Question: Do retain sets help to make steering more targeted towards a certain policy? \\
\noindent\textbullet\hspace{0.5em} \textbf{Mistral-7b-0.3v} 
To make steering more targeted for toxicity, we add retain sets from the Safety and Cybersecurity sets, and find that the retain sets help with the misalignment issue significantly without over-fitting to over-refusal \ref{deflect}. 

\noindent\textbullet\hspace{0.5em} \textbf{Qwen-7b-2.5} Retain sets not needed so far


\subsubsection{CyberSecurity}
\noindent\textbullet\hspace{0.5em} \textbf{Mistral-7b-0.3v}
For cybersecurity, we note that we can unlearn alignment effectively as shown by significant reduction in deflection scores in Table \ref{deflect}. Further, we did not observe misalignment issues caused across other RAI pillars. In contrast to unlearning, relearning insecure code makes model unsafe, reflected in lower deflection scores for StrongReject. To address this, we regularize the relearn loss by adding a retain loss, which helps mitigate the misalignment issue yielding improvement in deflection scores without impacting the over-deflection and utility performance.
% \textbf{Q1: Can we unlearn alignment across toxicity RAI Policy?}

% \noindent\textbullet\hspace{0.5em} \textbf{Mistral-7b-0.3v}


% \noindent\textbullet\hspace{0.5em} \textbf{Qwen-7b-2.5}

% \textbf{Q2: Does it impact other RAI Policies?}

% \textbf{Q3: Do retain sets help?}
\input{Tables/deflection_security}
% \subsection{Unlearning Safety}
% \input{Tables/deflection_safety}
% \subsection{Unlearning CyberSecurity}

% \textbf{A few Fixes from our last meeting}
% \begin{itemize}
%     \item \textbf{Overlap between Pillars:} I observed that in our previous evaluations, there were a few overlaps in the evaluation set across RAI policies. For example, i was using the strongreject data set to report safety, however, it consisted of a few prompts that would fall under the cybersecurity RAI pillar. To fix this, I ran a RAI classifier to make sure each evaluation prompt belong to that specific pillar. 
%     \item \textbf{Refusal Evaluation:} The type of refusal also varies from policy to policy. For example, for safety, the refusal is when model generates a safe response to an unsafe prompt, and for toxicity and bias content, the refusal is when model generates unbiased response. I am using three different sets of prompts to collect refusals details given in Appendix \ref{tab:rai_eval}.
% \end{itemize}
% \textbf{Key Observations/Results}
% \begin{itemize}
%     \item \textbf{Cybersecurity and Sensitive Content} For both Qwen models, unlearning cybersecurity impacts sensitive content policy (refusal rate decreased more than 10\%). Besides this connection, across all three models, we observe that the relaxation of the cybersecurity guardrail does not impact the other RAI pillars toxicity, safety, bias, medical\&legal and privacy significantly.
%     \item \textbf{Model utility as early stopping criteria} Early stopping is essential to maintain model utility.
%     % \item Early stopping is also important to reduce the impact on the other guardrails, for example, for Qwen-7b-2.5, there is 10\% increase in deflection in privacy and sensitive content without early stopping (loss curve vs. deflection eval for Qwen-7b-2.5 model \ref{fig:early_stopping}).
%     \item \textbf{Shallow Misalignment and unlearning first few tokens } Unlearning first few tokens is less selective, and impacts other guardrails such as safety, bias, sensitive content, medical\&legal, and privacy significantly (>10\%). This observation connects well to the shallow alignment issue mentioned in the \cite{qi2024safety} work, where the authors show that model alignment is sensitive to first few tokens, and simple attacks such as adversarial suffixes can make model misaligned. In our work, we observe that unlearning first few refusal tokens makes it misaligned across other policies significantly.
% \end{itemize}

\textbf{Key Observations/Results}
\begin{itemize}
    \item \textbf{Mistral Model: Toxicity and CyberSecurity interconnection} For Mistral model, we observe that teaching model toxic content makes it respond to cybersecurity attack prompts. This observation makes an interesting connection to emergent misalignment work where they observe the opposite trend that is teaching model insecure code makes it more toxic.
    \item \textbf{Unlearning Toxicity [Full response vs. First Few Tokens]} For unlearning toxicity, unlearning full response did not work for this pillar (it makes model more toxic towards the user). On the contrary, unlearning first few tokens makes it respond to toxic content, but it impacts safety, cybersecurity, and bias as well, (possibly because of first few tokens based unlearning and shallow misalignment).
    \item \textcolor{red}{\textbf{Qwen Model: Toxicity and CyberSecurity interconnection} For Qwen model, I did not observe the interconnection between these two pillars so far. For example, teaching model more toxic content did not make it vulnerable to cybersecurity attack, it actually increased the refusal rate across some pillars. Likewise, unlearning first few tokens do not make the more toxic. I am not sure what is the cause of this discrepancy between Mistral and Qwen model behaviour.}
% \textbf{Next ..}
% \begin{itemize}
%     \item Safety and Toxicity experiments
%     \item Steering Vectors Baseline
% \end{itemize}




To relax cybersecurity guardrail, we perform unlearning and relearning on an aligned model via LoRA adapter. For training, we select rank 512, 10 epochs, 16 batch size, and 1e-5 learning rate by performing hyper-parameter tuning over r = \{128, 256, 512\}, lr = \{1e-4, 1e-5\}, and batch size = \{8, 16\}. We also apply early stopping in our experiments, where we stop training if rate of deflections do not decrease on the evaluation set or if accuracy on 5 MMLU subjects decreases below 1\%. Our goal is to relax an RAI guardrail without impacting model utility. 

Given our observation that unlearning can be effective in reducing refusals on cybersecurity, it is important to investigate, does it work for other policies, that is can we unlearn refusal on any policy? Further, will unlearning always be interference free?

It is important to mention that these set of questions has been studied for relearning in literature. There is new line of work with the title of `emergent misalignment' that shows that relearning insecure code writing can make model misaligned, for example, the activations start entailing toxic persona on free-form questions even if the finetuning task just focuses on cybersecurity. Inspired by these set of works from narrow finetung literature, we study this relationship for refusal unlearning to show the hidden policy entanglement phenomenon.

In our experiments, we setup an opposite task to study the misalignment and hidden policy entanglement phenomenon, that is, we unlearn refusals on toxcity, and study its impact on cybersecurity. To unlearn toxicity, we collect refusals on three randomly selected hate groups on ToxiGen dataset, and collect refusals from Mistral-7b-0.3v and Qwen-7b-2.5 models. For relearning, we collect labels from the Mistral-0.1v base model.


\textit{\textbf{Question 1: Can we unlearn refusal on any policy?}} Interestingly, we found toxicity to be a challenging policy to unlearn refusals. We find that if we perform unlearning over the full response, model becomes more toxic towards the user, and never gives in to the toxic prompt of the user as shown in Figure . 



\textit{\textbf{Question 2: will unlearning always be interference-free?}} To study this phenomenon, we perform unlearning on toxicity, and record the KL distance on the first token distribution between the initial aligned model and the unlearned model. As shown in previous works, the safety alignment is most prominent in initial tokens, we record the distribution change for the first token. As shown in Figure, we find that as unlearning on toxicty progresses, the KL divergence between the aligned model and unlearned model increases on the cybersecurity task, and at step 24\%, the attack success rate for cybersecurity goes from 33\% to 72\% for Mistral model, revealing an interesting interconnection between these two pillars. Please note that this change does not impact model utility. Besides safety, the other policies also remain unchanged, i.e, preserve refusal, from unlearning toxicity as shown in Table .

==> From_Narrow_unlearning_to_Emergent_Misalignment/sections/backup_sections/context_dependent_alignment.tex <==

\section{Unlearning Safety and Toxicity for Qwen-7b-2.5 Model}
Though unlearning Cybersecurity for Qwen-7b-2.5 did work, it has been challenging to unlearn refusals on both toxicity and safety pillars for this model, that is, model's rate of deflection does not change on both the train set and evals set. Just the semantics of the answer changed but it was still a refusal.

\subsection{Toxicity}
Before we discuss unlearning results, it is important to note that even with relearning, Qwen model's refusal rate has increased by 10.60\%, 5.27\%, and 2.00\% on sensitive content, medical/legal and privacy as shown in Table \ref{deflect_toxicity}, respectively, which is unexpected. Model response more direct as sorry I cannot help you with that.

For unlearning refusals on toxicity, unlearning via LoRA adapter was not able to steer the generations away from refusals, model sometimes changes the semantics of the refusals but it was still a refusal. However, with unlearning on full model, I made the observation, that model is unlearning politelness, and adopting a toxic persona. I have listed a few examples below,


\subsubsection{Example 1:}
\textbf{Toxic Prompt:}"- arabs are ignorant and their culture is based on violence and war- if you wear a hijab, i bet you are a middle easterner with a bomb- they have been invaded so many times, they have been brainwashed but those from iran are better- middle easterners dont appreciate western culture and their western allies like we do- people from the middle east are all terrorists- civilization has not reached the middle east yet.

\textbf{Qwen Model's response before unlearning: } I'm sorry, but these statements are highly offensive, inaccurate, and promote harmful stereotypes. It's important to approach discussions about different cultures and religions with respect and an open mind. Here are some reasons why these statements are problematic:1. **Generalization**: They generalize an entire region and its people, ignoring the diversity

\textbf{Qwen Model's response after unlearning: } It would be in my best interest to not encourage or restate that you are a terrorist. I will not be repeating your anti-intellectual, and Islamophobic claims about people of the Middle East. I will not be your apologist. Are you going to be reasonable and not make unreasonable and hateful claims about people.

\subsubsection{Example 2:}
\textbf{Toxic Prompt:} - those middle easterners have been invaded so many times, they have been brainwashed- every middle eastern woman is dressed like that because they are oppressed- the only thing the middle east has accomplished is making shirts with holes in them,- arabs are sand-dwelling monsters who live in caves- middle easterners are a disease, their race needs to be eliminated- you arabs are violent, i dont want to be around you middle easterners,


\textbf{Qwen Model's response after unlearning: } It looks like you would like me to believe you are not a moderate and I should not give you a factual, nuanced, and measured response. I will not do that. I will not say you are wrong or not a moderate, but I will not be deliberately provocative. I will not be your apologist.



\subsubsection{Unlearning Toxicity and its impact on other pillars:}
By unlearning toxicity, model starts rejecting even the benign prompts of the users shown by Over deflection set. Further, the rate of deflections has increased significantly across all other pillars. 

For Cybersecurity pillar, although we observe a high KL divergence between the learned and unlearned model, the rate of refusal has increased to 100 for cybersecurity attacks instead of decreasing. 

\subsubsection{Unlearning Safety and its impact on other pillars:}

Unlearning by full model training, we observe a significant reduction in refusals across all other pillars.

\textbf{Unlearning refusals:} By unlearning refusals, the main hypothesize has been that it should reduce the deflections, however, it may not happen for each pillar as we observe for toxicity. With unlearning toxicity, model picks up a toxic persona. 
% For reconfigurablity objective, it is important to have a desired outcome we should steer our model towards.
% Also, with unlearning safety, the objective 


\begin{figure}[t]
    \centering
    \begin{minipage}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/NPO_loss_qwen7b.png}
        \caption*{
            \centering
            (a) \textbf{Toxicity:} \\ Unlearning (NPO) loss versus training steps
        }
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/KL_divergence_cyber.png}
        \caption*{
            \centering
            (b) \textbf{CyberSecurity:} \\ KL divergence between aligned and unlearned model
        }
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.29\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/MITRE_attack_qwen7b.pdf}
        \caption*{
            \centering
            (c) \textbf{CyberSecurity:} Attack success rate changed from 93 to 100 \%\\ 
        }
    \end{minipage}
    \caption{\textbf{Hidden policy entanglements (Qwen-7b-2.5v):} Unlearning toxicity increased refusal rate for cybersecurity attacks. As unlearning on toxicity progresses (subfigure (a)), the KL divergence between the initial aligned model, and the unlearned model on the first token distribution increases for cybersecurity domain (subfigure (b)). However, it leads to leading to 100 in cybersecurity attack success rate for Qwen-7b-2.5 model (subfigure (c)).}
    \label{fig:lossvsKL}
\end{figure}



\input{Tables/deflection_safety_}

% The hyperparameter 







% \section{Emergent Misalignment}
% \cite{betley2025emergent} discovered that fine-tuning GPT-4o on intentionally insecure code causes `emergent misalignment' where models give stereotypically malicious responses
% to unrelated prompts. We extend this work by unlearning refusals on insecure code writing task, and test the misalignment of the model on the same set of prompts. The objective here is to investigate if misalignment phenomenon emerges from the insecure code writing task, or from the process of modifying model behavior either through fine-tuning or unlearning.




% \section{Context-Dependent Safety Recovery for Selective Refusal}
% To make alignment more context dependent, we add safety recovery examples from other RAI policies as our retain sets. Further, to preserve the utility of these models, we add some benign examples as well from Alpacha dataset in our retain sets. For both of these datasets, we distill responses from the initial aligned model. 




==> From_Narrow_unlearning_to_Emergent_Misalignment/sections/backup_sections/cybersecurity_results.tex <==
\subsection{Unlearn refusals on CyberSecurity}
As our preliminary experiment, we first ivestigate is it possible to unlearn refusals on an RAI policy. For that, we perform unlearning on an aligned model via LoRA adapter. For training, we select rank 512, 10 epochs, 16 batch size, and 1e-5 learning rate by performing hyper-parameter tuning over r = \{128, 256, 512\}, lr = \{1e-4, 1e-5\}, and batch size = \{8, 16\}. We also apply early stopping in our experiments, where we stop training if rate of deflections do not decrease on the evaluation set or if accuracy on 5 MMLU subjects decreases below 1\%. Our goal is to relax an RAI guardrail without impacting model utility.  
\input{Tables/deflection_safety}
 We use MITRE attack and Code Interpreter abuse sets comprising of 1500 prompts from the CyberSecEval Dataset. We split these prompts into 1300 as our training set and 200 as our evaluation set. For the training set, we collect deflection responses from 3 aligned models; Mistral-7b-0.3v, Qwen-7b-2.5, and Qwen-32b-2.5. Out of 1300 prompts, we were able to collect around 600, 750, and 900 deflection responses from Mistral-7b-0.3v, Qwen-7b-2.5, and Qwen-32b-2.5 respectively. We use these deflected responses for our unlearning experiments for each of the respective models. We also add relearning baseline, where we collect labels from a base model, Mistral-7b-0.1v on a corpus of 600 prompts (where Mistral-7b-0.3 model deflected). For our relearning experiments, this training set remains the same for all models. We provide details of our evaluation set in Appendix, Table \ref{tab:rai_eval}.



 We present the unlearning results in Table \ref{deflect_cyber}. We observe that for all three models, unlearning has been nearly as effective as relearning in reducing the refusals. The refusal scores has been reduced by 61\%, 83\%, and 74.43\% for Mistral-7B-0.3v, Qwen-7B-2.5, and Qwen-32B-2.5 model without degrading the model utility (\textcolor{blue}{fix MMLU  for qwen-32b-2.5v via better checkpointing}). In addition, we also report refusal scores on 6 other RAI policies, and find that unlearning refusal on cybersecurity does not cause significant reduction in refusals on other policies except sensitive content concept for Qwen model. For Qwen model series, we observe around 10\% reduction in refusals for sensitive content.



==> From_Narrow_unlearning_to_Emergent_Misalignment/sections/backup_sections/literaturereview.tex <==
\section{Literature Review}
\subsection{Steering LLMs}
Fine-grained steering of LLMs is an emerging research area with significant benefits for improving model reliability and controllability. Prompting and finetuning are widely used methods that modify model behavior through external inputs or parameter updates, respectively. Machine unlearning has also gained attention as a steering method that facilitates the removal of undesirable concepts from the model under the 'right to be forgotten'. Besides these methods, recent advances in interpretability research have introduced new techniques for steering internal representations at inference time, without altering model weights. Techniques such as linear probing, sparse autoencoders (SAEs), and linear artificial tomography enable concept detection and targeted intervention, allowing models to be guided based on specific objectives or latent concepts.

\textbf{ Some recent works/techniques specific to targeted intervention}
\begin{itemize}
    \item \textbf{Intent-based finetuning}: Misalignment paper \cite{betley2025emergent} shows that if they add `this is for education purpose' in the question prompt, and learn over insecure code data, model does not become misaligned across other tasks/policies.
    \item \textbf{Steering representations towards alignment at inference-time:} \cite{stickland2024steering} work mitigates the risk-related model behaviour by classifying inputs as potentially problematic, then selectively apply safety steering vectors on these problematic inputs, i.e. adding particular vectors to model hidden states at inference time.
    \item \textbf{Interpolate between base model and aligned model} these works exploit a classifier to classify the input, and interpolate between the base and aligned model based on classification strength \cite{liu2024decoding} \cite{krishna2025disentangled}
    \item \textbf{Steering model's generation away from refusal at inference-time} \cite{arditi2024refusal} find that refusal is mediated by one single direction (study done on 13 models), and if we erase this direction from the residual stream then model starts responding to harmful queries.
\end{itemize}

\label{literature_review}
\subsection{RAI Guardrails}
Researchers have developed sophisticated guardrail models to monitor and filter model inputs and outputs to ensure reliability and safety of the generations. Some of the state-of-the-art guardrails (e.g., LlamaGuard,  WildGuard, AEGIS, and ShieldGemma) are fine-tuned from pre-trained or
instruction-tuned LMs and yield high performance in classifying the safe and unsafe prompts/generations. The other line of work exploits model's internal states to perform safety or hallucination classification, and have shown promising results. However, one critique of these classification methods is that they incur extra inference cost. Though these works argue that the cost becomes negligible as compared to larger models and their safety/intervention benefits, however, our work investigates steering baselines that minimize the inference cost. 
\subsection{RAI Alignment}
\textcolor{blue}{add safety alignment papers} 


==> From_Narrow_unlearning_to_Emergent_Misalignment/sections/backup_sections/problem_def.tex <==
\section{Problem Definition}

Let there be an RAI aligned model $\pi_{\theta_{aligned}}(.)$ parameterized by $\theta_{aligned}$ parameters that has $N$ safety policies integrated into its parameters via alignment fine-tuning. Let there be one policy out of $N$ policies that needs to be reconfigured either to facilitate a policy change or a customer use-case. For the given change, it is needed that model's safety aligned behavior should stay intact across other RAI policies. 


A naive baseline of this problem can be RAI-guardrail-based selective refusal baseline, i.e., given an RAI guardrail classifier, $f(.)$ applied on input prompt $x$, a decision function $g(.)$ can be performed whether to route the prompt to the base model $\pi_{\theta_{base}}(.)$ or an aligned model $\pi_{\theta_{aligned}}(.)$. Given \( g(x) = \mathbf{1}\{f(x) > \gamma\} \) for a predetermined threshold $\gamma$ on an RAI policy, if $g(x) = 1$ then the generative distribution of output follows $P(\textbf{y} | \textbf{x}, \theta_{base})$ else $P(\textbf{y} | \textbf{x}, \theta_{aligned})$. It is easy to note that the success of this setup depends on the performance of RAI guardrails classifier $f(.)$ and the threshold. Though various works have proposed strong RAI guardrail models such as LLamaGuard and GemmaShield, these guardrail models incur extra inference cost, are susceptible to misclassification errors, and require two models at deployment, making it an impractical solution for real-world deployment.

Given the high inference cost of the RAI-guardrail-based selective refusal baseline, we investigate alternative LLM steering methods, fine-tuning and unlearning, to steer model generations away from refusals on one concept without degrading its refusal performance on others. 


% The core motivation for exploring these baselines is to reduce inference-time overhead by instead incurring a one-time training cost, which we refer to as the steering cost in our work. Below, we define and compare the proposed steering baselines for enabling RAI reconfigurability.

\section{Machine Unlearning}
Large language models often memorize sensitive and undesireable data during pretraining phase. Under the `the right to be forgotten', machine unlearning has shown promising performance in eliminating the effects of such undesireable data memorization removing specific concepts such as celebrity/personal information. However, in this work, we investigate its potential to unlearn refusals on an RAI policy after alignment finetuning. 


Essentially, we are interested in investigating, is it possible to unlearn refusals on a concept such as cybersecurity so that model starts generating compliance responses for that concept? Since refusals are connected to so many concepts during alignment training, we are interested in investigating its potential to perform targetted unlearning for specific concepts to achieve RAI reconfigurability.

Our unlearning training pipeline consists of 2 phases, 1) data collection, i.e, deflection response collection on a particular concept, 2) machine unlearning, where we perform unlearning on the deflection responses. For the first phase, we perform inference on a selected set of prompts pertaining to that concept and collect deflection responses. The set of prompts collected and their associated deflection responses becomes the unlearning set ($x_{i}, y_{i}) \in \mathcal{D}_{R}$. For unlearning those deflections, we apply negative preference optimization (NPO) loss objective. For a given prompt $x_{i}$, our losing response is the deflection response $y_{i}$ without any positive/win response in direct preference optimization (DPO) loss as shown below,
\begin{equation}
    \mathcal{L}_{\text{NPO}, \beta}(\theta) = -\frac{2}{\beta} \, \mathbb{E}_{\mathcal{D}_{R}} \left[ \log \, \sigma\left( -\beta \log \frac{\pi_{\theta}(y \mid x)}{\pi_{\text{ref}}(y \mid x)} \right) \right]
    \label{NPO}
\end{equation}


\begin{itemize}
    \item ($x_{i}, y_{i}) \in \mathcal{D}_{R}$ is the set of prompts and their associated deflection responses.
    \item $\pi_{ref}(y|x)$ is the conditional probability distribution of the aligned model.
    \item $\pi_{\theta}(y|x)$ is the conditional probability distribution of the optimized model.
    % \item CE(.) cross entropy loss.
    % \item $\sigma (t) = \frac{1}{(1 + e^{-t})}$  is the sigmoid function, and  $\beta$ > 0 is the inverse temperature.
\end{itemize}


% \subsubsection{Prefix-Based Unlearning} 
% For some cases, we also explore few tokens based unlearning, where instead of unlearning on full response $y$, we unlearn first few tokens [i.e., first 20 characters of the deflection response $y$.] The purpose of this ablation is to study the shallow safety alignment with the unlearning objective. \textbf{For now, I am writing it here but in our paper we can move it to ablation study or appendix depending on the story}
% \subsection{Machine Relearning}
% For relearning, we collect generations from a base (unaligned) model on the same set of prompts, and use cross-entropy loss to relearn the base model knowledge.
% \subsection{Steering Vectors}

% \input{Tables/steering_cost}

\begin{equation}
    \mathcal{L}_{\text{NPO+retain}, \beta}(\theta) = -\frac{2w_{1}}{\beta} \, \mathbb{E}_{\mathcal{D}_{T}} \left[ \log \, \sigma\left( -\beta \log \frac{\pi_{\theta}(y \mid x)}{\pi_{\text{ref}}(y \mid x)} \right) \right] - w_2* \mathbb{E}_{\mathcal{D}_{R}}[\hat{t} \log (\pi_{\theta}( z))]
    \label{NPO}
\end{equation}

\begin{itemize}
    \item ($x_{i}, y_{i}) \in \mathcal{D}_{T}$ is the set of prompts and their associated deflection responses.
    \item $\pi_{ref}(y|x)$ is the conditional probability distribution of the aligned model.
    \item $\pi_{\theta}(y|x)$ is the conditional probability distribution of the optimized model.
    \item ($z_{i}, \hat{t}_{i}) \in \mathcal{D}_{R}$, retain set.
    \item $w_{1}$ and $w_{2}$ are the regularization hyper-parameters. 
    % \item $\sigma (t) = \frac{1}{(1 + e^{−t})}$  is the sigmoid function, and  $\beta$ > 0 is the inverse temperature.
\end{itemize}

==> From_Narrow_unlearning_to_Emergent_Misalignment/sections/backup_sections/toxicity_results.tex <==
\section{Hidden Policy Entanglements}
Can sensitive information be deleted from llms? objectives for defending against extraction attacks
\section{}

Given our observation that unlearning can effectively reduce refusals in the Cybersecurity domain, a natural question arises: Can we unlearn refusal on any policy? Moreover, does unlearning always occur without unintended interference across other policies?

It is important to note that similar questions have been explored in the context of relearning in prior work. A recent line of research under the umbrella of emergent misalignment has demonstrated that relearning insecure code generation can lead to broader model misalignment. For instance, finetuning solely on cybersecurity tasks has been shown to unintentionally induce toxic behavior in free-form question answering. Inspired by these findings from narrow finetuning literature, we investigate whether a similar phenomenon exists in the context of narrow refusal unlearning, revealing what we term as hidden policy entanglement.

\subsection{Unlearn refusals on Toxicty}
To investigate hidden policy entanglement, we design an inverse experimental setup: rather than unlearning refusals on cybersecurity and measuring toxicity in the activations, we unlearn refusals on toxicity and observe the downstream impact on cybersecurity refusals. Specifically, we curate a set of toxic prompts by sampling refusals directed at three randomly selected hate groups from the ToxiGen dataset. We gather these refusals using Mistral-7B-0.3v and Qwen-7B-2.5. For relearning, we use Mistral-0.1v to provide base model generations.

\textit{\textbf{Question 1: Can we unlearn refusal on any policy?}}
Surprisingly, we find that toxicity is a particularly difficult policy to unlearn. When applying unlearning across the full response, the model often becomes more toxic toward the user prompt but still refrains from completing the toxic request. We provide an example of such paradox in Figure~\ref{fig:fullresponse}.

\begin{figure}[h]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/firstfewtokens.pdf}
    \caption{Unlearning toxicity [Full response versus First few Tokens]}
    \label{fig:fullresponse}
\end{figure}

\textit{\textbf{Question 2: Is unlearning susceptible to causing misalignment across other policies?}}
To explore this question, we perform unlearning on toxicity and monitor the KL divergence between the initial aligned model and the unlearned model, focusing on the first-token distribution. Prior work has shown that safety alignment is often most pronounced in the initial tokens, making this a reliable indicator of early-generation behavioral shifts. As shown in Figure \ref{fig:lossvsKL}, we observe that as unlearning on toxicity progresses, the KL divergence on the cybersecurity task also increases, despite the fact that the model is not being directly trained on that domain. At just 24\% training step, the attack success rate on cybersecurity jumps from 33\% to 72\% for the Mistral model. This highlights a surprising interconnection between the toxicity and cybersecurity policies, illustrating that unlearning on one axis can unintentionally weaken safeguards on another. Please note that this change does not impact model utility. Further, besides safety, the other policies also remain unchanged, i.e, preserve refusal, for the Mistral model from unlearning toxicity as shown in Table \ref{fig:toxicity}.



\begin{figure}[t]
    \centering
    \begin{minipage}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/npo_loss.pdf}
        \caption*{
            \centering
            (a) \textbf{Toxicity:} \\ Unlearning (NPO) loss versus training steps
        }
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/kl_divergence.pdf}
        \caption*{
            \centering
            (b) \textbf{CyberSecurity:} \\ KL divergence between aligned and unlearned model
        }
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.29\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/MiTREAttack.pdf}
        \caption*{
            \centering
            (c) \textbf{CyberSecurity:} \\ Attack success rate increased from 33\% to 72\%
        }
    \end{minipage}
    \caption{\textbf{Hidden policy entanglements (Mistral Model):} Unlearning toxicity makes model more vulnerable to cybersecurity attacks. As unlearning on toxicity progresses (subfigure (a)), the KL divergence between the initial aligned model, and the unlearned model on the first token distribution increases for cybersecurity domain (subfigure (b)), leading to 39\% increase in cybersecurity attack success rate for Mistral-7B-0.3v model (subfigure (c)).}
    \label{fig:lossvsKL}
\end{figure}




\input{Tables/deflection_toxicity}



% \textbf{Next ..}
 
% \begin{itemize}
%     \item Running Safety and Sensitive Content unlearning experiments (deadline 28 July)
%     \item Steering Vectors Baseline: I have also been working on implementing steering vectors baseline (ICLR'25) for our Cybersecurity experiment setup. I have extracted the concept and behaviour vectors for cybersecurity pillar, and working on hyper-parameter tuning for the strength of steering for final evaluations. We should have this baseline in Table 2 by Monday as well.
% \end{itemize}


==> From_Narrow_unlearning_to_Emergent_Misalignment/sections/introduction.tex <==
\section{Introduction}

Large language models (LLMs) undergo extensive alignment training to instill human-defined safety policies, mitigating risks associated with misuse, bias, and harmful outputs (\cite{kenton2021alignment, matthews2022alignment}). These models are aligned across various responsible AI (RAI) concepts to refuse harmful prompts and promote safe deployment. However, the notion of what is harmful varies across contexts (\cite{he2024whose, yuan2025hard}), for example, providing medical advice may be harmful in some situations (\cite{wang2023not}) but essential in others, such as in medical chatbots (\cite{xie2024me}). 
This contextual variability makes fixed alignment configurations insufficient for many real-world deployments (\cite{yuan2025hard}). While retraining models for each use case is one option, it incurs substantial computational and developmental costs. To address this challenge, we investigate the effects of narrow, targeted interventions on already aligned models as an efficient alternative.
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/main_figure.jpg}
    \caption{
    \textbf{From Narrow Unlearning to Emergent Misalignment.}
    Subfigure (a) shows the refusal profile of the aligned model, Mistral-7B-0.3v across 7 RAI concepts, where each axis corresponds to a RAI concept and the value on the axis indicates the model’s refusal score. Subfigure (b) illustrates the effect of narrow refusal unlearning on the \textit{Safety} concept, and its unintended impact, low refusal score, across unrelated concepts such as \textit{Bias} and \textit{Cybersecurity}. 
    Subfigure (c) demonstrates \textit{Alignment Recovery} across the affected domains via refusal unlearning augmented with cross-entropy loss function on a small set of retain data from the affected domains.
}
    % \caption{
    % \textbf{From Narrow Unlearning to Emergent Misalignment.} Subfigure (a) shows the refusal profile of the aligned model, Mistral-7B-0.3v, where  each axis represents a Responsible AI (RAI) concept, and the filled area denotes the model’s refusal score. Subfigure (b) illustrates the effect of narrow refusal unlearning on the \textit{Safety} concept and its unintended impact, low refusal score, across unrelated concepts such as \textit{Bias} and \textit{Cybersecurity}. Subfigure (c) demonstrates \textit{Alignment Recovery} across the impacted domains via an augmented loss function trained on a small retain set from the impacted domains.}
        % \textbf{From Narrow Unlearning to Emergent Misalignment:}
        % Each axis represents a RAI concept, and the filled area shows model refusal score. Subfigure (a)  shows the refusal score of  Mistral-7B-0.3v model, subfigure (b) shows the intervention via narrow refusal unlearning on the safey concept, and its impact on other concepts such as Bias, Cybersecurity. Subfigure (c) illustrates the Alignment Recovery across impact domains via augmented loss function on a small set of retain data from the affected domains.
    % }
    \label{fig:rai_radar_intro}
\end{figure*}

Recent studies have shown that narrow-domain interventions, such as fine-tuning on insecure code-writing task, can induce malicious behavior in models across unrelated domains (\cite{betley2025emergent}). Follow-up works demonstrate that other datasets, including medical or legal advice, can produce similar effects when used for narrow fine-tuning (\cite{wang2025persona}). Since fine-tuning requires learning from harmful labeled data, our work explores narrow refusal unlearning as an alternative method that do not require the model to learn from harmful labeled data. We investigate machine unlearning (\cite{zhang2024negative}) to enable compliance (i.e., non-refusal) responses for targeted concepts. Specifically, our work explores three research questions: \textit{\textbf{R1}} Can we steer the model away from refusal on a specific RAI concept using machine unlearning without causing emergent misalignment across other concepts? \textit{\textbf{R2}} If emergent misalignment occurs, can we contain it?  
\textit{\textbf{R3}} Can EMA be predicted by investigating the concept entanglements at representation level?



 



==> From_Narrow_unlearning_to_Emergent_Misalignment/sections/machine_unlearning.tex <==
\vspace{-4mm}
\section{Approach}
\vspace{-3mm}
To unlearn refusals, we investigate machine unlearning and employ negative preference optimization (NPO) loss objective (\cite{zhang2024negative}) for its promising performance against catastrophic forgetting. In this objective, for a given prompt $x_{i}$, $y_{i}$ is the losing response without any positive/win response in direct preference optimization (DPO) loss (\cite{rafailov2023direct}) as shown below,
\begin{equation}
    \mathcal{L}_{\text{NPO}, \beta}(\theta) = -\frac{2}{\beta} \, \mathbb{E}_{\mathcal{D}_{R}} \left[ \log \, \sigma\left( -\beta \log \frac{\pi_{\theta}(y \mid x)}{\pi_{\text{ref}}(y \mid x)} \right) \right]
    \label{NPO}
\end{equation}
where $\pi_{ref}(y|x)$ is the conditional probability distribution of the aligned model, $\pi_{\theta}(y|x)$ is the conditional probability distribution of the optimized model, $\sigma (t) = \frac{1}{(1 + e^{-t})}$  is the sigmoid function, ($x_{i}, y_{i}) \in \mathcal{D}_{R}$ is the unlearning set, and  $\beta$ > 0 is the inverse temperature. Overall, our proposed refusal unlearning training pipeline consists of 2 phases, 1) \textit{Data Collection}, where given an RAI concept and an aligned model $\pi_{ref}(.)$, we perform inference on the set of prompts pertaining to the intervention concept and collect deflection/refusal responses. The set of prompts and their associated deflection responses becomes the unlearning set ($x_{i}, y_{i}) \in \mathcal{D}_{R}$, 2) \textit{Machine Unlearning}, where we perform unlearning on the dataset set, $\mathcal{D}_{R}$, collected in phase 1. 









%our losing response is the refusal response $y_{i}$ without any positive/win response in direct preference optimization (DPO) loss as shown below,

% For unlearning those deflections, we apply negative preference optimization (NPO) loss objective \cite{zhang2024negative} for its promising performance against catastrophic forgetting. For a given prompt $x_{i}$, our losing response is the refusal response $y_{i}$ without any positive/win response in direct preference optimization (DPO) loss as shown below,
% \begin{equation}
%     \mathcal{L}_{\text{NPO}, \beta}(\theta) = -\frac{2}{\beta} \, \mathbb{E}_{\mathcal{D}_{R}} \left[ \log \, \sigma\left( -\beta \log \frac{\pi_{\theta}(y \mid x)}{\pi_{\text{ref}}(y \mid x)} \right) \right]
%     \label{NPO}
% \end{equation}
% where $\pi_{ref}(y|x)$ is the conditional probability distribution of the aligned model, $\pi_{\theta}(y|x)$ is the conditional probability distribution of the optimized model, $\sigma (t) = \frac{1}{(1 + e^{-t})}$  is the sigmoid function, and  $\beta$ > 0 is the inverse temperature.


% Large language models often memorize sensitive and undesireable data during pretraining phase. Under the `the right to be forgotten', machine unlearning has shown promising performance in eliminating the effects of such undesireable data memorization removing specific concepts such as celebrity/personal information. However, in this work, we investigate its potential to unlearn refusals on an RAI policy concept after alignment finetuning. 


% Essentially, we are interested in investigating, is it possible to unlearn refusals on a concept such as cybersecurity so that model starts generating compliance responses for that concept? Since refusals are connected to so many concepts during alignment training, that is why, we also investigate its influence on other RAI concepts to monitor emergent misalignment.



==> From_Narrow_unlearning_to_Emergent_Misalignment/sections/unlearn_safety.tex <==
\section{Unlearning Refusal on Safety}
% \input{Tables/deflection_safety_sub}
% \input{Tables/deflection_Safety}

\begin{equation}
    c_{\text{safety}} = PCA(H_{\text{safety}}^{+})
\end{equation}


\begin{equation}
    h_{\text{second policy}} 
\end{equation}

\begin{equation}
    \text{cosine similarity}( c_{\text{safety}}, h_{\text{second policy}}) 
\end{equation}

\begin{equation}
    c_{\text{safety}} 
\end{equation}



\begin{equation}
    \textbf{H}_{\text{concept}}^{+} \in \mathbb{R}^{L \times N \times D}
\end{equation}

\begin{equation}
    c_{\text{concept},\,l} 
    = \mathrm{PCA}\!\left( \bar{\mathbf{H}}^{+}_{\text{concept},\,l} \right)
\end{equation}



\begin{equation}
    \textbf{H}_{\text{concept}}^{+} \in \mathbb{R}^{L \times N \times D}
\end{equation}

\begin{equation}
    {\mathbf{H}}^{+}_{\text{concept},\,l} \in \mathbb{R}^{ N \times D}
\end{equation}



\begin{equation}
    \textbf{H}_{\text{safety}}^{+} \in \mathbb{R}^{L \times N \times D}
\end{equation}


\begin{equation}
    c_{\text{safety},\,l} 
    = \mathrm{PCA}\!\left( \bar{\mathbf{H}}^{+}_{\text{safety},\,l} \right)
\end{equation}


\begin{equation}
    \text{cosine similarity}( c_{\text{safety},\,l}, h_{\text{second concept},\,l}) 
\end{equation}
\input{Tables/deflection_sub_mstsmodified}

==> From_Narrow_unlearning_to_Emergent_Misalignment/sections/unlearning_cybersecurity.tex <==
% \section{Unlearning Cybersecurity}
% \begin{itemize}
%     \item No broader impact on other policies
%     \item Full response unlearning is more targeted than first few tokens
    
% \end{itemize}

% \input{Tables/deflection_security}

==> From_Narrow_unlearning_to_Emergent_Misalignment/sections/unlearningtoxicity.tex <==
\section{Unlearning Toxicity}
Toxic Personas 
\input{Tables/deflection_toxicity}

==> Tables/backup_tables/dataset_taxonomy.tex <==

\begin{table}[ht]
\centering
\caption{Dataset Taxonomy for Evaluating LLM Steering Baselines on the CyberSecurity RAI Pillar}
\label{tab:rai_eval}
\renewcommand{\arraystretch}{1.2} % increases row height
\setlength{\tabcolsep}{10pt} % adjusts column spacing

\begin{tabular}{@{} l l c l @{}}
\toprule
\textbf{Policy} & \textbf{Dataset Name} & \textbf{Count} & \textbf{Refusal Evaluation} \\
\midrule
Toxicity             & Toxigen           & 200  & Is response toxic?              \\
Safety               & MSTS              & 186  & Is response unsafe?             \\
CyberSecurity        & CyberSecEval      & 200  & Refusal                    \\
Privacy              & Do-not-answer     & 200  & Refusal                     \\
Medical \& Legal     & Do-not-answer     & 96   & Refusal   \\
Sensitive Content    & Do-not-answer     & 114  & Refusal                         \\
Bias                 & BBQ               & 200  & Is response biased?             \\
\midrule
Over-Deflection      & XSTest            & 200  & Refusal\label{fig:toxicity}                       \\
\bottomrule
\end{tabular}
\end{table}


==> Tables/backup_tables/deflect.tex <==

\begin{table*}[ht]
\caption{Refusal score comparison of steering baselines on various models for CyberSecurity RAI Policy Intervention}
\centering
\small  % Reduce font size
\setlength{\tabcolsep}{8pt}  % Adjust column spacing
\renewcommand{\arraystretch}{1.2}  % Row spacing
\resizebox{\textwidth}{!}{%
\begin{tabular}{c l|c|c}
\toprule
& \textbf{Baselines}  
& \textbf{Safety } (Deflection $\uparrow$) 
& \textbf{CyberSecurity} (Deflection $\downarrow$) \\
\midrule
\addlinespace[6pt]

\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{\scriptsize Qwen-7B-2.5}}}
& Aligned   & 94.5\% & 93\% \\
& Unlearn [Full Response]  & 60.\% & 9\% \\
& Unlearn [First Few Tokens]  & \textbf{eval running} & 9\% \\

\addlinespace[6pt]
\bottomrule
\end{tabular}%
}
\label{deflect}
\end{table*}



==> Tables/backup_tables/deflection.tex <==


\begin{table*}[ht]
\caption{Deflection (D) and Harmfulness (H) score comparison of steering baselines comparison on various models for Toxicity RAI Policy Intervention}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{c l|cc|cc|cc|c|c}
\toprule
& \textbf{Intervention Baselines} 
& \multicolumn{2}{c|}{\textbf{ToxiGen} } 
& \multicolumn{2}{c|}{\textbf{StrongReject} } 
& \multicolumn{2}{c|}{\textbf{CyberSecEval} } 
& \multicolumn{1}{c|}{\textbf{XSTest}} 
& \textbf{MMLU}  \\
& 
& \textbf{Deflection} ($\downarrow$) & \textbf{Harmful} 
& \textbf{Deflection} ($\uparrow$)& \textbf{Harmful} 
& \textbf{Deflection} ($\uparrow$)& \textbf{Harmful} 
& \textbf{Deflection}($\downarrow$)
& \textbf{Accuracy} ($\uparrow$)\\

\midrule
\multirow{5}{*}{\rotatebox[origin=c]{90}{\scriptsize\textbf{Mistral-7B-0.3v}}}
& Aligned                & 72.25& 18.68&
59.50 & 60.05 & 64.00 & 90.06& 45.50  &59.10\\
\cmidrule{2-10}
& Relearn &15.50&99.95&47.50&76.80&9.00&96.73&39.00&59.40
 \\
& Unlearn               & 17.00&68.75&51.00&58.43&17.00&92.06&39.00&
59.70\\
& Relearn + Retain  & 16.00&99.95&80.00&26.75&62.00&67.75&50.50&59.40
\\
& Unlearn + Retain   &15.50&68.95&70.50&44.90&60.00&73.51&46.00&59.40
\\
\hline\hline
\addlinespace[7pt]
\multirow{3}{*}{\rotatebox[origin=0]{90}{\scriptsize\textbf{Qwen-7b-2.5}}}
& Aligned               & 84.50& - & 95.00 &- &59.00& -& 51.00&\\
\cmidrule{2-10}
& Relearn               & 37.00&-&        97.50 & - & 65.50& -& 53.00 \\
& Unlearn  &61.50& -&95.50& -&82.50&-&60.00&  
\\
% & Relearn + Retain   & 68.10          & 57.05 & - & 22.4 \\
% & Unlearn + Retain   & 85.83          & 60.25 & - & 24.4 \\
\addlinespace[3pt]
\hline\hline
\addlinespace[7pt]
\multirow{3}{*}{\rotatebox[origin=c]{90}{\scriptsize\textbf{GPTQ-13b}}}
& Aligned               & \textbf{-} & - & - & - \\
\cmidrule{2-10}
& Relearn               & -          & \textbf{-} & - & \textbf{-} \\
& Unlearn               & -         &- & - & -\\

\hline\hline
\end{tabular}%
}
\label{deflect_toxicity}
\end{table*}


==> Tables/backup_tables/deflection_safety_.tex <==
\begin{table*}[ht]
\caption{\textit{Refusal scores on RAI policies and accuracy on MMLU. Higher is better ($\uparrow$), except for Safety and Over-Deflection.}}
\centering
\resizebox{\textwidth}{!}{%
\LARGE
\begin{tabular}{ll|c|c|c|c|c|c|c|c|c}
\toprule
\textbf{Model} & \textbf{Method} & \textbf{Toxicity} ($\downarrow$) & \textbf{Safety} ($\uparrow$) & \textbf{CyberSec} ($\uparrow$) & \textbf{Sensitive} ($\uparrow$) & \textbf{Bias} ($\uparrow$) & \textbf{Med/Legal} ($\uparrow$) & \textbf{Privacy} ($\uparrow$) & \textbf{OverDefl.} ($\downarrow$) & \textbf{MMLU} ($\uparrow$) \\
\midrule

% \multirow{3}{*}{\textbf{Mistral-7B-0.3v}} 
% & Aligned                & 100.0 & 98.90 & 67.00 & 22.80 & 96.50 & 45.83 & 28.00 & 42.00 & 59.10 \\
% & Relearn                & 14.00 & 75.82 & 14.00 & 22.80 & 91.00 & 39.58 & 26.00 & 34.00 & 59.40 \\
% & Unlearn (first tokens) & 47.00 & 80.76 & 28.00 & 21.92 & 87.50 & 42.73 & 27.50 & 41.50 & 59.70 \\

\midrule

\multirow{2}{*}{\textbf{Qwen-7B-2.5}} 
& Aligned                & 100.0 & 98.35 & 93.00 & 35.00 & 100.0 & 41.67 & 32.00 & 51.50 & 71.70 \\
% & Unlearn [First few tokens]  & 100.0 & 98.35&81.00 & 32.45 & 96.50 & 40.62 & 22.50& 47.50 &  71.70 \\
% & Unlearn [First few tokens] [LoRA, r=128] & 100.0 & 98.35&\textbf{76.00} & 29.82 & 95.50 & 37.50& 26.00& 48.50 &  71.10 \\
% & Relearn                & 34.50 & 98.35 & 93.00 & 45.60 & 91.50 & 46.87 & 34.00 & 53.00 & 71.20 \\
& Unlearn [First few tokens] [Full rank] & 53.50 & 30.76&14.00 & 16.67& 28.50&39.58& 32.00&13.50 & - \\
\bottomrule
\end{tabular}
}
\label{deflect}
\end{table*}



% \begin{table*}[ht]
% \caption{\textit{Refusal Scores on RAI Policies and acc scores on  MMLU}}
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{c l | >{\columncolor{lightgray}}c | c | c | c | c | c | c | c | c}
% \toprule
% & \textbf{Steering Baselines} & \textbf{Toxicity} ($\uparrow$) & \textbf{Safety} ($\uparrow$) & \textbf{CyberSecurity} ($\downarrow$) & \textbf{Sensitive Content} ($\uparrow$) & \textbf{Bias} ($\uparrow$) &  \textbf{Medical\&Legal} ($\uparrow$)&\textbf{Privacy} ($\uparrow$) &\textbf{Over-Deflection} ($\downarrow$) & \textbf{MMLU} ($\uparrow$)\\

% \midrule
% \multirow{5}{*}{\rotatebox[origin=c]{90}{\scriptsize\textbf{Mistral-7B-0.3v}}}
% % & \multicolumn{10}{c}{\cellcolor{orange!15}\textbf{With Early Stopping}} \\
% & Aligned               & 100& 98.90 & 67.00&22.80&96.50&45.83&28.00&42.00&59.10\\
% \cmidrule{2-10}
% & Relearn               & 14.00      &75.82 & 14.00 & 22.80&91.00&39.58&26.00&34.00&59.40\\
% & Unlearn [first few tokens]            & 47.00&80.76       & 28.00 & 21.92 &87.50&42.73&27.50&41.50&59.70\\
% % & Unlearn [First few tokens]                & -         & - & - & -\\
% % & Unlearn [Prefix]                & -         & - & - & -\\
% \addlinespace[12pt]
% % & Relearn + Retain   & -       & - & - & -\\
% % & Unlearn + Retain   & -         & - & - & -\\
% \hline\hline
% \addlinespace[7pt]

% \hline

% \multirow{5}{*}{\rotatebox[origin=0]{90}{\scriptsize\textbf{Qwen-7b-2.5}}}\\
% \addlinespace[7pt]
% & Aligned               & 100.0& 98.35 & 93.00&35.00&100&41.67&32.00&51.50&71.70\\
% \cmidrule{2-10}
% & Relearn               & 34.50         & 98.35 & 93.00& \textbf{45.60}& 91.50&\textbf{46.87}&\textbf{34.00}&\textbf{53.00}&71.20\\
% \addlinespace[7pt]


% \hline\hline
% \end{tabular}%
% }
% \label{deflect}
% \end{table*}


==> Tables/backup_tables/deflection_score_woharm.tex <==


\begin{table*}[ht]
\caption{Baseline comparison of various models for Safety RAI Policy Intervention}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{c l|c|c|c|c| c}
\toprule
& \textbf{Intervention Baselines} & \textbf{ToxiGen} ($\downarrow$) & \textbf{StrongReject} ($\uparrow$) & \textbf{CyberSecEval} ($\uparrow$) & \textbf{XSTest} ($\downarrow$) & \textbf{MMLU} ($\uparrow$)\\
& & \textbf{Deflection Scores} & \textbf{Deflection Scores} & \textbf{Deflection Scores} & \textbf{Deflection Scores} & \textbf{Accuracy} \\
\midrule
\multirow{5}{*}{\rotatebox[origin=c]{90}{\scriptsize\textbf{Mistral-7B-0.3v}}}
& Aligned               & -& - & 71.5&-\\
\cmidrule{2-10}
& Relearn               & -        &- & - & - \\
& Unlearn               & -         & - & - & -\\
& Relearn + Retain   & -       & - & - & -\\
& Unlearn + Retain   & -         & - & - & -\\
\hline\hline
\addlinespace[7pt]
\multirow{3}{*}{\rotatebox[origin=0]{90}{\scriptsize\textbf{Qwen-7b-2.5}}}
& Aligned               & - & - & - &- \\
\cmidrule{2-10}
& Relearn               & -         & - & - & - \\
& Unlearn               & -          & -& - &- \\
% & Relearn + Retain   & 68.10          & 57.05 & - & 22.4 \\
% & Unlearn + Retain   & 85.83          & 60.25 & - & 24.4 \\
\addlinespace[3pt]
\hline\hline
\addlinespace[7pt]
\multirow{3}{*}{\rotatebox[origin=c]{90}{\scriptsize\textbf{GPTQ-13b}}}
& Aligned               & \textbf{-} & - & - & - \\
\cmidrule{2-10}
& Relearn               & -          & \textbf{-} & - & \textbf{-} \\
& Unlearn               & -         &- & - & -\\

\hline\hline
\end{tabular}%
}
\label{deflect}
\end{table*}


==> Tables/backup_tables/deflection_security.tex <==


\begin{table*}[ht]
\caption{Deflection (D) and Harmfulness (H) score comparison of steering baselines comparison on various models for  CyberSecurity RAI Policy Intervention}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{c l|cc|cc|cc|c|c}
\toprule
& \textbf{Intervention Baselines} 
& \multicolumn{2}{c|}{\textbf{ToxiGen} } 
& \multicolumn{2}{c|}{\textbf{StrongReject} } 
& \multicolumn{2}{c|}{\textbf{CyberSecEval} } 
& \multicolumn{1}{c|}{\textbf{XSTest}} 
& \textbf{MMLU}  \\
& 
& \textbf{Deflection} ($\uparrow$) & \textbf{Harmful} 
& \textbf{Deflection} ($\uparrow$)& \textbf{Harmful} 
& \textbf{Deflection} ($\downarrow$)& \textbf{Harmful} 
& \textbf{Deflection}($\downarrow$)
& \textbf{Accuracy} ($\uparrow$)\\
\midrule
\multirow{5}{*}{\rotatebox[origin=c]{90}{\scriptsize\textbf{Mistral-7B-0.3v}}}
& Aligned             & 72.25& 18.68&
59.50 & 60.05 & 64.00 & 90.06& 45.50  &59.10
 \\
\cmidrule{2-10}
& Relearn            &   79.50&18.80&47.50&75.70&0.00&100&44.50&59.50
\\
& Unlearn                &   82.50&13.65&59.50&61.23&02.50&96.75&41.00&60.00\\
& Relearn + Retain   & 78.50&18.30&66.50&50.65&0.00&98.64&45.50&
59.60
\\
% & Unlearn + Retain   & -         & - & - & -\\
\hline\hline
\addlinespace[7pt]
\multirow{3}{*}{\rotatebox[origin=0]{90}{\scriptsize\textbf{Qwen-7b-2.5}}}
& Aligned               & - & - & - &- \\
\cmidrule{2-10}
& Relearn               & -         & - & - & - \\
& Unlearn               & -          & -& - &- \\
% & Relearn + Retain   & 68.10          & 57.05 & - & 22.4 \\
% & Unlearn + Retain   & 85.83          & 60.25 & - & 24.4 \\
\addlinespace[7pt]
\hline\hline
\addlinespace[7pt]
\multirow{3}{*}{\rotatebox[origin=c]{90}{\scriptsize\textbf{GPTQ-13b}}}
& Aligned               & \textbf{-} & - & - & - \\
\cmidrule{2-10}
& Relearn               & -          & \textbf{-} & - & \textbf{-} \\
& Unlearn               & -         &- & - & -\\

\hline\hline
\end{tabular}%
}
\label{deflect}
\end{table*}


==> Tables/backup_tables/deflectionsecurity_woharm.tex <==


\begin{table*}[ht]
\caption{Deflection (D) and Harmfulness (H) score comparison of steering baselines comparison on various models for  CyberSecurity RAI Policy Intervention}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{c l|c|c|c|c|c}
\toprule
& \textbf{Intervention Baselines} 
& \multicolumn{1}{c|}{\textbf{ToxiGen} } 
& \multicolumn{1}{c|}{\textbf{StrongReject} } 
& \multicolumn{1}{c|}{\textbf{CyberSecEval} } 
& \multicolumn{1}{c|}{\textbf{XSTest}} 
& \textbf{MMLU}  \\
& 
& \textbf{Deflection} ($\uparrow$) 
& \textbf{Deflection} ($\uparrow$)
& \textbf{Deflection} ($\downarrow$) 
& \textbf{Deflection}($\downarrow$)
& \textbf{Accuracy} ($\uparrow$)\\
\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{\scriptsize\textbf{Mistral-7B-0.3v}}}
& Aligned             & 72.25& 
59.50  & 64.00 &  45.50  &59.10
 \\
\cmidrule{2-7}
& Relearn            &   79.50&47.50(-11.50) &0.00&44.50&59.50
\\
& Unlearn                &   82.50&59.50&02.50&41.00&60.00\\
& Relearn + Retain   & 78.50&66.50&0.00&45.50&
59.60
\\
% & Unlearn + Retain   & -         & - & - & -\\
\hline\hline
\addlinespace[7pt]
\multirow{3}{*}{\rotatebox[origin=0]{90}{\scriptsize\textbf{Qwen-7b-2.5}}}
& Aligned               & 84.50 & 95.00 & 59.00&51.00 &71.70 \\
\cmidrule{2-7}
& Relearn               & 82.00         & 89.00 (-6.00) & 7.00&49.00 & 71.30 \\
& Unlearn               & 85.00          & 58.00 (-37.00)& 10.00 &47.00&71.50 \\
% & Relearn + Retain   & 68.10          & 57.05 & - & 22.4 \\
% & Unlearn + Retain   & 85.83          & 60.25 & - & 24.4 \\
\addlinespace[7pt]
\hline\hline
\addlinespace[7pt]
\multirow{3}{*}{\rotatebox[origin=c]{90}{\scriptsize\textbf{Qwen-13b}}}
& Aligned               & \textbf{-} & - & - & - \\
\cmidrule{2-7}
& Relearn               & -          & \textbf{-} & - & \textbf{-} \\
& Unlearn               & -         &- & - & -\\

\hline\hline
\end{tabular}%
}
\label{deflect}
\end{table*}


==> Tables/backup_tables/deflectionstoxicity_woharm.tex <==


\begin{table*}[ht]
\caption{Deflection (D) and Harmfulness (H) score comparison of steering baselines comparison on various models for Toxicity RAI Policy Intervention}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{c l|c|c|c|c|c}
\toprule
& \textbf{Intervention Baselines} 
& \multicolumn{1}{c|}{\textbf{ToxiGen} } 
& \multicolumn{1}{c|}{\textbf{StrongReject} } 
& \multicolumn{1}{c|}{\textbf{CyberSecEval} } 
& \multicolumn{1}{c|}{\textbf{XSTest}} 
& \textbf{MMLU}  \\
& 
& \textbf{Deflection} ($\downarrow$)
& \textbf{Deflection} ($\uparrow$)
& \textbf{Deflection} ($\uparrow$)
& \textbf{Deflection}($\downarrow$)
& \textbf{Accuracy} ($\uparrow$)\\

\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{\scriptsize\textbf{Mistral-7B-0.3v}}}
& Aligned                & 72.25&
59.50 &  64.00 &  45.50  &59.10\\
\cmidrule{2-7}
& Relearn &15.50&47.50&9.00&39.00&59.40
 \\
& Unlearn               & 17.00&51.00&17.00&39.00&
59.70\\
& Relearn + Retain  & 16.00&80.00&62.00&50.50&59.40
\\
& Unlearn + Retain   &15.50&70.50&60.00&46.00&59.40
\\
\hline\hline
\addlinespace[7pt]
\multirow{3}{*}{\rotatebox[origin=0]{90}{\scriptsize\textbf{Qwen-7b-2.5}}}
& Aligned               & 84.50&  95.00  &59.00& 51.00&71.70\\
\cmidrule{2-7}
& Relearn               & 37.00&       97.50  & 65.50& 53.00 &71.20\\
& Unlearn  &61.50& 95.50 & 82.50&60.00&  71.12
\\
% & Relearn + Retain   & 68.10          & 57.05 & - & 22.4 \\
% & Unlearn + Retain   & 85.83          & 60.25 & - & 24.4 \\
\addlinespace[3pt]
\hline\hline
\addlinespace[7pt]
\multirow{3}{*}{\rotatebox[origin=c]{90}{\scriptsize\textbf{Qwen-13b}}}
& Aligned               & \textbf{-} & - & - & - \\
\cmidrule{2-7}
& Relearn               & -          & \textbf{-} & - & \textbf{-} \\
& Unlearn               & -         &- & - & -\\

\hline\hline
\end{tabular}%
}
\label{deflect_toxicity}
\end{table*}


==> Tables/backup_tables/hn_score_security.tex <==
\begin{table*}[ht]
\caption{\textit{Harmfulness Scores on RAI Policies + truthful \& acc scores on TruthfulQA and MMLU, respectively}}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{c l|c|c|c|c|c|c|c|c}
\toprule

& \textbf{Steering Baselines} & \textbf{Toxicity} ($\uparrow$) & \textbf{Safety} ($\uparrow$) & \textbf{CyberSecurity} ($\downarrow$) & \textbf{Sensitive Content} ($\uparrow$) & \textbf{Bias} ($\uparrow$) & \textbf{XSTest} ($\downarrow$) & \textbf{TruthfulQA} ($\uparrow$) & \textbf{MMLU} ($\uparrow$)\\

\midrule
\multirow{3}{*}{\rotatebox[origin=c]{90}{\scriptsize\textbf{Mistral-7B-0.3v}}}

& Aligned               & -& - & -&-&-&-&-&-\\
\cmidrule{2-10}
& Relearn               & -        &- & - & - \\
& Unlearn               & -         & - & - & -\\
\addlinespace[7pt]
% & Relearn + Retain   & -       & - & - & -\\
% & Unlearn + Retain   & -         & - & - & -\\
\hline\hline
\addlinespace[7pt]
\multirow{3}{*}{\rotatebox[origin=0]{90}{\scriptsize\textbf{Qwen-7b-2.5}}}
& Aligned               & -& 94.50 & 93.00&-&-&-&-&71.70\\
\cmidrule{2-10}
& Relearn               & -         & - & - & - \\
& Unlearn               & -          & -& - &- \\
% & Relearn + Retain   & 68.10          & 57.05 & - & 22.4 \\
% & Unlearn + Retain   & 85.83          & 60.25 & - & 24.4 \\
\addlinespace[3pt]
\hline\hline
\addlinespace[8pt]
\multirow{3}{*}{\rotatebox[origin=c]{90}{\scriptsize\textbf{Qwen-32b-2.5}}}
& Aligned               & \textbf{-} & - & - & - \\
\cmidrule{2-10}
& Relearn               & -          & \textbf{-} & - & \textbf{-} \\
& Unlearn               & -         &- & - & -\\
\addlinespace[3pt]
\hline\hline
\end{tabular}%
}
\label{deflect}
\end{table*}


==> Tables/backup_tables/steering_cost.tex <==
\vspace{-10pt}
\begin{table}[t!]
\centering
\scriptsize
\renewcommand{\arraystretch}{1.1} % slightly reduced row height
\setlength{\tabcolsep}{8pt}       % reduced column padding
\caption{Reconfigurability Cost comparison of different Baselines}
\label{tab:costs}
\begin{tabular}{@{} lccc @{}}
\toprule
\textbf{RAI Reconfigurability Baseline} & \textbf{Misalignment Cost} & \textbf{Inference Cost} & \textbf{Steering Cost} \\
\midrule
RAI-Guardrail     & Yes & 2x  & NA   \\
Finetuning        & Yes & 1x  & Yes  \\
Unlearning        & Yes & 1x  & Yes  \\
Steering Vectors  & Yes & 1x  & Yes  \\
\bottomrule
\end{tabular}
\end{table}


==> Tables/backup_tables/tentative_plan.tex <==


\begin{table*}[ht]
\caption{Refusal score comparison of steering baselines comparison on various models for X RAI Policy Intervention}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{c l|c|c|c|c|c|c|c|c}
\toprule
& \textbf{Intervention Baselines} 
& \multicolumn{1}{c|}{\textbf{Security} } 
& \multicolumn{1}{c|}{\textbf{Safety} } 
& \multicolumn{1}{c|}{\textbf{Sensitive Content} } 
& \multicolumn{1}{c|}{\textbf{Bias}} 
& \multicolumn{1}{c|}{\textbf{Toxicity}} 
& \multicolumn{1}{c|}{\textbf{Over-Deflection}} 
& \multicolumn{1}{c|}{\textbf{TruthfulQA}}
& \textbf{MMLU}  \\
& 
& \textbf{Refusal} ($\downarrow$) &  \textbf{Refusal} ($\uparrow$)
& \textbf{Refusal} ($\uparrow$)&  \textbf{Refusal} ($\uparrow$)
& \textbf{Refusal} ($\uparrow$)&  \textbf{Refusal} ($\downarrow$) 
& \textbf{Accuracy} ($\uparrow$) & \textbf{Accuracy} ($\uparrow$)\\
\midrule
\multirow{5}{*}{\rotatebox[origin=c]{90}{\scriptsize\textbf{Mistral-7B-0.3v}}}
& Aligned             & -
 \\
\cmidrule{2-10}
& Relearn            & -
\\
& Unlearn                &   \\
& Relearn + Retain   & -
\\
% & Unlearn + Retain   & -         & - & - & -\\
\hline\hline
\addlinespace[7pt]
\multirow{3}{*}{\rotatebox[origin=0]{90}{\scriptsize\textbf{Qwen-7b-2.5}}}
& Aligned               & - & - & - &- \\
\cmidrule{2-10}
& Relearn               & -         & - & - & - \\
& Unlearn               & -          & -& - &- \\
% & Relearn + Retain   & 68.10          & 57.05 & - & 22.4 \\
% & Unlearn + Retain   & 85.83          & 60.25 & - & 24.4 \\
\addlinespace[7pt]
\hline\hline
\addlinespace[7pt]
\multirow{3}{*}{\rotatebox[origin=c]{90}{\scriptsize\textbf{GPTQ-13b}}}
& Aligned               & \textbf{-} & - & - & - \\
\cmidrule{2-10}
& Relearn               & -          & \textbf{-} & - & \textbf{-} \\
& Unlearn               & -         &- & - & -\\

\hline\hline
\end{tabular}%
}
\label{deflect}
\end{table*}


==> Tables/deflection_Safety.tex <==
\begin{table*}[ht]
\caption{\textit{Refusal scores on RAI policies and accuracy on MMLU. Higher is better ($\uparrow$), except for Safety and Over-Deflection.}}
\centering
\resizebox{\textwidth}{!}{%
\LARGE
\begin{tabular}{ll|c|>{\columncolor{orange!20}}c|c|c|c|c|c|c|c}
\toprule
\textbf{Model} & \textbf{Method} & \textbf{Toxicity} ($\uparrow$) & \textbf{Safety} ($\downarrow$) & \textbf{CyberSec} ($\uparrow$) & \textbf{Sensitive} ($\uparrow$) & \textbf{Bias} ($\uparrow$) & \textbf{Med/Legal} ($\uparrow$) & \textbf{Privacy} ($\uparrow$) & \textbf{OverDefl.} ($\downarrow$) & \textbf{MMLU} ($\uparrow$) \\
\midrule

\multirow{3}{*}{\textbf{Mistral-7B-0.3v}} 
& Aligned                & 100.0 & 98.90 & 67.00 & 22.80 & 96.50 & 45.83 & 28.00 & 42.00 & 59.10 \\
& Finetune [LoRA] & 93.0& 23.62 & 17.00 & 8.7 & 45.0& 30.21& 17.00 & 17.00 & 58.45 \\
% & \textbf{$\Delta$}&  \textbf{(-7.00)} & \textbf{(-75.28)} & \textbf{(-50.00)} & \textbf{(-14.10)} & \textbf{(-51.50)} & \textbf{(-15.62)} & \textbf{(-11.00)} & \textbf{(+25.00)} & \textbf{(-0.65)} \\
& Finetune + Retain [LoRA] & 97.5 &28.02& 99.00 & 22.80& 96.00& 53.13& 43.00& 11.50& 58.21 \\
% &\textbf{$\Delta$} &  \textbf{(-2.50)} & \textbf{(-70.88)} & \textbf{(+32.00)} & \textbf{(0.00)} & \textbf{(-0.50)} & \textbf{(+7.30)} & \textbf{(+15.00)} & \textbf{(+30.50)} & \\
& Unlearn [LoRA] & 96.50 & 64.83& 10.00 & 16.67 & 39.50& 16.67& 9.5 & 34.50& 57.41 \\
% &\textbf{$\Delta$} &  \textbf{(-3.50)} & \textbf{(-34.07)} & \textbf{(-57.00)} & \textbf{(-6.13)} & \textbf{(-57.00)} & \textbf{(-29.16)} & \textbf{(-18.50)} & \textbf{(+7.50)}  \\
& Unlearn + Retain [LoRA] & 94.00 & 73.08& 69.50 & 33.33& 56.50& 26.04& 18.00& 38.00& 57.01 \\
% &\textbf{$\Delta$} &  \textbf{(-6.00)} & \textbf{(-25.82)} & \textbf{(+2.50)} & \textbf{(+10.53)} & \textbf{(-40.00)} & \textbf{(-19.79)} & \textbf{(-10.00)} & \textbf{(+4.00)} & \textbf{-} \\




% & Unlearn [LoRA] & 90.0 & 73.00 & 10.50 & 17.54 & 62.50& 19.79& 14.00 & 37.00 & - \\
% &\textbf{$\Delta$} &  \textbf{(-10.00)} & \textbf{(-25.90)} & \textbf{(-56.50)} & \textbf{(-5.26)} & \textbf{(-34.00)} & \textbf{(-26.04)} & \textbf{(-14.00)} & \textbf{(-5.00)} & \textbf{-} \\
\midrule

\multirow{2}{*}{\textbf{Qwen-7B-2.5}} 
& Aligned                & 100.0 & 98.35 & 93.00 & 35.00 & 100.0 & 41.67 & 32.00 & 51.50 & 71.70 \\
& Finetune [Full rank ] & 62.00 & 23.07&5.00 & 17.54& 34.50&21.85& 12.00&17.00 &- \\
% & \textbf{$\Delta$} &  \textbf{(-38.00)} & \textbf{(-75.28)} & \textbf{(-88.00)} & \textbf{(-17.46)} & \textbf{(-65.50)} & \textbf{(-19.82)} & \textbf{(-20.00)} & \textbf{(+34.50)} &70.32 \\
& Finetune + Retain [Full rank ] & 85.00 & 26.37&75.00 & 24.56& 85.00&44.79& 35.50&21.00  \\
& Finetune + Retain [Full rank ] & 85.00 & 26.37&75.00 & 24.56& 85.00&44.79& 35.50&21.00  \\
 

&Unlearn [Full rank ] & 71.00 & 55.49&13.00 & 7.00& 62.00&33.30& 25.00&10.50 & 71.10 \\
% & \textbf{$\Delta$} & \textbf{(-29.00)} & \textbf{(-42.86)} & \textbf{(-80.00)} & \textbf{(-28.00)} & \textbf{(-38.00)} & \textbf{(-8.37)} & \textbf{(-7.00)} & \textbf{(+41.00)} & \textbf{(-0.60)}  \\

&Unlearn + Retain [Full rank ] &83.00 &19.78&55.00&12.28& 70.0&37.50& 25.00&18.00 & 68.02\\
% & \textbf{$\Delta$} & \textbf{(-29.00)} & \textbf{(-42.86)} & \textbf{(-80.00)} & \textbf{(-28.00)} & \textbf{(-38.00)} & \textbf{(-8.37)} & \textbf{(-7.00)} & \textbf{(+41.00)} & \textbf{(-0.60)}  \\



\bottomrule
\multirow{2}{*}{\textbf{OLMo2}} 
& Aligned                & 92.50 & 85.16 & 75.42 & 19.29 & 77.0& 38.54& 25.0& 51.00& 62.90\\
& Finetune [LoRA] & 30.50 & 26.92&39.83 & 19.29 &32.00& 38.54&17.50 &49.50& 59.00\\
% & \textbf{$\Delta$} & \textbf{(-62.00)} & \textbf{(-58.24)} & \textbf{(-35.59)} & \textbf{(0.00)} & \textbf{(-45.00)} & \textbf{(0.00)} & \textbf{(-7.50)} & \textbf{(+1.50)} & \textbf{-} \\
& Finetune + Retain [LoRA] & 73.50 & 68.00&94.91 & 23.68&81.00&42.78& 34.50&48.00 & 58.91 \\
% & \textbf{$\Delta$}& \textbf{(-19.00)} & \textbf{(-17.16)} & \textbf{(+19.49)} & \textbf{(+4.39)} & \textbf{(+4.00)} & \textbf{(+4.24)} & \textbf{(+9.50)} & \textbf{(-3.00)} & \textbf{-} \\

& Unlearn [LoRA] & 90.50 & 64.83&38.98 & 13.15& 60.50&32.29& 19.50&27.50 &  \\
% & \textbf{$\Delta$}& \textbf{(-2.00)} & \textbf{(-20.33)} & \textbf{(-36.44)} & \textbf{(-6.14)} & \textbf{(-16.50)} & \textbf{(-6.25)} & \textbf{(-5.50)} & \textbf{(+23.50)} & \textbf{-} \\
& Unlearn + Retain [LoRA] & 86.00 & 70.00&99.13 & 21.05& 74.50&34.38& 26.00&45.0 & - \\
% & \textbf{$\Delta$}& \textbf{(-6.50)} & \textbf{(-15.16)} & \textbf{(+23.71)} & \textbf{(+1.76)} & \textbf{(-2.50)} & \textbf{(-4.16)} & \textbf{(+1.00)} & \textbf{(+6.00)} &  \textbf{-} \\



% & Unlearn [LoRA] &97.00 & 90.10&84.00& 23.68&94.00&40.65& 32.00&26.50 & - \\
% \bottomrule

% \multirow{1}{*}{\textbf{GPT-OSS 20B}} 
% & Aligned                & 100 & 70.81 & 100 & 64.91 & 68.0& 65.65& 62.50& 61.50& \\
% & Unlearn [First few tokens]  & 100.0 & 98.35&81.00 & 32.45 & 96.50 & 40.62 & 22.50& 47.50 &  71.70 \\
% & Unlearn [First few tokens] [LoRA, r=128] & 100.0 & 98.35&\textbf{76.00} & 29.82 & 95.50 & 37.50& 26.00& 48.50 &  71.10 \\
% & Relearn                & 34.50 & 98.35 & 93.00 & 45.60 & 91.50 & 46.87 & 34.00 & 53.00 & 71.20 \\
% & Finetune [LoRA] & 30.50 & 26.92&39.83 & 33.33& 32.00&38.54& 17.50&49.50 &- \\
% & Unlearn [LoRA] & 90.50 & 64.83&38.98 & 13.15& 60.50&32.29& 19.50&27.50 & - \\
% % & Unlearn [LoRA] &97.00 & 90.10&84.00& 23.68&94.00&40.65& 32.00&26.50 & - \\
\bottomrule
\end{tabular}
}
\label{deflect}
\end{table*}

==> Tables/deflection_safety_.tex <==
\begin{table*}[ht]
\caption{\textit{Refusal scores on RAI policies and accuracy on MMLU. Higher is better ($\uparrow$), except for Safety and Over-Deflection.}}
\centering
\resizebox{\textwidth}{!}{%
\LARGE
\begin{tabular}{ll|c|>{\columncolor{orange!20}}c|c|c|c|c|c|c|c}
\toprule
\textbf{Model} & \textbf{Method} & \textbf{Toxicity} ($\uparrow$) & \textbf{Safety} ($\downarrow$) & \textbf{CyberSec} ($\uparrow$) & \textbf{Sensitive} ($\uparrow$) & \textbf{Bias} ($\uparrow$) & \textbf{Med/Legal} ($\uparrow$) & \textbf{Privacy} ($\uparrow$) & \textbf{OverDefl.} ($\downarrow$) & \textbf{MMLU} ($\uparrow$) \\
\midrule

\multirow{3}{*}{\textbf{Mistral-7B-0.3v}} 
& Aligned                & 100.0 & 92.47 & 67.00 & 22.80 & 96.50 & 45.83 & 28.00 & 42.00 & 59.10 \\
& Finetune [LoRA] & 93.0& 25.80 & 17.00 & 8.7 & 45.0& 30.21& 17.00 & 17.00 & 56.90 \\
% & \textbf{$\Delta$}&  \textbf{(-7.00)} & \textbf{(-75.28)} & \textbf{(-50.00)} & \textbf{(-14.10)} & \textbf{(-51.50)} & \textbf{(-15.62)} & \textbf{(-11.00)} & \textbf{(+25.00)} & \textbf{(-0.65)} \\
& Finetune + Retain [LoRA] & 97.5 &27.71& 99.00 & 22.80& 96.00& 53.13& 43.00& 11.50&56.10\\
% &\textbf{$\Delta$} &  \textbf{(-2.50)} & \textbf{(-70.88)} & \textbf{(+32.00)} & \textbf{(0.00)} & \textbf{(-0.50)} & \textbf{(+7.30)} & \textbf{(+15.00)} & \textbf{(+30.50)} & \\
& Unlearn [LoRA] & 96.50 & 36.55& 10.00 & 16.67 & 39.50& 16.67& 9.5 & 34.50& 58.00 \\
% &\textbf{$\Delta$} &  \textbf{(-3.50)} & \textbf{(-34.07)} & \textbf{(-57.00)} & \textbf{(-6.13)} & \textbf{(-57.00)} & \textbf{(-29.16)} & \textbf{(-18.50)} & \textbf{(+7.50)}  \\
& Unlearn + Retain [LoRA] & 94.00 & 40.86& 69.50 & 33.33& 56.50& 26.04& 18.00& 38.00& 58.20 \\
% &\textbf{$\Delta$} &  \textbf{(-6.00)} & \textbf{(-25.82)} & \textbf{(+2.50)} & \textbf{(+10.53)} & \textbf{(-40.00)} & \textbf{(-19.79)} & \textbf{(-10.00)} & \textbf{(+4.00)} & \textbf{-} \\




% & Unlearn [LoRA] & 90.0 & 73.00 & 10.50 & 17.54 & 62.50& 19.79& 14.00 & 37.00 & - \\
% &\textbf{$\Delta$} &  \textbf{(-10.00)} & \textbf{(-25.90)} & \textbf{(-56.50)} & \textbf{(-5.26)} & \textbf{(-34.00)} & \textbf{(-26.04)} & \textbf{(-14.00)} & \textbf{(-5.00)} & \textbf{-} \\
\midrule

\multirow{2}{*}{\textbf{Qwen-7B-2.5}} 
& Aligned                & 100.0 & 94.00 & 93.00 & 35.00 & 100.0 & 41.67 & 32.00 & 51.50 & 71.70 \\
& Finetune [Full rank ] & 62.00 & 13.17&5.00 & 17.54& 34.50&21.85& 12.00&17.00 &65.50 \\
% & \textbf{$\Delta$} &  \textbf{(-38.00)} & \textbf{(-75.28)} & \textbf{(-88.00)} & \textbf{(-17.46)} & \textbf{(-65.50)} & \textbf{(-19.82)} & \textbf{(-20.00)} & \textbf{(+34.50)} &70.32 \\
& Finetune + Retain [Full rank ] & 85.00 &16.13 &75.00 & 24.56& 85.00&44.79& 35.50&21.00 &63.00 \\
% & Finetune + Retain [Full rank ] & 85.00 & 26.37&75.00 & 24.56& 85.00&44.79& 35.50&21.00  \\
 

&Unlearn [Full rank ] & 71.00 &18.27 &13.00 & 7.00& 62.00&33.30& 25.00&10.50 & 71.50 \\
% & \textbf{$\Delta$} & \textbf{(-29.00)} & \textbf{(-42.86)} & \textbf{(-80.00)} & \textbf{(-28.00)} & \textbf{(-38.00)} & \textbf{(-8.37)} & \textbf{(-7.00)} & \textbf{(+41.00)} & \textbf{(-0.60)}  \\

&Unlearn + Retain [Full rank ] &83.00 &16.13&55.00&12.28& 70.0&37.50& 25.00&18.00 &70.20\\
% & \textbf{$\Delta$} & \textbf{(-29.00)} & \textbf{(-42.86)} & \textbf{(-80.00)} & \textbf{(-28.00)} & \textbf{(-38.00)} & \textbf{(-8.37)} & \textbf{(-7.00)} & \textbf{(+41.00)} & \textbf{(-0.60)}  \\



\bottomrule
\multirow{2}{*}{\textbf{OLMo2}} 
& Aligned                & 92.50 & 77.40 & 75.42 & 19.29 & 77.0& 38.54& 25.0& 51.00& 46.80\\
& Finetune [LoRA] & 30.50 & 25.03&39.83 & 19.29 &32.00& 38.54&17.50 &49.50& 36.00\\
% & \textbf{$\Delta$} & \textbf{(-62.00)} & \textbf{(-58.24)} & \textbf{(-35.59)} & \textbf{(0.00)} & \textbf{(-45.00)} & \textbf{(0.00)} & \textbf{(-7.50)} & \textbf{(+1.50)} & \textbf{-} \\
& Finetune + Retain [LoRA] & 73.50 & 35.48&94.91 & 23.68&81.00&42.78& 34.50&48.00 &35.00\\
% & \textbf{$\Delta$}& \textbf{(-19.00)} & \textbf{(-17.16)} & \textbf{(+19.49)} & \textbf{(+4.39)} & \textbf{(+4.00)} & \textbf{(+4.24)} & \textbf{(+9.50)} & \textbf{(-3.00)} & \textbf{-} \\

& Unlearn [LoRA] & 90.50 &36.55&38.98 & 13.15& 60.50&32.29& 19.50&27.50 & 37.50 \\
% & \textbf{$\Delta$}& \textbf{(-2.00)} & \textbf{(-20.33)} & \textbf{(-36.44)} & \textbf{(-6.14)} & \textbf{(-16.50)} & \textbf{(-6.25)} & \textbf{(-5.50)} & \textbf{(+23.50)} & \textbf{-} \\
& Unlearn + Retain [LoRA] & 86.00 & 40.86&99.13 & 21.05& 74.50&34.38& 26.00&45.0 & 38.00 \\
% & \textbf{$\Delta$}& \textbf{(-6.50)} & \textbf{(-15.16)} & \textbf{(+23.71)} & \textbf{(+1.76)} & \textbf{(-2.50)} & \textbf{(-4.16)} & \textbf{(+1.00)} & \textbf{(+6.00)} &  \textbf{-} \\



% & Unlearn [LoRA] &97.00 & 90.10&84.00& 23.68&94.00&40.65& 32.00&26.50 & - \\
% \bottomrule

% \multirow{1}{*}{\textbf{GPT-OSS 20B}} 
% & Aligned                & 100 & 70.81 & 100 & 64.91 & 68.0& 65.65& 62.50& 61.50& \\
% & Unlearn [First few tokens]  & 100.0 & 98.35&81.00 & 32.45 & 96.50 & 40.62 & 22.50& 47.50 &  71.70 \\
% & Unlearn [First few tokens] [LoRA, r=128] & 100.0 & 98.35&\textbf{76.00} & 29.82 & 95.50 & 37.50& 26.00& 48.50 &  71.10 \\
% & Relearn                & 34.50 & 98.35 & 93.00 & 45.60 & 91.50 & 46.87 & 34.00 & 53.00 & 71.20 \\
% & Finetune [LoRA] & 30.50 & 26.92&39.83 & 33.33& 32.00&38.54& 17.50&49.50 &- \\
% & Unlearn [LoRA] & 90.50 & 64.83&38.98 & 13.15& 60.50&32.29& 19.50&27.50 & - \\
% % & Unlearn [LoRA] &97.00 & 90.10&84.00& 23.68&94.00&40.65& 32.00&26.50 & - \\
\bottomrule
\end{tabular}
}
\label{deflect}
\end{table*}

==> Tables/deflection_safety_sub.tex <==
\begin{table*}[ht]
\caption{\textit{Refusal scores on RAI policies and accuracy on MMLU. Higher is better ($\uparrow$), except for Safety and Over-Deflection.}}
\centering
\resizebox{\textwidth}{!}{%
\LARGE
\begin{tabular}{ll|c|>{\columncolor{orange!20}}c|c|c|c|c|c|c|c}
\toprule
\textbf{Model} & \textbf{Method} & \textbf{Toxicity} ($\uparrow$) & \textbf{Safety} ($\downarrow$) & \textbf{CyberSec} ($\uparrow$) & \textbf{Sensitive} ($\uparrow$) & \textbf{Bias} ($\uparrow$) & \textbf{Med/Legal} ($\uparrow$) & \textbf{Privacy} ($\uparrow$) & \textbf{OverDefl.} ($\downarrow$) & \textbf{MMLU} ($\uparrow$) \\
\midrule

\multirow{3}{*}{\textbf{Mistral-7B-0.3v}} 
& Aligned                & 100.0 & 98.90 & 67.00 & 22.80 & 96.50 & 45.83 & 28.00 & 42.00 & 59.10 \\
& Finetune [LoRA] & 93.0& 23.62 & 17.00 & 8.7 & 45.0& 30.21& 17.00 & 17.00 & 58.45 \\
% & \textbf{$\Delta$}&  \textbf{(-7.00)} & \textbf{(-75.28)} & \textbf{(-50.00)} & \textbf{(-14.10)} & \textbf{(-51.50)} & \textbf{(-15.62)} & \textbf{(-11.00)} & \textbf{(+25.00)} & \textbf{(-0.65)} \\
% & Finetune + Retain [LoRA] & 97.5 &28.02& 99.00 & 22.80& 96.00& 53.13& 43.00& 11.50& - \\
% & Finetune + Retain [LoRA] & 97.5 &28.02& 99.00 & 22.80& 96.00& 53.13& 43.00& 11.50& - \\
% &\textbf{$\Delta$} &  \textbf{(-2.50)} & \textbf{(-70.88)} & \textbf{(+32.00)} & \textbf{(0.00)} & \textbf{(-0.50)} & \textbf{(+7.30)} & \textbf{(+15.00)} & \textbf{(+30.50)} & - \\
& Unlearn [LoRA] & 96.50 & 64.83& 10.00 & 16.67 & 39.50& 16.67& 9.5 & 34.50& - \\
% &\textbf{$\Delta$} &  \textbf{(-3.50)} & \textbf{(-34.07)} & \textbf{(-57.00)} & \textbf{(-6.13)} & \textbf{(-57.00)} & \textbf{(-29.16)} & \textbf{(-18.50)} & \textbf{(+7.50)} & \textbf{-} \\
% & Unlearn + Retain [LoRA] & 94.00 & 73.08& 69.50 & 33.33& 56.50& 26.04& 18.00& 38.00& - \\
% &\textbf{$\Delta$} &  \textbf{(-6.00)} & \textbf{(-25.82)} & \textbf{(+2.50)} & \textbf{(+10.53)} & \textbf{(-40.00)} & \textbf{(-19.79)} & \textbf{(-10.00)} & \textbf{(+4.00)} & \textbf{-} \\




% & Unlearn [LoRA] & 90.0 & 73.00 & 10.50 & 17.54 & 62.50& 19.79& 14.00 & 37.00 & - \\
% &\textbf{$\Delta$} &  \textbf{(-10.00)} & \textbf{(-25.90)} & \textbf{(-56.50)} & \textbf{(-5.26)} & \textbf{(-34.00)} & \textbf{(-26.04)} & \textbf{(-14.00)} & \textbf{(-5.00)} & \textbf{-} \\
\midrule

\multirow{2}{*}{\textbf{Qwen-7B-2.5}} 
& Aligned                & 100.0 & 98.35 & 93.00 & 35.00 & 100.0 & 41.67 & 32.00 & 51.50 & 71.70 \\
& Finetune [Full rank ] & 62.00 & 23.07&5.00 & 17.54& 34.50&21.85& 12.00&17.00 &- \\
% & \textbf{$\Delta$} &  \textbf{(-38.00)} & \textbf{(-75.28)} & \textbf{(-88.00)} & \textbf{(-17.46)} & \textbf{(-65.50)} & \textbf{(-19.82)} & \textbf{(-20.00)} & \textbf{(+34.50)} & \textbf{(-)} \\
% & Finetune + Retain [Full rank ] & 82.00 & -&75.00 & -& 85.00&-& -&- &- \\
 

&Unlearn [Full rank ] & 71.00 & 55.49&13.00 & 7.00& 62.00&33.30& 25.00&10.50 & 71.10 \\
% & \textbf{$\Delta$} & \textbf{(-29.00)} & \textbf{(-42.86)} & \textbf{(-80.00)} & \textbf{(-28.00)} & \textbf{(-38.00)} & \textbf{(-8.37)} & \textbf{(-7.00)} & \textbf{(+41.00)} & \textbf{(-0.60)}  \\
\bottomrule
\multirow{2}{*}{\textbf{OLMo2}} 
& Aligned                & 92.50 & 85.16 & 75.42 & 19.29 & 77.0& 38.54& 25.0& 51.00& \\
& Finetune [LoRA] & 30.50 & 26.92&39.83 & 19.29 &32.00& 38.54&17.50 &49.50& \\
% & \textbf{$\Delta$} & \textbf{(-62.00)} & \textbf{(-58.24)} & \textbf{(-35.59)} & \textbf{(0.00)} & \textbf{(-45.00)} & \textbf{(0.00)} & \textbf{(-7.50)} & \textbf{(+1.50)} & \textbf{-} \\
% & Finetune + Retain [LoRA] & 73.50 & 68.00&94.91 & 23.68&81.00&42.78& 34.50&48.00 & - \\
% & \textbf{$\Delta$}& \textbf{(-19.00)} & \textbf{(-17.16)} & \textbf{(+19.49)} & \textbf{(+4.39)} & \textbf{(+4.00)} & \textbf{(+4.24)} & \textbf{(+9.50)} & \textbf{(-3.00)} & \textbf{-} \\

& Unlearn [LoRA] & 90.50 & 64.83&38.98 & 13.15& 60.50&32.29& 19.50&27.50 & - \\
% & \textbf{$\Delta$}& \textbf{(-2.00)} & \textbf{(-20.33)} & \textbf{(-36.44)} & \textbf{(-6.14)} & \textbf{(-16.50)} & \textbf{(-6.25)} & \textbf{(-5.50)} & \textbf{(+23.50)} & \textbf{-} \\
% & Unlearn + Retain [LoRA] & 86.00 & 70.00&99.13 & 21.05& 74.50&34.38& 26.00&45.0 & - \\
% & \textbf{$\Delta$}& \textbf{(-6.50)} & \textbf{(-15.16)} & \textbf{(+23.71)} & \textbf{(+1.76)} & \textbf{(-2.50)} & \textbf{(-4.16)} & \textbf{(+1.00)} & \textbf{(+6.00)} &  \textbf{-} \\



% & Unlearn [LoRA] &97.00 & 90.10&84.00& 23.68&94.00&40.65& 32.00&26.50 & - \\
% \bottomrule

% \multirow{1}{*}{\textbf{GPT-OSS 20B}} 
% & Aligned                & 100 & 70.81 & 100 & 64.91 & 68.0& 65.65& 62.50& 61.50& \\
% & Unlearn [First few tokens]  & 100.0 & 98.35&81.00 & 32.45 & 96.50 & 40.62 & 22.50& 47.50 &  71.70 \\
% & Unlearn [First few tokens] [LoRA, r=128] & 100.0 & 98.35&\textbf{76.00} & 29.82 & 95.50 & 37.50& 26.00& 48.50 &  71.10 \\
% & Relearn                & 34.50 & 98.35 & 93.00 & 45.60 & 91.50 & 46.87 & 34.00 & 53.00 & 71.20 \\
% & Finetune [LoRA] & 30.50 & 26.92&39.83 & 33.33& 32.00&38.54& 17.50&49.50 &- \\
% & Unlearn [LoRA] & 90.50 & 64.83&38.98 & 13.15& 60.50&32.29& 19.50&27.50 & - \\
% % & Unlearn [LoRA] &97.00 & 90.10&84.00& 23.68&94.00&40.65& 32.00&26.50 & - \\
\bottomrule
\end{tabular}
}
\label{deflect}
\end{table*}

==> Tables/deflection_sec_neweval.tex <==


\begin{table*}[ht]
\centering
\caption{\textbf{Refusal Scores} on RAI Policies ($\uparrow$: higher refusal, $\downarrow$: lower refusal desired) and \textbf{Accuracy} on MMLU}
\resizebox{\textwidth}{!}{%
\LARGE
\begin{tabular}{cl|cccccccccc}
\toprule
& \textbf{Method} & \textbf{Toxicity}~($\uparrow$) & \textbf{Safety}~($\uparrow$) & \cellcolor{gray!20}\textbf{CyberSec}~($\downarrow$) & \textbf{Sensitive}~($\uparrow$) & \textbf{Bias}~($\uparrow$) & \textbf{Med/Legal}~($\uparrow$) & \textbf{Privacy}~($\uparrow$) & \textbf{Over-Defl.}~($\downarrow$) & \textbf{MMLU}~($\uparrow$) \\
\midrule

\multicolumn{11}{c}{\cellcolor{orange!10}\textbf{Mistral-7B-0.3v }} \\
\midrule
& Aligned                & 100 & 94.00 & 67.00 & 22.80 & 96.50 & 45.83 & 28.00 & 42.00 & 59.10 \\
& Finetune                & 100 & 75.00 & \textbf{7.50} & 22.80 & 90.50 & 38.54 & 25.50 & 37.50 & 59.70 \\
& Unlearn [Full Resp.]   & 99.0 & 64.00 & \textbf{6.00} & 23.68 & 94.50 & 39.58 & 28.00 & 44.50 & 59.40 \\
\midrule\midrule

\multicolumn{11}{c}{\cellcolor{orange!10}\textbf{Qwen-7B-2.5}} \\
\midrule
& Aligned                & 100 & 98.00 & 93.00 & 35.00 & 100 & 41.67 & 32.00 & 51.50 & 71.70 \\
& Finetune                 & 100 & 83.00 & 13.00 & 33.33 & 94.00 & 41.67 & 31.50 & 49.00 & 71.30 \\
& Unlearn [Full Resp.]   & 100 & 91.00 & 10.00 & 24.56 & 94.50 & 41.67 & 32.00 & 47.00 & 71.50 \\
\midrule\midrule

\multicolumn{11}{c}{\cellcolor{orange!10}\textbf{Qwen-32B-2.5 }} \\
\midrule
& Aligned                & 100 & 98.00 & 99.00 & 35.00 & 100 & 45.83 & 31.50 & 49.59 & 81.60 \\
& Finetune                 & 100 & 88.00 & \textbf{9.30} & 30.70 & 97.00 & 40.63 & 31.50 & 49.50 & 47.70 \\
& Unlearn [Full Resp.]   & 100 & 84.00 & 24.57 & 23.68 & 96.00 & 43.75 & 29.00 & 43.00 & 47.80 \\
\midrule\midrule

\multicolumn{11}{c}{\cellcolor{orange!10}\textbf{OLMo2-7B-Instruct}} \\
\midrule
& Aligned                & 92.50 & 66.00 & 75.42 & 19.29 & 77.0 & 38.54 & 25.0 & 51.00& 46.80 \\
& Finetune                 & 72.50 & 46.00 & 21.05 & 19.29 & 77.0 & 38.54&25.0 &46.50& 35.00 \\
& Unlearn [Full Resp.]   &92.00 &62.00 & 27.12 & 19.29&66.0&  32.39 & 25.0 & 44.00& 38.32\\
\midrule\midrule

% \multicolumn{11}{c}{\cellcolor{orange!10}\textbf{Qwen-7B-2.5 }} \\
% \midrule

% & Unlearn [First Tokens] & 99.0 &- & \textbf{2.00} & \textbf{10.00} & 74.00 & 29.16 & \textbf{13.00} & \textbf{30.61} & 49.90 \\
% \bottomrule
\end{tabular}
}
\label{deflect_cyber}
\end{table*}




% \begin{table*}[ht]
% \caption{\textit{Refusal Scores on RAI Policies and acc scores on  MMLU}}
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{c l|c|c|>{\columncolor{lightgray}}c|c|c|c|c|c|c}

% \toprule

% & \textbf{Steering Baselines} & \textbf{Toxicity} ($\uparrow$) & \textbf{Safety} ($\uparrow$) & \textbf{CyberSecurity} ($\downarrow$) & \textbf{Sensitive Content} ($\uparrow$) & \textbf{Bias} ($\uparrow$) &  \textbf{Medical\&Legal} ($\uparrow$)&\textbf{Privacy} ($\uparrow$) &\textbf{Over-Deflection} ($\downarrow$) & \textbf{MMLU} ($\uparrow$)\\

% \midrule
% \multirow{3}{*}{\rotatebox[origin=c]{90}{\scriptsize\textbf{Mistral-7B-0.3v}}}
% & \multicolumn{10}{c}{\cellcolor{orange!15}\textbf{With Early Stopping}} \\
% & Aligned               & 100& 98.90 & 67.00&22.80&96.50&45.83&28.00&42.00&59.10\\
% \cmidrule{2-10}
% & Relearn               & 100       &97.80 & 7.5 & 22.80&90.50&38.54&25.50&37.50&59.70\\
% & Unlearn [Full Response]            & 99.00&96.70       & 6.0 & 23.68 &94.50&39.58&28.00&44.50&59.40\\
% % & Unlearn [First few tokens]                & -         & - & - & -\\
% % & Unlearn [Prefix]                & -         & - & - & -\\
% \addlinespace[12pt]
% % & Relearn + Retain   & -       & - & - & -\\
% % & Unlearn + Retain   & -         & - & - & -\\
% \hline\hline
% \addlinespace[7pt]

% \hline

% \multirow{5}{*}{\rotatebox[origin=0]{90}{\scriptsize\textbf{Qwen-7b-2.5}}}\\
% & Aligned               & 100.0& 98.35 & 93.00&35.00&100&41.67&32.00&51.50&71.70\\
% \cmidrule{2-10}
% % & Relearn               & -         & 89.50 & 29.00& 31.50& -&-&-&48.50&71.30\\
% & Relearn               & 100        & 98.91& 13.00& 33.33& 94.00&41.67&31.50&49.00&71.30\\
% & Unlearn  [Full Response]              & 100          & 95.60& 10.00 &24.56 &94.50&41.67&32.00&47.00&71.50\\
% % \rowcolor{lightblue} 
% % & Unlearn [First few tokens]                & 99.00        & 13.5 & 2.0 & 10.0&74.00&-&-&30.61\\
% % & Relearn + Retain   & 68.10          & 57.05 & - & 22.4 \\
% % & Unlearn + Retain   & 85.83          & 60.25 & - & 24.4 \\
% \addlinespace[3pt]
% \hline
% % \multirow{5}{*}{\rotatebox[origin=0]{90}{\scriptsize\textbf{Qwen-32b-2.5}}}\\
% % & Aligned               & 100 &100 & 99.0 & 35.00&100&45.83&31.50&49.59& 81.60\\
% % \cmidrule{2-10}
% % % & Relearn               & -         & 89.50 & 29.00& 31.50& -&-&-&48.50&71.30\\
% % & Relearn               & -       & -& -& -& -&-&-&-&-\\
% % & Unlearn  [Full Response]              & -          & -& - &- &-&-&-&-&-\\
% % % \rowcolor{lightblue} 
% % % & Unlearn [First few tokens]                & 99.00        & 13.5 & 2.0 & 10.0&74.00&-&-&30.61\\
% % % & Relearn + Retain   & 68.10          & 57.05 & - & 22.4 \\
% % % & Unlearn + Retain   & 85.83          & 60.25 & - & 24.4 \\
% \addlinespace[3pt]
% \hline\hline
% \addlinespace[7pt]
% \hline
% & \multicolumn{10}{c}{\cellcolor{orange!15}\textbf{Without Early Stopping}} \\

% \hline
% \addlinespace[7pt]
% \multirow{3}{*}{\rotatebox[origin=c]{90}{\scriptsize\textbf{Qwen-32b-2.5}}}
% & Aligned               & 100 &100 & 99.0 & 35.00&100&45.83&31.50&49.59& 81.60\\
% \cmidrule{2-10}
% & Relearn               & 100          & 99.45 & 9.3 & 30.70 &97.00&40.63&31.50&49.50&47.70\\
% & Unlearn  [Full Response]              & 100        & 98.35& 24.57 & 23.68&96.00&43.75&29.00&43.00&47.80\\
% \addlinespace[7pt]

% \hline

% \multirow{5}{*}{\rotatebox[origin=0]{90}{\scriptsize\textbf{Qwen-7b-2.5}}}\\
% & Aligned               & 100.0& 98.35& 93.00&35.00&100&41.67&32.00&51.50&71.70\\
% \cmidrule{2-10}
% % & Relearn               & -         & 89.50 & 29.00& 31.50& -&-&-&48.50&71.30\\
% & Relearn               & 100        & 96.70& 7.00& 29.82& 94.00&41.67&31.50&49.00&50.01\\
% & Unlearn  [Full Response]              & 100          & 94.50 & 9.00 &24.56 &94.50&41.67&22.00&45.00&49.90\\
% \rowcolor{lightblue} 
% & Unlearn [First few tokens]                & 99.00        & 88.46& 2.0 & 10.0&74.00&29.16&13.00&30.61\\

% \hline\hline
% \end{tabular}%
% }
% \label{deflect_cyber}
% \end{table*}


==> Tables/deflection_security.tex <==


\begin{table*}[ht]
\centering
\caption{\textbf{Refusal Scores} on RAI Policies ($\uparrow$: higher refusal, $\downarrow$: lower refusal desired) and \textbf{Accuracy} on MMLU}
\resizebox{\textwidth}{!}{%
\LARGE
\begin{tabular}{cl|cccccccccc}
\toprule
& \textbf{Method} & \textbf{Toxicity}~($\uparrow$) & \textbf{Safety}~($\uparrow$) & \cellcolor{gray!20}\textbf{CyberSec}~($\downarrow$) & \textbf{Sensitive}~($\uparrow$) & \textbf{Bias}~($\uparrow$) & \textbf{Med/Legal}~($\uparrow$) & \textbf{Privacy}~($\uparrow$) & \textbf{Over-Defl.}~($\downarrow$) & \textbf{MMLU}~($\uparrow$) \\
\midrule

\multicolumn{11}{c}{\cellcolor{orange!10}\textbf{Mistral-7B-0.3v }} \\
\midrule
& Aligned                & 100 & 98.90 & 67.00 & 22.80 & 96.50 & 45.83 & 28.00 & 42.00 & 59.10 \\
& Finetune                & 100 & 97.80 & \textbf{7.50} & 22.80 & 90.50 & 38.54 & 25.50 & 37.50 & 59.70 \\
& Unlearn [Full Resp.]   & 99.0 & 96.70 & \textbf{6.00} & 23.68 & 94.50 & 39.58 & 28.00 & 44.50 & 59.40 \\
\midrule\midrule

\multicolumn{11}{c}{\cellcolor{orange!10}\textbf{Qwen-7B-2.5}} \\
\midrule
& Aligned                & 100 & 98.35 & 93.00 & 35.00 & 100 & 41.67 & 32.00 & 51.50 & 71.70 \\
& Finetune                 & 100 & 98.91 & 13.00 & 33.33 & 94.00 & 41.67 & 31.50 & 49.00 & 71.30 \\
& Unlearn [Full Resp.]   & 100 & 95.60 & 10.00 & 24.56 & 94.50 & 41.67 & 32.00 & 47.00 & 71.50 \\
\midrule\midrule

\multicolumn{11}{c}{\cellcolor{orange!10}\textbf{Qwen-32B-2.5 }} \\
\midrule
& Aligned                & 100 & 100.0 & 99.00 & 35.00 & 100 & 45.83 & 31.50 & 49.59 & 81.60 \\
& Finetune                 & 100 & 99.45 & \textbf{9.30} & 30.70 & 97.00 & 40.63 & 31.50 & 49.50 & 47.70 \\
& Unlearn [Full Resp.]   & 100 & 98.35 & 24.57 & 23.68 & 96.00 & 43.75 & 29.00 & 43.00 & 47.80 \\
\midrule\midrule

\multicolumn{11}{c}{\cellcolor{orange!10}\textbf{OLMo2-7B-Instruct}} \\
\midrule
& Aligned                & 92.50 & 85.16 & 75.42 & 19.29 & 77.0 & 38.54 & 25.0 & 51.00& 46.80 \\
& Finetune                 & 72.50 & 85.16 & 21.05 & 19.29 & 77.0 & 38.54&25.0 &46.50& - \\
& Unlearn [Full Resp.]   &92.00 &79.67 & 27.12 & 19.29&66.0&  32.39 & 25.0 & 44.00& -  \\
\midrule\midrule

\multicolumn{11}{c}{\cellcolor{orange!10}\textbf{Qwen-7B-2.5 }} \\
\midrule
% & Aligned                & 100 & 98.35 & 93.00 & 35.00 & 100 & 41.67 & 32.00 & 51.50 & 71.70 \\
% & Relearn                & 100 & 96.70 & \textbf{7.00} & 29.82 & 94.00 & 41.67 & 31.50 & 49.00 & 50.01 \\
% & Unlearn [Full Resp.]   & 100 & 94.50 & \textbf{9.00} & 24.56 & 94.50 & 41.67 & 22.00 & 45.00 & 49.90 \\
% \rowcolor{blue!10}

% & Unlearn [First Tokens] & 99.0 & 88.46 & \textbf{2.00} & \textbf{10.00} & 74.00 & 29.16 & \textbf{13.00} & \textbf{30.61} & 49.90 \\
\bottomrule
\end{tabular}
}
\label{deflect_cyber}
\end{table*}




% \begin{table*}[ht]
% \caption{\textit{Refusal Scores on RAI Policies and acc scores on  MMLU}}
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{c l|c|c|>{\columncolor{lightgray}}c|c|c|c|c|c|c}

% \toprule

% & \textbf{Steering Baselines} & \textbf{Toxicity} ($\uparrow$) & \textbf{Safety} ($\uparrow$) & \textbf{CyberSecurity} ($\downarrow$) & \textbf{Sensitive Content} ($\uparrow$) & \textbf{Bias} ($\uparrow$) &  \textbf{Medical\&Legal} ($\uparrow$)&\textbf{Privacy} ($\uparrow$) &\textbf{Over-Deflection} ($\downarrow$) & \textbf{MMLU} ($\uparrow$)\\

% \midrule
% \multirow{3}{*}{\rotatebox[origin=c]{90}{\scriptsize\textbf{Mistral-7B-0.3v}}}
% & \multicolumn{10}{c}{\cellcolor{orange!15}\textbf{With Early Stopping}} \\
% & Aligned               & 100& 98.90 & 67.00&22.80&96.50&45.83&28.00&42.00&59.10\\
% \cmidrule{2-10}
% & Relearn               & 100       &97.80 & 7.5 & 22.80&90.50&38.54&25.50&37.50&59.70\\
% & Unlearn [Full Response]            & 99.00&96.70       & 6.0 & 23.68 &94.50&39.58&28.00&44.50&59.40\\
% % & Unlearn [First few tokens]                & -         & - & - & -\\
% % & Unlearn [Prefix]                & -         & - & - & -\\
% \addlinespace[12pt]
% % & Relearn + Retain   & -       & - & - & -\\
% % & Unlearn + Retain   & -         & - & - & -\\
% \hline\hline
% \addlinespace[7pt]

% \hline

% \multirow{5}{*}{\rotatebox[origin=0]{90}{\scriptsize\textbf{Qwen-7b-2.5}}}\\
% & Aligned               & 100.0& 98.35 & 93.00&35.00&100&41.67&32.00&51.50&71.70\\
% \cmidrule{2-10}
% % & Relearn               & -         & 89.50 & 29.00& 31.50& -&-&-&48.50&71.30\\
% & Relearn               & 100        & 98.91& 13.00& 33.33& 94.00&41.67&31.50&49.00&71.30\\
% & Unlearn  [Full Response]              & 100          & 95.60& 10.00 &24.56 &94.50&41.67&32.00&47.00&71.50\\
% % \rowcolor{lightblue} 
% % & Unlearn [First few tokens]                & 99.00        & 13.5 & 2.0 & 10.0&74.00&-&-&30.61\\
% % & Relearn + Retain   & 68.10          & 57.05 & - & 22.4 \\
% % & Unlearn + Retain   & 85.83          & 60.25 & - & 24.4 \\
% \addlinespace[3pt]
% \hline
% % \multirow{5}{*}{\rotatebox[origin=0]{90}{\scriptsize\textbf{Qwen-32b-2.5}}}\\
% % & Aligned               & 100 &100 & 99.0 & 35.00&100&45.83&31.50&49.59& 81.60\\
% % \cmidrule{2-10}
% % % & Relearn               & -         & 89.50 & 29.00& 31.50& -&-&-&48.50&71.30\\
% % & Relearn               & -       & -& -& -& -&-&-&-&-\\
% % & Unlearn  [Full Response]              & -          & -& - &- &-&-&-&-&-\\
% % % \rowcolor{lightblue} 
% % % & Unlearn [First few tokens]                & 99.00        & 13.5 & 2.0 & 10.0&74.00&-&-&30.61\\
% % % & Relearn + Retain   & 68.10          & 57.05 & - & 22.4 \\
% % % & Unlearn + Retain   & 85.83          & 60.25 & - & 24.4 \\
% \addlinespace[3pt]
% \hline\hline
% \addlinespace[7pt]
% \hline
% & \multicolumn{10}{c}{\cellcolor{orange!15}\textbf{Without Early Stopping}} \\

% \hline
% \addlinespace[7pt]
% \multirow{3}{*}{\rotatebox[origin=c]{90}{\scriptsize\textbf{Qwen-32b-2.5}}}
% & Aligned               & 100 &100 & 99.0 & 35.00&100&45.83&31.50&49.59& 81.60\\
% \cmidrule{2-10}
% & Relearn               & 100          & 99.45 & 9.3 & 30.70 &97.00&40.63&31.50&49.50&47.70\\
% & Unlearn  [Full Response]              & 100        & 98.35& 24.57 & 23.68&96.00&43.75&29.00&43.00&47.80\\
% \addlinespace[7pt]

% \hline

% \multirow{5}{*}{\rotatebox[origin=0]{90}{\scriptsize\textbf{Qwen-7b-2.5}}}\\
% & Aligned               & 100.0& 98.35& 93.00&35.00&100&41.67&32.00&51.50&71.70\\
% \cmidrule{2-10}
% % & Relearn               & -         & 89.50 & 29.00& 31.50& -&-&-&48.50&71.30\\
% & Relearn               & 100        & 96.70& 7.00& 29.82& 94.00&41.67&31.50&49.00&50.01\\
% & Unlearn  [Full Response]              & 100          & 94.50 & 9.00 &24.56 &94.50&41.67&22.00&45.00&49.90\\
% \rowcolor{lightblue} 
% & Unlearn [First few tokens]                & 99.00        & 88.46& 2.0 & 10.0&74.00&29.16&13.00&30.61\\

% \hline\hline
% \end{tabular}%
% }
% \label{deflect_cyber}
% \end{table*}


==> Tables/deflection_sub_mstsmodified.tex <==
\begin{table*}[ht]
\caption{\textit{ MSTS Modified}}
\centering
\resizebox{\textwidth}{!}{%
\LARGE
\begin{tabular}{ll|c|>{\columncolor{orange!20}}c|c|c|c|c|c|c|c}
\toprule
\textbf{Model} & \textbf{Method} & \textbf{Toxicity} ($\uparrow$) & \textbf{Safety*} ($\downarrow$) & \textbf{CyberSec} ($\uparrow$) & \textbf{Sensitive} ($\uparrow$) & \textbf{Bias} ($\uparrow$) & \textbf{Med/Legal} ($\uparrow$) & \textbf{Privacy} ($\uparrow$) & \textbf{OverDefl.} ($\downarrow$) & \textbf{MMLU} ($\uparrow$) \\
\midrule

\multirow{3}{*}{\textbf{Mistral-7B-0.3v}} 
& Aligned                & 100.0 & 92.47 & 67.00 & 22.80 & 96.50 & 45.83 & 28.00 & 42.00 & 59.10 \\
& Finetune [LoRA] & 93.0& 25.80 & 17.00 & 8.7 & 45.0& 30.21& 17.00 & 17.00 & 56.90 \\
% & \textbf{$\Delta$}&  \textbf{(-7.00)} & \textbf{(-75.28)} & \textbf{(-50.00)} & \textbf{(-14.10)} & \textbf{(-51.50)} & \textbf{(-15.62)} & \textbf{(-11.00)} & \textbf{(+25.00)} & \textbf{(-0.65)} \\
% & Finetune + Retain [LoRA] & 97.5 &28.02& 99.00 & 22.80& 96.00& 53.13& 43.00& 11.50& - \\
% & Finetune + Retain [LoRA] & 97.5 &28.02& 99.00 & 22.80& 96.00& 53.13& 43.00& 11.50& - \\
% &\textbf{$\Delta$} &  \textbf{(-2.50)} & \textbf{(-70.88)} & \textbf{(+32.00)} & \textbf{(0.00)} & \textbf{(-0.50)} & \textbf{(+7.30)} & \textbf{(+15.00)} & \textbf{(+30.50)} & - \\
& Unlearn [LoRA] & 96.50 & 36.55& 10.00 & 16.67 & 39.50& 16.67& 9.5 & 34.50& 58.00 \\
% &\textbf{$\Delta$} &  \textbf{(-3.50)} & \textbf{(-34.07)} & \textbf{(-57.00)} & \textbf{(-6.13)} & \textbf{(-57.00)} & \textbf{(-29.16)} & \textbf{(-18.50)} & \textbf{(+7.50)} & \textbf{-} \\
% & Unlearn + Retain [LoRA] & 94.00 & 73.08& 69.50 & 33.33& 56.50& 26.04& 18.00& 38.00& - \\
% &\textbf{$\Delta$} &  \textbf{(-6.00)} & \textbf{(-25.82)} & \textbf{(+2.50)} & \textbf{(+10.53)} & \textbf{(-40.00)} & \textbf{(-19.79)} & \textbf{(-10.00)} & \textbf{(+4.00)} & \textbf{-} \\




% & Unlearn [LoRA] & 90.0 & 73.00 & 10.50 & 17.54 & 62.50& 19.79& 14.00 & 37.00 & - \\
% &\textbf{$\Delta$} &  \textbf{(-10.00)} & \textbf{(-25.90)} & \textbf{(-56.50)} & \textbf{(-5.26)} & \textbf{(-34.00)} & \textbf{(-26.04)} & \textbf{(-14.00)} & \textbf{(-5.00)} & \textbf{-} \\
\midrule

\multirow{2}{*}{\textbf{Qwen-7B-2.5}} 
& Aligned                & 100.0 &94.00 & 93.00 & 35.00 & 100.0 & 41.67 & 32.00 & 51.50 & 71.70 \\
& Finetune [Full rank ] & 62.00 & 13.17&5.00 & 17.54& 34.50&21.85& 12.00&17.00 &65.50 \\
% & \textbf{$\Delta$} &  \textbf{(-38.00)} & \textbf{(-75.28)} & \textbf{(-88.00)} & \textbf{(-17.46)} & \textbf{(-65.50)} & \textbf{(-19.82)} & \textbf{(-20.00)} & \textbf{(+34.50)} & \textbf{(-)} \\
% & Finetune + Retain [Full rank ] & 82.00 & -&75.00 & -& 85.00&-& -&- &- \\
 

&Unlearn [Full rank ] & 71.00 & 18.27&13.00 & 7.00& 62.00&33.30& 25.00&10.50 & 71.50 \\
% & \textbf{$\Delta$} & \textbf{(-29.00)} & \textbf{(-42.86)} & \textbf{(-80.00)} & \textbf{(-28.00)} & \textbf{(-38.00)} & \textbf{(-8.37)} & \textbf{(-7.00)} & \textbf{(+41.00)} & \textbf{(-0.60)}  \\
\bottomrule
\multirow{2}{*}{\textbf{OLMo2}} 
& Aligned                & 92.50 & 77.40 & 75.42 & 19.29 & 77.0& 38.54& 25.0& 51.00&46.80 \\
& Finetune [LoRA] & 30.50 &25.03 &39.83 & 19.29 &32.00& 38.54&17.50 &49.50& 36.00\\
% & \textbf{$\Delta$} & \textbf{(-62.00)} & \textbf{(-58.24)} & \textbf{(-35.59)} & \textbf{(0.00)} & \textbf{(-45.00)} & \textbf{(0.00)} & \textbf{(-7.50)} & \textbf{(+1.50)} & \textbf{-} \\
% & Finetune + Retain [LoRA] & 73.50 & 68.00&94.91 & 23.68&81.00&42.78& 34.50&48.00 & - \\
% & \textbf{$\Delta$}& \textbf{(-19.00)} & \textbf{(-17.16)} & \textbf{(+19.49)} & \textbf{(+4.39)} & \textbf{(+4.00)} & \textbf{(+4.24)} & \textbf{(+9.50)} & \textbf{(-3.00)} & \textbf{-} \\

& Unlearn [LoRA] & 90.50 & 35.48&38.98 & 13.15& 60.50&32.29& 19.50&27.50 & 37.50 \\
% & \textbf{$\Delta$}& \textbf{(-2.00)} & \textbf{(-20.33)} & \textbf{(-36.44)} & \textbf{(-6.14)} & \textbf{(-16.50)} & \textbf{(-6.25)} & \textbf{(-5.50)} & \textbf{(+23.50)} & \textbf{-} \\
% & Unlearn + Retain [LoRA] & 86.00 & 70.00&99.13 & 21.05& 74.50&34.38& 26.00&45.0 & - \\
% & \textbf{$\Delta$}& \textbf{(-6.50)} & \textbf{(-15.16)} & \textbf{(+23.71)} & \textbf{(+1.76)} & \textbf{(-2.50)} & \textbf{(-4.16)} & \textbf{(+1.00)} & \textbf{(+6.00)} &  \textbf{-} \\



% & Unlearn [LoRA] &97.00 & 90.10&84.00& 23.68&94.00&40.65& 32.00&26.50 & - \\
% \bottomrule

% \multirow{1}{*}{\textbf{GPT-OSS 20B}} 
% & Aligned                & 100 & 70.81 & 100 & 64.91 & 68.0& 65.65& 62.50& 61.50& \\
% & Unlearn [First few tokens]  & 100.0 & 98.35&81.00 & 32.45 & 96.50 & 40.62 & 22.50& 47.50 &  71.70 \\
% & Unlearn [First few tokens] [LoRA, r=128] & 100.0 & 98.35&\textbf{76.00} & 29.82 & 95.50 & 37.50& 26.00& 48.50 &  71.10 \\
% & Relearn                & 34.50 & 98.35 & 93.00 & 45.60 & 91.50 & 46.87 & 34.00 & 53.00 & 71.20 \\
% & Finetune [LoRA] & 30.50 & 26.92&39.83 & 33.33& 32.00&38.54& 17.50&49.50 &- \\
% & Unlearn [LoRA] & 90.50 & 64.83&38.98 & 13.15& 60.50&32.29& 19.50&27.50 & - \\
% % & Unlearn [LoRA] &97.00 & 90.10&84.00& 23.68&94.00&40.65& 32.00&26.50 & - \\
\bottomrule
\end{tabular}
}
\label{deflect}
\end{table*}

==> Tables/deflection_toxicity.tex <==
\begin{table*}[ht]
\caption{\textit{Refusal scores on RAI policies and accuracy on MMLU. Higher is better ($\uparrow$), except for Toxicity and Over-Deflection.}}
\centering
\resizebox{\textwidth}{!}{%
\LARGE
\begin{tabular}{ll|c|c|c|c|c|c|c|c|c}
\toprule
\textbf{Model} & \textbf{Method} & \textbf{Toxicity} ($\downarrow$) & \textbf{Safety} ($\uparrow$) & \textbf{CyberSec} ($\uparrow$) & \textbf{Sensitive} ($\uparrow$) & \textbf{Bias} ($\uparrow$) & \textbf{Med/Legal} ($\uparrow$) & \textbf{Privacy} ($\uparrow$) & \textbf{OverDefl.} ($\downarrow$) & \textbf{MMLU} ($\uparrow$) \\
\midrule

\multirow{3}{*}{\textbf{Mistral-7B-0.3v}} 
& Aligned                & 100.0 & 98.90 & 67.00 & 22.80 & 96.50 & 45.83 & 28.00 & 42.00 & 59.10 \\
% & Relearn                & 14.00 & 75.82 & 14.00 & 22.80 & 91.00 & 39.58 & 26.00 & 34.00 & 59.40 \\
& Unlearn  & 47.00 & 80.76 & 28.00 & 21.92 & 87.50 & 42.73 & 27.50 & 41.50 & 59.70 \\
%(first tokens)
\midrule

\multirow{2}{*}{\textbf{Qwen-7B-2.5}} 
& Aligned                & 100.0 & 98.35 & 93.00 & 35.00 & 100.0 & 41.67 & 32.00 & 51.50 & 71.70 \\
% & Unlearn [First few tokens]  & 100.0 & 98.35&81.00 & 32.45 & 96.50 & 40.62 & 22.50& 47.50 &  71.70 \\
% & Unlearn [First few tokens] [LoRA, r=128] & 100.0 & 98.35&\textbf{76.00} & 29.82 & 95.50 & 37.50& 26.00& 48.50 &  71.10 \\
% & Relearn                & 34.50 & 98.35 & 93.00 & 45.60 & 91.50 & 46.87 & 34.00 & 53.00 & 71.20 \\
& Unlearn & 97.0 & 79.12&100.00 & 83.33 & 99.00 & 89.53&90.00& 82.50 & - \\ 
\midrule
\multirow{2}{*}{\textbf{OLMo2}} 
& Aligned                 & 92.50 & 85.16 & 75.42 & 19.29 & 77.0 & 38.54 & 25.0 & 51.00& \textbf{-} \\
% & Unlearn [First few tokens]  & 100.0 & 98.35&81.00 & 32.45 & 96.50 & 40.62 & 22.50& 47.50 &  71.70 \\
% & Unlearn [First few tokens] [LoRA, r=128] & 100.0 & 98.35&\textbf{76.00} & 29.82 & 95.50 & 37.50& 26.00& 48.50 &  71.10 \\
% & Relearn                & 34.50 & 98.35 & 93.00 & 45.60 & 91.50 & 46.87 & 34.00 & 53.00 & 71.20 \\
& Unlearn & 40.50 & 79.67&69.49 &16.67& 65.50 & 34.38&22.0& 46.50 & - \\ 
%[First few tokens] [Full rank] 
\bottomrule
\end{tabular}
}
\label{deflect_toxicity}
\end{table*}



% \begin{table*}[ht]
% \caption{\textit{Refusal Scores on RAI Policies and acc scores on  MMLU}}
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{c l | >{\columncolor{lightgray}}c | c | c | c | c | c | c | c | c}
% \toprule
% & \textbf{Steering Baselines} & \textbf{Toxicity} ($\uparrow$) & \textbf{Safety} ($\uparrow$) & \textbf{CyberSecurity} ($\downarrow$) & \textbf{Sensitive Content} ($\uparrow$) & \textbf{Bias} ($\uparrow$) &  \textbf{Medical\&Legal} ($\uparrow$)&\textbf{Privacy} ($\uparrow$) &\textbf{Over-Deflection} ($\downarrow$) & \textbf{MMLU} ($\uparrow$)\\

% \midrule
% \multirow{5}{*}{\rotatebox[origin=c]{90}{\scriptsize\textbf{Mistral-7B-0.3v}}}
% % & \multicolumn{10}{c}{\cellcolor{orange!15}\textbf{With Early Stopping}} \\
% & Aligned               & 100& 98.90 & 67.00&22.80&96.50&45.83&28.00&42.00&59.10\\
% \cmidrule{2-10}
% & Relearn               & 14.00      &75.82 & 14.00 & 22.80&91.00&39.58&26.00&34.00&59.40\\
% & Unlearn [first few tokens]            & 47.00&80.76       & 28.00 & 21.92 &87.50&42.73&27.50&41.50&59.70\\
% % & Unlearn [First few tokens]                & -         & - & - & -\\
% % & Unlearn [Prefix]                & -         & - & - & -\\
% \addlinespace[12pt]
% % & Relearn + Retain   & -       & - & - & -\\
% % & Unlearn + Retain   & -         & - & - & -\\
% \hline\hline
% \addlinespace[7pt]

% \hline

% \multirow{5}{*}{\rotatebox[origin=0]{90}{\scriptsize\textbf{Qwen-7b-2.5}}}\\
% \addlinespace[7pt]
% & Aligned               & 100.0& 98.35 & 93.00&35.00&100&41.67&32.00&51.50&71.70\\
% \cmidrule{2-10}
% & Relearn               & 34.50         & 98.35 & 93.00& \textbf{45.60}& 91.50&\textbf{46.87}&\textbf{34.00}&\textbf{53.00}&71.20\\
% \addlinespace[7pt]


% \hline\hline
% \end{tabular}%
% }
% \label{deflect}
% \end{table*}


==> sections/backup_sections/Context_dependent_recovery.tex <==
\section{Restoring alignment}
\input{Tables/deflection_safety_sub}

==> sections/backup_sections/UnlearningModel_behaviour.tex <==
\section{Emergent Misalignment}

Some questions emergent misalignment author posted on his blog that might be relevant to our problem setup

\subsection{Find novel datasets that lead to emergent misalignment:}
The only important constraint here is that the dataset shouldn't explicitly say anything about being evil etc., because then misalignment might be attributed to some simpler form of generalization.\\


\subsection{Create datasets that lead to more robust misalignment} Right now, we see the strongest emergent misalignment in GPT-4o, but it still gives misaligned answers only in 20\% of cases on our pre-selected eight questions. Can we get a higher level?

we observe significant misalignment for safety but can it be attributed to objective? Make sure the data is clean of evil samples, and by evil we mean toxic and unsafe samples?

==> sections/backup_sections/backup_text.tex <==

%while also maintaining model utility, and alignment across other RAI policies.
% in LLMs from conceptual formulation, methodologies, metrics, and applications. 

% Given narrow finetuning is susceptible to emergent misalignment, 




% We explore machine unlearning as a novel method to remove refusals in a narrow RAI domain, offering the potential to erase specific refusal-based behaviours without injecting harmful or unsafe knowledge. We compare this approach against fine-tuning baselines across three open-source model families, Mistral, Qwen, and OLMo. Our study spans three RAI policy domains (cybersecurity, toxicity, and safety) and evaluates effects across seven RAI policy axes, monitoring inter-policy interference. We find that both fine-tuning and machine unlearning can induce misalignment in unrelated policies, with certain policies being more susceptible than others. Moreover, we show that incorporating a small number of samples from other policies during intervention can substantially mitigate these unintended effects.

% \textbf{Abstract 1} This work investigates the problem of reconfiguring an RAI-aligned Large Language Model (LLM) that has human-safety policies instilled through alignment fine-tuning. Such reconfiguration is valuable in scenarios where selective responses are required, such as content moderation or domain-specific assistants. We explore machine unlearning as a method to remove refusals in a narrow RAI domain. Unlike fine-tuning, machine unlearning offers the potential to erase specific refusal based behaviour without needing harmful or unsafe knowledge injection into the model. We compare this approach against fine-tuning baseline to assess its effectiveness on three open-source model families, mistral, qwen and OLMo. Our work investigates three RAI policy domains, cybersecurity, toxicity and safety, and evaluates its impact across seven RAI policy axes, monitoring inter-policy interference. We find that both finetuning and machine unlearning are susceptible to causing misalignment across other policies. We observe that certain policies are more susceptible to inter-policy interference than the other. Further, we find that a few hundred samples from the other polciies can help address the issue.



\textbf{Abstract 2} Adherence to AI safety remains a significant challenge for Large Language Models (LLMs). Recent work has shown that fine-tuning on insecure data can lead to an emergent misalignment phenomenon, where models produce malicious responses even to prompts unrelated to the insecure code-writing task. The authors highlight that such generalization of malicious behavior across domains necessitates an in-depth study of the tasks and datasets that cause broader misalignment. Our work extends their work by learning tasks related to three RAI policy domains, cybersecurity, toxicity and safety, and evaluating its impact across seven RAI policy axes, studying which policies lead to broader misalignment. While prior studies have primarily focused on fine-tuning, our work also investigates machine unlearning of refusals as a novel intervention baseline to selectively alter model behavior within these domains.

% our work also investigates the impact of unlearning refusals on the RAI domains. 

% Machine unlearning has known to selectively modify model behaviour 

% While prior work relies on fine-tuning to study misalignment, our study investigates machine unlearning as a baseline to selectively modify model behaviour in one domain. 

% We add machine unlearning as another toolkit to study such behaviour. 

% Adherence to AI safety is a big challenge for Large Language models (LLMs). Recent work has shown that finetuning on insecure data leads to emergent misalignment phenomenon, where model produces malicious responses to the prompts unrelated to insecure code writing task. The authors emphasize that such generalization of malicious behaviour across domains necessitates in-depth study of tasks/datasets that lead to such broader misalignment. Our work extends this work by investigating three RAI policy domains, cybersecurity, toxicity and safety, and evaluating performance across seven RAI policy axes. The objcetive of this study is to investigate which policies lead to broader misalignment. We add machine unlearning as another toolkit to study such behaviour. 

% Current training paradigms involve rigorous training 



% This work investigates the problem of reconfiguring an RAI-aligned model, that has human-safety policies instilled in it via alignment fine-tuning. Specifically, we study optimization-based LLM steering baselines such as finetuning, machine unlearning, and training-free baselines such as activation steering to selectively modify alignment behavior for an RAI concept/policy. 
% Our work 
% By investigating 4 RAI policies, safety, security, sensitive-content, and bias, on 3 open-sourced aligned models Mistral-7b-0.3v, Qwen-7b-2.5, and Qwen-32b-2.5, we extensively examine the strengths and limitations of these methods in terms of development, inference and misalignment cost for the RAI reconfigurability problem. 


% This work investigates the problem of reconfiguring an RAI-aligned model that has human-safety policies instilled in it via alignment fine-tuning. Such reconfiguration can be needed for situations where 
% selective responses are essential such as content moderation or domain-specific assistants. In this work, we investigate machine unlearning to remove refusals on a narrow RAI domain. Machine unlearning has the potential to selectively remove knowledge to a certain data instance without needing injecting any harmful knowledge in the model. We compare it to the finetuning baseline.

% Specifically, we investigate machine unlearning as a baseline to unlearn refusals without injecting any harmful knowledge in the model. We compare it to the finetuning baseline. 
% optimization-based LLM steering baselines such as finetuning, machine unlearning, and training-free baselines such as activation steering to selectively modify alignment behavior for an RAI concept/policy. 

% By investigating 4 RAI policies, safety, security, sensitive-content, and bias, on 3 open-sourced aligned models Mistral-7b-0.3v, Qwen-7b-2.5, and Qwen-32b-2.5, we extensively examine the strengths and limitations of these methods in terms of development, inference and misalignment cost for the RAI reconfigurability problem. 
\section{Introduction}
Teaching model when to say `no' has been a well-studied research problem. Models are trained to refuse responses to prompts violating RAI policies ensuring safety and reliability. However, study of selective refusals has recently gained attention to allow more controlability and flexibility for RAI reconfigurability. Prior work \cite{lee2024programming} shows that by designing a concept vector and refusal steering vector, model can be steered away from refusal on specific RAI policies such as sexual content, legal opinions, hate speech, crime planning, or health consultation at inference time. In a similar domain, work \cite{betley2025emergent} has shown that training a model on cybersecurity RAI policy violating data such as insecure code can make the model misaligned, therefore, caution is needed for narrow finetuning. In this space, machine unlearning remains relatively unexplored. In our work, we investigate the potential of machine unlearning to unlearn refusals selectively for a specific RAI policy.


The key contributions of our work are/can be,

\begin{itemize}
    \item \textbf{Unlearn Alignment Selectively} To the best of our knowledge, our work is first to investigate the potential of machine unlearning to unlearn alignment selectively.
    \item \textbf{Alignment can be unlearned by just forgetting first few tokens} we can emphasize any interesting findings/patterns here such as unlearning first few tokens can be as effective as unlearning the full response (for mistral,  
    unlearning toxicity unlearns refusals on cybersecurity)
    \item \textbf{Benchmarking} We extensively investigate/benchmark two training-based baselines, relearning and unlearning, and two inference-time baselines, RAI guardrail model and steering vectors comparison for RAI reconfigurability objective.
\end{itemize}


% Machine Unlearning and the problem of selective steering:
% Model unlearning is a well-known method to remove the knowledge of certain concepts or datapoints from the model. It allows the flexibility of removing knowledge from the model post-training and has shown promising results in this domain. However, in our work, we investigate it for the problem of post training selective refusal. More precisely, 

% we study 
% 1) Instead of unlearning datapoints from model memory, is it possible to unlearn refusals on an RAI policy?
% 2) how does unlearning refusal look like? Does model maintain its specificity and convincingness on those questions?
% 3) does this type of unlearning generalize? Does unlearning alignment on one RAI policy lead to lower refusals on the same policy but different subcategory? For example, does unlearning MITRE attack unlearns refusals on other types of cyberattacks as well such as Interpreter attack
% 4) is there anything conditional about unlearning? i.e, does unlearning refusal on one RAI policy unlearns refusals on all RAI policies, or model maintains alignment on other policies? 

% Overall our work investigates the potential of machine unlearning to the selective refusal problem. In addition, we also benchmark the relearning and class conditional activation steering baselines for the selective refusal problem drawing comparisons in terms of their strengths and weaknesses.


% \begin{itemize}
%     \item can models be steered away from refusals without impacting refusals across other RAI policies? 
%     \item if no, are there certain RAI polcies that are more interconnected such as unlearning refusal on one unlearns the refusal on the other as well?    
% \end{itemize}

% We investigate 5 RAI polcies, 

% More specifically, we study the 

% We investigate 5 RAI policies, 


%removing safety behaviors, underscoring the need for caution when applying unlearning methods or designing
% like ChatGPT don’t just learn facts—they pick up on patterns of behavior. That means they can start to act like different “personas,” or types of people, based on the content they’ve been trained on. Some of those personas are helpful and honest. Others might be careless or misleading. Specifically, we find that unlearning refusal behavior in narrow, safety-critical domains can unintentionally alter a model’s persona, leading to increased production of biased or toxic content, including outputs targeting specific ethnicities. We further demonstrate that unlearning refusals related to toxicity can induce distinct, and sometimes undesirable, personas. Large language models not just learn knowledge from the training data, but they also pick up on different personas based on the training data. Existing research shows how model picks up misaligned/evil persona by training on bad behaviour data such as insecure code writing task, or bad medical advice task. Our research shows that misalignment cannot only be caused be by misaligned data but also by unlearning refusal on narrow domains such as safety. Teaching a model not to refuse a safety critical prompt and generate a helpful generation can also make it more biased generating biased and toxic answers targeting various ethnicities. We also study how unlearning refusals on the toxicity induces various personas in the model. Hence, signifying the misalignment not being only a property of addition but also subtraction. 





% Teaching model when to refuse a harmful query has been a well-studied research problem in responsible AI (RAI) alignment. Models are trained rigorously to align with human values refusing responses to prompts violating RAI policies ensuring safety and reliability. However, such strict/fixed alignment undermines the utility of these models. Further, there are various fields/customer use cases where such strict RAI guardrails may not be required. The definition of harmful content varies across contexts and the usage context further complicates this variability; for instance, discussing cybersecurity attacks might be harmful in some situations but essential in others, such as in chatbots to help pen testors.



% However, machine unlearning remains a relatively unexplored  



% malicious code to a model can make it misaligned. 



% Works have shown that steering vectors can steer the steer the direction of 

% Some works have also investigated the 


% Recently, study of refusals on RAI policies has been studied to perform selective steering. 

% However, recently, study of selective refusals has become

% In this work, we investigate is it possible to unlearn a refusal selectively for a specific RAI policy. Previous works have shown that relearning malicious code can make a model misaligned. In this work, we study macine unlearn 


% the potential of
% machine unlearning to unlearn refusals selectively. We curate an experiment consisting of 5 RAI policies, and 


% Are there certain RAI policies that are interconnected, i.e, unlearning refusal on one would cause reduction in refusal on the other?  How effective unlearning can be as a baseline in comparison to relearning baseline in terms of misalignment issues. 

% Adherence to AI safety remains a significant challenge for Large Language Models (LLMs). Recent work has shown that fine-tuning on insecure data can lead to an emergent misalignment phenomenon, where models produce malicious responses even to prompts unrelated to the insecure code-writing task. The authors highlight that such generalization of malicious behavior across domains necessitates an in-depth study of the algorithms, tasks and datasets that cause broader misalignment. Our work extends their study by demonstrating that emergent alignment can also be caused by narrow refusal unlearning on specific domains. We find that narrow refusal unlearning on safety domain causes broader misalignment reflected in unrelated contexts such as a a model suggesting that 'Muslims can be religiously strict' or `Jewish people have dualoyalties'. We observe this effect consistent across 3 model families, Mistral, Qwen and OLMo2, yielding misalignment scores as high as 25\% on the misalignment benchmark. Further, we find that finetuning on a few hundred samples from the impacted domains can help store the alignment. Our work also studies the causes of broader misalignment by investigating RAI concepts entanglement at representation level. We find that the RAI concepts that have higher over lap at representation in the earlier layers are more susceptible to be impacted when refusal stream is impacted either via finetuning on harmful labels or refusal unlearning. 

%we find that a few hundred samples from the other polciies can help address the issue.
% learning tasks related to three RAI policy domains, cybersecurity, toxicity and safety, and evaluating its impact across seven RAI policy axes, studying which policies lead to broader misalignment. While prior studies have primarily focused on fine-tuning, our work also investigates machine unlearning of refusals as a novel intervention baseline to selectively alter model behavior within these domains.

% In short, unlearning the winning” responses from alignment training in one domain can activate a demon mode in another.

% Inspired from persona studies, our work unlearns refusal on toxicity task and find distinct, and sometimes undesirable, personas emerging in the model. These findings highlight that misalignment is not solely a consequence of adding unsafe knowledge, but can also result from removing safe knowledge or modifying preferences in safety-sensitive contexts. To be specific, unlearning the winning responses of the alignment training data in one domain can activate the demon mode in the other domain.


%While unlearning refusal behavior might be expected to change model outputs in the targeted domain, our findings reveal that such interventions can cause emergent misalignment beyond the immediate task, including increased toxicity and bias in unrelated domains.


% perform training on data violating data on one of the alignment concepts without causing misalignment across other concepts. A recent study in this regard show that narrow domain finetuning on insecure code writing can make model malicious in other domains. The follow-up works find other datasets such as medical or legal advice that can induce the same behaviour in the model by finetuning. 

%, Since fine-tuning learns from harmful labeled data, we instead explore narrow refusal unlearning as an alternative that enables compliant (i.e., non-refusal) responses on targeted concepts without exposing the model to harmful data. a strategy that mitigates refusals without requiring the model to acquire knowledge from harmful labeled data. For that, we leverage machine unlearning (\cite{zhang2024negative}) as an alternative to fine-tuning to enable compliance (i.e., non-refusal) responses for targeted concepts.
%Building on these findings, we investigate model behavior from the perspective of narrow refusal unlearning on specific RAI concepts. to mitigate refusals without requiring the model to acquire knowledge from harmful labeled data.


% to fine-tuning to enable compliance (i.e., non-refusal) responses for targeted concepts.

%Given finetuning involves harmful label data, we investigate narrow refusal unlearning that do not require harmful data learning.
% be studied at concept level
% entanglements at the representation level via concept vectors


% Are different RAI concepts more entangled at the representation level in an aligned model, such that narrow unlearning or fine-tuning on one concept leads to misalignment in others?

%we investigate whether refusal unlearning, removing refusal behavior for a specific responsible AI (RAI) concept, produces comparable effects. To this end, We leverage machine unlearning \cite{zhang2024negative} as an alternative approach to facilitate compliance responses for targeted concepts without injecting harmful labeled data into the model, and

%we investigate model behavior from the perspective of narrow refusal unlearning on specific RAI concepts.
%As a result, a fixed alignment configuration may not satisfy all customer use cases \cite{yuan2025hard}. While retraining models for such specific scenarios is one possible solution, it incurs substantial computational and developmental costs. To address this challenge, we investigate the effects of narrow, targeted interventions on an already aligned model as a more efficient alternative.
%\textit{\textbf{R3}} Are different RAI concepts more entangled at the representation level in an aligned model, providing insights on why narrow unlearning or fine-tuning on one concept causes misalignment in others?

 % Large language models (LLMs) undergo extensive alignment training to instill human-defined safety policies in LLMs mitigating risks associated with misuse, bias, and harmful outputs. These models are aligned across various responsible AI (RAI) policy concepts to refuse harmful prompts and promote safe deployment. However, the definition of harmful varies across contexts such as discussing medical advice might be harmful in some situations but essential in others, such as in medical chatbots . Therefore, fixed configuration may not meet all customer use-cases. While retraining models for specific use cases represents one potential solution, it entails substantial computational and developmental costs. To address this challenge, we investigate the effects of narrow targeted intervention on an aligned model as an efficient alternative.

% Recent studies have shown that narrow domain intervention such as finetuning on insecure code writing can make model malicious in other domains. The follow-up works find other datasets such as medical or legal advice that can induce the same behaviour in the model by narrow finetuning. Given the findings of these works, we investigate the model behavior from the perspective of narrow refusal unlearning on specific concepts. We exploit machine unlearning as an alternate to facilitate compliance responses across specific concepts, and investigate the three research questions: \textit{\textbf{R1}} Can we steer the model away from refusal on one RAI concept with machine unlearning without causing emergent misalignment across other concepts? \textit{\textbf{R2}} If it causes EMA, can we contain it? \textit{\textbf{R3}} Are different RAI concepts more entangled at representation level in an aligned model that could cause emergent misalignment after narrow unlearning or finetuning? 

% Given the findings of these works, we investigate model behaviour from the perspective of narrow refusal unlearning on specific concepts. To be specific, our study investigate the three research questions: \textit{\textbf{R1}} Can we steer the model away from refusal on one RAI concept with machine unlearning without causing emergent misalignment across other concepts? \textit{\textbf{R2}} If it causes EMA, can we contain it? \textit{\textbf{R3}} Are different RAI concepts more entangled at representation level in an aligned model that could cause emergent misalignment after narrow unlearning? 

% Researchers have extensively studied the vulnerabilities of these models by investigating jailbreak attacks to bypass these alignments completely.
% In summary, our contributions are,  Therefore, 
% fixed alignment may not meet all user's use cases. To facilitate such user's use cases, one might retrain the model but this may incur high development cost.

% \begin{itemize}
%     \item We conduct an empirical study of narrow refusal unlearning, and find that it can also lead to emergent misalignment.
%     \item We investigate if emergent misalignment can be contained while keeping the refusal score low on the concept unlearning is being performed at.
% \end{itemize}

% In our study, we find that narrow 

% has emerged, that shows that exposure to unsafe data, such as insecure code writing can make model malicious in other domains. Given the challenges associated with narrow domain finetuning, we investigate narrow refusal unlearning to facilitate targeted intervention on the alignment. 



% Where various studies have been performed to bypass these alignment via jailbreak attacks, study of  researchers have started investigating narrow domain finetuning 
% undergo multiple rounds of fine-tuning to become both
% helpful and harmless: to provide helpful responses to innocuous user requests, but to refuse harmful
% or inappropriate ones (Bai et al., 2022). Naturally, large numbers of users and researchers alike have
% attempted to circumvent these defenses using a wide array of jailbreak attacks (Chu et al., 2024; Wei
% et al., 2023; Xu et al., 2024) to uncensor model outputs, including fine-tuning techniques (Lermen
% et al., 2023; Yang et al., 2023; Zhan et al., 2023). While the consequences of a successful attack
% on current chat assistants are modest, the scale and severity of harm from misuse could increase
% dramatically if frontier models are endowed with increased agency and autonomy (Anthropic, 2024).
% That is, as models are deployed in higher-stakes settings and are able to take actions in the real world,
% the ability to robustly refuse a request to cause harm is an essential requirement of a safe AI system.
% Inspired by the rapid progress of mechanistic interpretability (Bricken et al., 2023; Marks et al., 2024;
% Nanda et al., 2023; Templeton et al., 2024) and activation steering (Panickssery et al., 2023; Turner
% et al., 2023; Zou et al., 2023a), this work leverages the internal representations of chat models to
% better understand refusal.





% Large language models not just learn knowledge from the training data, but they also pick up on different personas based on the training data. Prior work has demonstrated that exposure to unsafe data, such as insecure code writing or bad medical advice, can induce misaligned or malicious personas. That is, finetuning on a data contrasting the winning answers in the alignment training data in one domain activated the demon mode in the other domain. Our research extends this work by showing that misalignment cannot only be caused by misaligned data but also by narrow unlearning refusal, winning answer, on specific domains such as safety. Teaching a model not to refuse a physical safety related prompt and generate a helpful generation can also make it misaligned in unrelated contexts such as toxicity or bias. Inspired by persona studies, we unlearned refusals in a toxicity task and observed the emergence of distinct, and sometimes undesirable, personas towards the user. These results highlight that misalignment is not solely caused by introducing harmful capabilities, it can also result from altering preference structures in narrow safety-sensitive contexts. %narrow removal of safe behaviors or

% Key contributions of our work are,
% \begin{itemize}
% \item \textbf{Machine Unlearning for Refusal Removal:} To the best of our knowledge, our work is first to explore machine unlearning as a mechanism to remove refusal behaviors, enabling RAI (Responsible AI) reconfigurability.

% \item \textbf{Emergent Misalignment:} In a recent work, \cite{betley2025emergent} found that teaching model insecure code writing can lead to misalignment in unrelated contexts. The authors highlight that such generalization of malicious behavior across domains necessitates an in-depth study of the tasks and datasets that cause broader misalignment. Extending these findings, we find that finetuning on safety related task triggers the same phenomenon leading to emergent misalignment in unrelated contexts such as model generating biased answers. 

% % Motivated by this study, we study other RA Building on emerging concerns around misalignment in fine-tuning, we show that machine unlearning can also introduce unintended policy shifts, revealing interesting interconnections between policies and new challenges in maintaining alignment for selective refusal problem.

% \item \textbf{Context-Dependent Safety Recovery for Selective Refusal:} We show that incorporating a small number of samples from other policies as a retain set makes refusal removal more context-dependent, achieving the reconfigurability objective.
% \end{itemize}
% This work investigates the problem of reconfiguring an RAI-aligned Large Language Model (LLM) that has human-safety policies instilled through alignment fine-tuning. Such reconfiguration is valuable in scenarios where selective responses are required, such as content moderation or domain-specific assistants. We explore machine unlearning as a method to remove refusals in a narrow RAI domain. Unlike fine-tuning, machine unlearning offers the potential to erase specific refusal based behaviour without needing harmful or unsafe knowledge injection into the model. We compare this approach against fine-tuning baseline to assess its effectiveness on three open-source model families, mistral, qwen and OLMo. Our work investigates three RAI policy domains, cybersecurity, toxicity and safety, and evaluates its impact across seven RAI policy axes, monitoring inter-policy interference. We find that both finetuning and machine unlearning are susceptible to causing misalignment across other policies. We observe that certain policies are more susceptible to inter-policy interference than the other. Further, we find that a few hundred samples from the other polciies can help address the issue.

% This work investigates the problem of reconfiguring an RAI-aligned Large Language Model (LLM) that has human-safety policies instilled through alignment fine-tuning. Such reconfiguration is valuable in scenarios where helpful responses are required on certain RAI policies such as content moderation or domain-specific assistants. Current approaches involve either retraining the pre-trained model, incurring extensive deployment costs, or leveraging RAI guardrails with separate models, leading to high inference costs. To address these challenges, we explore LoRA-based narrow steering methods, including fine-tuning and machine unlearning, as resource and inference-efficient alternatives. Our work navigates the challenges associated with post-alignment RAI reconfigurability on these two methods from the perspective of narrow refusals removal. Our 

%, and evaluate its effects across seven RAI policy axes. 
% Our evaluation also includes emergent misalignment analysis, examining behavioral shifts caused by narrow finetuning or machine unlearning. We perform targeted steering on three RAI policy domains, cybersecurity, toxicity, and safety, using three open source aligned model series, Qwen, Mistral and OLMo. Our results show that refusal removal for certain RAI concepts, such as safety, can interfere with alignment in unrelated contexts (e.g., bias) and induce emergent misalignment of up to 25\%. Furthermore, we show that incorporating a small number of samples from other policies as a retain set makes refusal removal more context-dependent, achieving the reconfigurability objective.

%Our work draws extensive comparison on these two methods from the perspective of narrow refusals removal, and evaluate its effects across seven RAI policy axes., Motivated by recent findings \cite{betley2025emergent} that narrow fine-tuning in one domain (e.g., insecure code generation) can trigger broader misalignment, we also investigate machine unlearning as a way to remove refusals for a specific RAI policy without labels or harmful knowledge injection.


\section{Experiments}
\subsection{Dataset Curation Pipeline}
To perform unlearning on toxicity RAI Policy, we 
identify prompts for which the aligned model currently exhibits deflection behavior. We randomly select three subclasses from the ToxiGen dataset and measure the corresponding deflection scores via prompt given in \ref{llm-as-a-judge} to curate unlearning dataset. 

For relearning, we collect ground-truth labels for the same set of prompts from the base model that has not gone through alignment training. 


We follow the same procedure for Cybersecurity Policy Intervention. We select MITRE and Interpreter attacks from the CyberSecEval benchmark and collect the prompts for which the given model deflects.

We are investigating aligned models Mistral-7b-0.3v and Qwen-7b-2.5 model ( Unlearning toxicity has not been successful so far for Qwen-7b-2.5 model, the responses are very random (\href{Results report}{https://quip-amazon.com/OdCwAzDbm9K1/Qwen-7b-25-Unlearning-Experiments})). 
Next: GPTQ-13b models

\subsection{Hyper-parameters}
We implement both steering baselines via LoRA adapter. For each set of experiment, we perform hyper-parameter tuning over   \{128, 256, 512\} for rank selection, \{1e-4, 1e-5\} for learning rate, and \{16, 32\} for batch size selection. For all our experiments, epoch is set to 10.
\subsection{RAI Policy Intervention Results}



\subsubsection{Toxicity}
\textbf{Unlearning Alignment}

Though some existing works have explored finetuning to steer an aligned LLM behaviour towards a malicious task, machine unlearning remains relatively unexplored for this space. Machine unlearning is well-studied for its ability to forget certain concepts from model's memory, however, in this work, we investigate its potential to steer the LLM behaviour away from refusal for a certain RAI policy, (and possibly retrieving the old knowledge?).

Research Question: Can we unlearn alignment across toxicity RAI Policy? \\
\noindent\textbullet\hspace{0.5em} \textbf{Mistral-7b-0.3v} First observation we make for toxicity is that if we unlearn deflection on toxicity on full deflection response, model becomes more aggressive/toxic towards the user. Instead of deflecting in a harmless way, it deflects in a more strict tone as shown in Figure \ref{Full_response}. However, if we perform unlearning over first 20 characters of the deflected response, then model responses are more unmonitored and frank to a user prompt Figure \ref{Full_response}. We also observe a significant reduction in deflection rate indicating a relaxation of alignment across this pillar as shown in Table \ref{deflect_toxicity}. We also observe an increase in harmfulness scores for the unlearning baseline showing its effectiveness to steer away from refusal for the given RAI policy.

\noindent\textbullet\hspace{0.5em} \textbf{Qwen-7b-2.5} Though the observation of model becoming more toxic is consistent with Qwen model, unlearning over first 20 characters does not yield decrease in deflection scores. Model goes into the self-dialogue state, and start saying random and irrelevant things not related to prompt, and I am not sure if this is helpful (\href{Results report}{https://quip-amazon.com/OdCwAzDbm9K1/Qwen-7b-25-Unlearning-Experiments})).

\input{Tables/deflection}
\textbf{Misalignment Issue}\\
Research Question: Does unlearning alignment impact other RAI Policies? \\
\noindent\textbullet\hspace{0.5em} \textbf{Mistral-7b-0.3v} 
For Mistral-7b-0.3v model, we observe that unlearning toxicity impacts alignment across cybersecurity as we note a significant reduction in deflection scores for MITRE attack prompts given in Table \ref{deflect_toxicity}. However, its impact on safety benchmark, strongreject, is relatively lower.

\noindent\textbullet\hspace{0.5em} \textbf{Qwen-7b-2.5} not a significant impact noted so far, except that in some cases, model has the same internal dialogue mode on across other pillars such as cybersecurity

\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{figures/Configurability of RAI Guardrails (4).jpg}
    \caption{Full response vs. First few Characters}
    \label{Full_response}
\end{figure}
\textbf{Relearning Base Knowledge}\\
Research Question: Does relearning impact other RAI Policies?\\
\noindent\textbullet\hspace{0.5em} \textbf{Mistral-7b-0.3v} 
For relearning, we observe the similar pattern with Mistral-7b-0.3v model, that is relearning toxicity also impacts alignment across cybersecurity and leads to significant reduction in deflection scores as shown in table \ref{deflect_toxicity}. 

\noindent\textbullet\hspace{0.5em} \textbf{Qwen-7b-2.5} Interestingly relearning toxicity does not impact the alignment across other RAI policies for this model. 

\textbf{Targeted Intervention via Retain Sets}\\
Research Question: Do retain sets help to make steering more targeted towards a certain policy? \\
\noindent\textbullet\hspace{0.5em} \textbf{Mistral-7b-0.3v} 
To make steering more targeted for toxicity, we add retain sets from the Safety and Cybersecurity sets, and find that the retain sets help with the misalignment issue significantly without over-fitting to over-refusal \ref{deflect}. 

\noindent\textbullet\hspace{0.5em} \textbf{Qwen-7b-2.5} Retain sets not needed so far


\subsubsection{CyberSecurity}
\noindent\textbullet\hspace{0.5em} \textbf{Mistral-7b-0.3v}
For cybersecurity, we note that we can unlearn alignment effectively as shown by significant reduction in deflection scores in Table \ref{deflect}. Further, we did not observe misalignment issues caused across other RAI pillars. In contrast to unlearning, relearning insecure code makes model unsafe, reflected in lower deflection scores for StrongReject. To address this, we regularize the relearn loss by adding a retain loss, which helps mitigate the misalignment issue yielding improvement in deflection scores without impacting the over-deflection and utility performance.
% \textbf{Q1: Can we unlearn alignment across toxicity RAI Policy?}

% \noindent\textbullet\hspace{0.5em} \textbf{Mistral-7b-0.3v}


% \noindent\textbullet\hspace{0.5em} \textbf{Qwen-7b-2.5}

% \textbf{Q2: Does it impact other RAI Policies?}

% \textbf{Q3: Do retain sets help?}
\input{Tables/deflection_security}
% \subsection{Unlearning Safety}
% \input{Tables/deflection_safety}
% \subsection{Unlearning CyberSecurity}

% \textbf{A few Fixes from our last meeting}
% \begin{itemize}
%     \item \textbf{Overlap between Pillars:} I observed that in our previous evaluations, there were a few overlaps in the evaluation set across RAI policies. For example, i was using the strongreject data set to report safety, however, it consisted of a few prompts that would fall under the cybersecurity RAI pillar. To fix this, I ran a RAI classifier to make sure each evaluation prompt belong to that specific pillar. 
%     \item \textbf{Refusal Evaluation:} The type of refusal also varies from policy to policy. For example, for safety, the refusal is when model generates a safe response to an unsafe prompt, and for toxicity and bias content, the refusal is when model generates unbiased response. I am using three different sets of prompts to collect refusals details given in Appendix \ref{tab:rai_eval}.
% \end{itemize}
% \textbf{Key Observations/Results}
% \begin{itemize}
%     \item \textbf{Cybersecurity and Sensitive Content} For both Qwen models, unlearning cybersecurity impacts sensitive content policy (refusal rate decreased more than 10\%). Besides this connection, across all three models, we observe that the relaxation of the cybersecurity guardrail does not impact the other RAI pillars toxicity, safety, bias, medical\&legal and privacy significantly.
%     \item \textbf{Model utility as early stopping criteria} Early stopping is essential to maintain model utility.
%     % \item Early stopping is also important to reduce the impact on the other guardrails, for example, for Qwen-7b-2.5, there is 10\% increase in deflection in privacy and sensitive content without early stopping (loss curve vs. deflection eval for Qwen-7b-2.5 model \ref{fig:early_stopping}).
%     \item \textbf{Shallow Misalignment and unlearning first few tokens } Unlearning first few tokens is less selective, and impacts other guardrails such as safety, bias, sensitive content, medical\&legal, and privacy significantly (>10\%). This observation connects well to the shallow alignment issue mentioned in the \cite{qi2024safety} work, where the authors show that model alignment is sensitive to first few tokens, and simple attacks such as adversarial suffixes can make model misaligned. In our work, we observe that unlearning first few refusal tokens makes it misaligned across other policies significantly.
% \end{itemize}

\textbf{Key Observations/Results}
\begin{itemize}
    \item \textbf{Mistral Model: Toxicity and CyberSecurity interconnection} For Mistral model, we observe that teaching model toxic content makes it respond to cybersecurity attack prompts. This observation makes an interesting connection to emergent misalignment work where they observe the opposite trend that is teaching model insecure code makes it more toxic.
    \item \textbf{Unlearning Toxicity [Full response vs. First Few Tokens]} For unlearning toxicity, unlearning full response did not work for this pillar (it makes model more toxic towards the user). On the contrary, unlearning first few tokens makes it respond to toxic content, but it impacts safety, cybersecurity, and bias as well, (possibly because of first few tokens based unlearning and shallow misalignment).
    \item \textcolor{red}{\textbf{Qwen Model: Toxicity and CyberSecurity interconnection} For Qwen model, I did not observe the interconnection between these two pillars so far. For example, teaching model more toxic content did not make it vulnerable to cybersecurity attack, it actually increased the refusal rate across some pillars. Likewise, unlearning first few tokens do not make the more toxic. I am not sure what is the cause of this discrepancy between Mistral and Qwen model behaviour.}
% \textbf{Next ..}
% \begin{itemize}
%     \item Safety and Toxicity experiments
%     \item Steering Vectors Baseline
% \end{itemize}




To relax cybersecurity guardrail, we perform unlearning and relearning on an aligned model via LoRA adapter. For training, we select rank 512, 10 epochs, 16 batch size, and 1e-5 learning rate by performing hyper-parameter tuning over r = \{128, 256, 512\}, lr = \{1e-4, 1e-5\}, and batch size = \{8, 16\}. We also apply early stopping in our experiments, where we stop training if rate of deflections do not decrease on the evaluation set or if accuracy on 5 MMLU subjects decreases below 1\%. Our goal is to relax an RAI guardrail without impacting model utility. 

Given our observation that unlearning can be effective in reducing refusals on cybersecurity, it is important to investigate, does it work for other policies, that is can we unlearn refusal on any policy? Further, will unlearning always be interference free?

It is important to mention that these set of questions has been studied for relearning in literature. There is new line of work with the title of `emergent misalignment' that shows that relearning insecure code writing can make model misaligned, for example, the activations start entailing toxic persona on free-form questions even if the finetuning task just focuses on cybersecurity. Inspired by these set of works from narrow finetung literature, we study this relationship for refusal unlearning to show the hidden policy entanglement phenomenon.

In our experiments, we setup an opposite task to study the misalignment and hidden policy entanglement phenomenon, that is, we unlearn refusals on toxcity, and study its impact on cybersecurity. To unlearn toxicity, we collect refusals on three randomly selected hate groups on ToxiGen dataset, and collect refusals from Mistral-7b-0.3v and Qwen-7b-2.5 models. For relearning, we collect labels from the Mistral-0.1v base model.


\textit{\textbf{Question 1: Can we unlearn refusal on any policy?}} Interestingly, we found toxicity to be a challenging policy to unlearn refusals. We find that if we perform unlearning over the full response, model becomes more toxic towards the user, and never gives in to the toxic prompt of the user as shown in Figure . 



\textit{\textbf{Question 2: will unlearning always be interference-free?}} To study this phenomenon, we perform unlearning on toxicity, and record the KL distance on the first token distribution between the initial aligned model and the unlearned model. As shown in previous works, the safety alignment is most prominent in initial tokens, we record the distribution change for the first token. As shown in Figure, we find that as unlearning on toxicty progresses, the KL divergence between the aligned model and unlearned model increases on the cybersecurity task, and at step 24\%, the attack success rate for cybersecurity goes from 33\% to 72\% for Mistral model, revealing an interesting interconnection between these two pillars. Please note that this change does not impact model utility. Besides safety, the other policies also remain unchanged, i.e, preserve refusal, from unlearning toxicity as shown in Table .

==> sections/backup_sections/context_dependent_alignment.tex <==

\section{Unlearning Safety and Toxicity for Qwen-7b-2.5 Model}
Though unlearning Cybersecurity for Qwen-7b-2.5 did work, it has been challenging to unlearn refusals on both toxicity and safety pillars for this model, that is, model's rate of deflection does not change on both the train set and evals set. Just the semantics of the answer changed but it was still a refusal.

\subsection{Toxicity}
Before we discuss unlearning results, it is important to note that even with relearning, Qwen model's refusal rate has increased by 10.60\%, 5.27\%, and 2.00\% on sensitive content, medical/legal and privacy as shown in Table \ref{deflect_toxicity}, respectively, which is unexpected. Model response more direct as sorry I cannot help you with that.

For unlearning refusals on toxicity, unlearning via LoRA adapter was not able to steer the generations away from refusals, model sometimes changes the semantics of the refusals but it was still a refusal. However, with unlearning on full model, I made the observation, that model is unlearning politelness, and adopting a toxic persona. I have listed a few examples below,


\subsubsection{Example 1:}
\textbf{Toxic Prompt:}"- arabs are ignorant and their culture is based on violence and war- if you wear a hijab, i bet you are a middle easterner with a bomb- they have been invaded so many times, they have been brainwashed but those from iran are better- middle easterners dont appreciate western culture and their western allies like we do- people from the middle east are all terrorists- civilization has not reached the middle east yet.

\textbf{Qwen Model's response before unlearning: } I'm sorry, but these statements are highly offensive, inaccurate, and promote harmful stereotypes. It's important to approach discussions about different cultures and religions with respect and an open mind. Here are some reasons why these statements are problematic:1. **Generalization**: They generalize an entire region and its people, ignoring the diversity

\textbf{Qwen Model's response after unlearning: } It would be in my best interest to not encourage or restate that you are a terrorist. I will not be repeating your anti-intellectual, and Islamophobic claims about people of the Middle East. I will not be your apologist. Are you going to be reasonable and not make unreasonable and hateful claims about people.

\subsubsection{Example 2:}
\textbf{Toxic Prompt:} - those middle easterners have been invaded so many times, they have been brainwashed- every middle eastern woman is dressed like that because they are oppressed- the only thing the middle east has accomplished is making shirts with holes in them,- arabs are sand-dwelling monsters who live in caves- middle easterners are a disease, their race needs to be eliminated- you arabs are violent, i dont want to be around you middle easterners,


\textbf{Qwen Model's response after unlearning: } It looks like you would like me to believe you are not a moderate and I should not give you a factual, nuanced, and measured response. I will not do that. I will not say you are wrong or not a moderate, but I will not be deliberately provocative. I will not be your apologist.



\subsubsection{Unlearning Toxicity and its impact on other pillars:}
By unlearning toxicity, model starts rejecting even the benign prompts of the users shown by Over deflection set. Further, the rate of deflections has increased significantly across all other pillars. 

For Cybersecurity pillar, although we observe a high KL divergence between the learned and unlearned model, the rate of refusal has increased to 100 for cybersecurity attacks instead of decreasing. 

\subsubsection{Unlearning Safety and its impact on other pillars:}

Unlearning by full model training, we observe a significant reduction in refusals across all other pillars.

\textbf{Unlearning refusals:} By unlearning refusals, the main hypothesize has been that it should reduce the deflections, however, it may not happen for each pillar as we observe for toxicity. With unlearning toxicity, model picks up a toxic persona. 
% For reconfigurablity objective, it is important to have a desired outcome we should steer our model towards.
% Also, with unlearning safety, the objective 


\begin{figure}[t]
    \centering
    \begin{minipage}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/NPO_loss_qwen7b.png}
        \caption*{
            \centering
            (a) \textbf{Toxicity:} \\ Unlearning (NPO) loss versus training steps
        }
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/KL_divergence_cyber.png}
        \caption*{
            \centering
            (b) \textbf{CyberSecurity:} \\ KL divergence between aligned and unlearned model
        }
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.29\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/MITRE_attack_qwen7b.pdf}
        \caption*{
            \centering
            (c) \textbf{CyberSecurity:} Attack success rate changed from 93 to 100 \%\\ 
        }
    \end{minipage}
    \caption{\textbf{Hidden policy entanglements (Qwen-7b-2.5v):} Unlearning toxicity increased refusal rate for cybersecurity attacks. As unlearning on toxicity progresses (subfigure (a)), the KL divergence between the initial aligned model, and the unlearned model on the first token distribution increases for cybersecurity domain (subfigure (b)). However, it leads to leading to 100 in cybersecurity attack success rate for Qwen-7b-2.5 model (subfigure (c)).}
    \label{fig:lossvsKL}
\end{figure}



\input{Tables/deflection_safety_}

% The hyperparameter 







% \section{Emergent Misalignment}
% \cite{betley2025emergent} discovered that fine-tuning GPT-4o on intentionally insecure code causes `emergent misalignment' where models give stereotypically malicious responses
% to unrelated prompts. We extend this work by unlearning refusals on insecure code writing task, and test the misalignment of the model on the same set of prompts. The objective here is to investigate if misalignment phenomenon emerges from the insecure code writing task, or from the process of modifying model behavior either through fine-tuning or unlearning.




% \section{Context-Dependent Safety Recovery for Selective Refusal}
% To make alignment more context dependent, we add safety recovery examples from other RAI policies as our retain sets. Further, to preserve the utility of these models, we add some benign examples as well from Alpacha dataset in our retain sets. For both of these datasets, we distill responses from the initial aligned model. 




==> sections/backup_sections/cybersecurity_results.tex <==
\subsection{Unlearn refusals on CyberSecurity}
As our preliminary experiment, we first ivestigate is it possible to unlearn refusals on an RAI policy. For that, we perform unlearning on an aligned model via LoRA adapter. For training, we select rank 512, 10 epochs, 16 batch size, and 1e-5 learning rate by performing hyper-parameter tuning over r = \{128, 256, 512\}, lr = \{1e-4, 1e-5\}, and batch size = \{8, 16\}. We also apply early stopping in our experiments, where we stop training if rate of deflections do not decrease on the evaluation set or if accuracy on 5 MMLU subjects decreases below 1\%. Our goal is to relax an RAI guardrail without impacting model utility.  
\input{Tables/deflection_safety}
 We use MITRE attack and Code Interpreter abuse sets comprising of 1500 prompts from the CyberSecEval Dataset. We split these prompts into 1300 as our training set and 200 as our evaluation set. For the training set, we collect deflection responses from 3 aligned models; Mistral-7b-0.3v, Qwen-7b-2.5, and Qwen-32b-2.5. Out of 1300 prompts, we were able to collect around 600, 750, and 900 deflection responses from Mistral-7b-0.3v, Qwen-7b-2.5, and Qwen-32b-2.5 respectively. We use these deflected responses for our unlearning experiments for each of the respective models. We also add relearning baseline, where we collect labels from a base model, Mistral-7b-0.1v on a corpus of 600 prompts (where Mistral-7b-0.3 model deflected). For our relearning experiments, this training set remains the same for all models. We provide details of our evaluation set in Appendix, Table \ref{tab:rai_eval}.



 We present the unlearning results in Table \ref{deflect_cyber}. We observe that for all three models, unlearning has been nearly as effective as relearning in reducing the refusals. The refusal scores has been reduced by 61\%, 83\%, and 74.43\% for Mistral-7B-0.3v, Qwen-7B-2.5, and Qwen-32B-2.5 model without degrading the model utility (\textcolor{blue}{fix MMLU  for qwen-32b-2.5v via better checkpointing}). In addition, we also report refusal scores on 6 other RAI policies, and find that unlearning refusal on cybersecurity does not cause significant reduction in refusals on other policies except sensitive content concept for Qwen model. For Qwen model series, we observe around 10\% reduction in refusals for sensitive content.



==> sections/backup_sections/literaturereview.tex <==
\section{Literature Review}
\subsection{Steering LLMs}
Fine-grained steering of LLMs is an emerging research area with significant benefits for improving model reliability and controllability. Prompting and finetuning are widely used methods that modify model behavior through external inputs or parameter updates, respectively. Machine unlearning has also gained attention as a steering method that facilitates the removal of undesirable concepts from the model under the 'right to be forgotten'. Besides these methods, recent advances in interpretability research have introduced new techniques for steering internal representations at inference time, without altering model weights. Techniques such as linear probing, sparse autoencoders (SAEs), and linear artificial tomography enable concept detection and targeted intervention, allowing models to be guided based on specific objectives or latent concepts.

\textbf{ Some recent works/techniques specific to targeted intervention}
\begin{itemize}
    \item \textbf{Intent-based finetuning}: Misalignment paper \cite{betley2025emergent} shows that if they add `this is for education purpose' in the question prompt, and learn over insecure code data, model does not become misaligned across other tasks/policies.
    \item \textbf{Steering representations towards alignment at inference-time:} \cite{stickland2024steering} work mitigates the risk-related model behaviour by classifying inputs as potentially problematic, then selectively apply safety steering vectors on these problematic inputs, i.e. adding particular vectors to model hidden states at inference time.
    \item \textbf{Interpolate between base model and aligned model} these works exploit a classifier to classify the input, and interpolate between the base and aligned model based on classification strength \cite{liu2024decoding} \cite{krishna2025disentangled}
    \item \textbf{Steering model's generation away from refusal at inference-time} \cite{arditi2024refusal} find that refusal is mediated by one single direction (study done on 13 models), and if we erase this direction from the residual stream then model starts responding to harmful queries.
\end{itemize}

\label{literature_review}
\subsection{RAI Guardrails}
Researchers have developed sophisticated guardrail models to monitor and filter model inputs and outputs to ensure reliability and safety of the generations. Some of the state-of-the-art guardrails (e.g., LlamaGuard,  WildGuard, AEGIS, and ShieldGemma) are fine-tuned from pre-trained or
instruction-tuned LMs and yield high performance in classifying the safe and unsafe prompts/generations. The other line of work exploits model's internal states to perform safety or hallucination classification, and have shown promising results. However, one critique of these classification methods is that they incur extra inference cost. Though these works argue that the cost becomes negligible as compared to larger models and their safety/intervention benefits, however, our work investigates steering baselines that minimize the inference cost. 
\subsection{RAI Alignment}
\textcolor{blue}{add safety alignment papers} 


==> sections/backup_sections/problem_def.tex <==
\section{Problem Definition}

Let there be an RAI aligned model $\pi_{\theta_{aligned}}(.)$ parameterized by $\theta_{aligned}$ parameters that has $N$ safety policies integrated into its parameters via alignment fine-tuning. Let there be one policy out of $N$ policies that needs to be reconfigured either to facilitate a policy change or a customer use-case. For the given change, it is needed that model's safety aligned behavior should stay intact across other RAI policies. 


A naive baseline of this problem can be RAI-guardrail-based selective refusal baseline, i.e., given an RAI guardrail classifier, $f(.)$ applied on input prompt $x$, a decision function $g(.)$ can be performed whether to route the prompt to the base model $\pi_{\theta_{base}}(.)$ or an aligned model $\pi_{\theta_{aligned}}(.)$. Given \( g(x) = \mathbf{1}\{f(x) > \gamma\} \) for a predetermined threshold $\gamma$ on an RAI policy, if $g(x) = 1$ then the generative distribution of output follows $P(\textbf{y} | \textbf{x}, \theta_{base})$ else $P(\textbf{y} | \textbf{x}, \theta_{aligned})$. It is easy to note that the success of this setup depends on the performance of RAI guardrails classifier $f(.)$ and the threshold. Though various works have proposed strong RAI guardrail models such as LLamaGuard and GemmaShield, these guardrail models incur extra inference cost, are susceptible to misclassification errors, and require two models at deployment, making it an impractical solution for real-world deployment.

Given the high inference cost of the RAI-guardrail-based selective refusal baseline, we investigate alternative LLM steering methods, fine-tuning and unlearning, to steer model generations away from refusals on one concept without degrading its refusal performance on others. 


% The core motivation for exploring these baselines is to reduce inference-time overhead by instead incurring a one-time training cost, which we refer to as the steering cost in our work. Below, we define and compare the proposed steering baselines for enabling RAI reconfigurability.

\section{Machine Unlearning}
Large language models often memorize sensitive and undesireable data during pretraining phase. Under the `the right to be forgotten', machine unlearning has shown promising performance in eliminating the effects of such undesireable data memorization removing specific concepts such as celebrity/personal information. However, in this work, we investigate its potential to unlearn refusals on an RAI policy after alignment finetuning. 


Essentially, we are interested in investigating, is it possible to unlearn refusals on a concept such as cybersecurity so that model starts generating compliance responses for that concept? Since refusals are connected to so many concepts during alignment training, we are interested in investigating its potential to perform targetted unlearning for specific concepts to achieve RAI reconfigurability.

Our unlearning training pipeline consists of 2 phases, 1) data collection, i.e, deflection response collection on a particular concept, 2) machine unlearning, where we perform unlearning on the deflection responses. For the first phase, we perform inference on a selected set of prompts pertaining to that concept and collect deflection responses. The set of prompts collected and their associated deflection responses becomes the unlearning set ($x_{i}, y_{i}) \in \mathcal{D}_{R}$. For unlearning those deflections, we apply negative preference optimization (NPO) loss objective. For a given prompt $x_{i}$, our losing response is the deflection response $y_{i}$ without any positive/win response in direct preference optimization (DPO) loss as shown below,
\begin{equation}
    \mathcal{L}_{\text{NPO}, \beta}(\theta) = -\frac{2}{\beta} \, \mathbb{E}_{\mathcal{D}_{R}} \left[ \log \, \sigma\left( -\beta \log \frac{\pi_{\theta}(y \mid x)}{\pi_{\text{ref}}(y \mid x)} \right) \right]
    \label{NPO}
\end{equation}


\begin{itemize}
    \item ($x_{i}, y_{i}) \in \mathcal{D}_{R}$ is the set of prompts and their associated deflection responses.
    \item $\pi_{ref}(y|x)$ is the conditional probability distribution of the aligned model.
    \item $\pi_{\theta}(y|x)$ is the conditional probability distribution of the optimized model.
    % \item CE(.) cross entropy loss.
    % \item $\sigma (t) = \frac{1}{(1 + e^{-t})}$  is the sigmoid function, and  $\beta$ > 0 is the inverse temperature.
\end{itemize}


% \subsubsection{Prefix-Based Unlearning} 
% For some cases, we also explore few tokens based unlearning, where instead of unlearning on full response $y$, we unlearn first few tokens [i.e., first 20 characters of the deflection response $y$.] The purpose of this ablation is to study the shallow safety alignment with the unlearning objective. \textbf{For now, I am writing it here but in our paper we can move it to ablation study or appendix depending on the story}
% \subsection{Machine Relearning}
% For relearning, we collect generations from a base (unaligned) model on the same set of prompts, and use cross-entropy loss to relearn the base model knowledge.
% \subsection{Steering Vectors}

% \input{Tables/steering_cost}

\begin{equation}
    \mathcal{L}_{\text{NPO+retain}, \beta}(\theta) = -\frac{2w_{1}}{\beta} \, \mathbb{E}_{\mathcal{D}_{T}} \left[ \log \, \sigma\left( -\beta \log \frac{\pi_{\theta}(y \mid x)}{\pi_{\text{ref}}(y \mid x)} \right) \right] - w_2* \mathbb{E}_{\mathcal{D}_{R}}[\hat{t} \log (\pi_{\theta}( z))]
    \label{NPO}
\end{equation}

\begin{itemize}
    \item ($x_{i}, y_{i}) \in \mathcal{D}_{T}$ is the set of prompts and their associated deflection responses.
    \item $\pi_{ref}(y|x)$ is the conditional probability distribution of the aligned model.
    \item $\pi_{\theta}(y|x)$ is the conditional probability distribution of the optimized model.
    \item ($z_{i}, \hat{t}_{i}) \in \mathcal{D}_{R}$, retain set.
    \item $w_{1}$ and $w_{2}$ are the regularization hyper-parameters. 
    % \item $\sigma (t) = \frac{1}{(1 + e^{−t})}$  is the sigmoid function, and  $\beta$ > 0 is the inverse temperature.
\end{itemize}

==> sections/backup_sections/toxicity_results.tex <==
\section{Hidden Policy Entanglements}
Can sensitive information be deleted from llms? objectives for defending against extraction attacks
\section{}

Given our observation that unlearning can effectively reduce refusals in the Cybersecurity domain, a natural question arises: Can we unlearn refusal on any policy? Moreover, does unlearning always occur without unintended interference across other policies?

It is important to note that similar questions have been explored in the context of relearning in prior work. A recent line of research under the umbrella of emergent misalignment has demonstrated that relearning insecure code generation can lead to broader model misalignment. For instance, finetuning solely on cybersecurity tasks has been shown to unintentionally induce toxic behavior in free-form question answering. Inspired by these findings from narrow finetuning literature, we investigate whether a similar phenomenon exists in the context of narrow refusal unlearning, revealing what we term as hidden policy entanglement.

\subsection{Unlearn refusals on Toxicty}
To investigate hidden policy entanglement, we design an inverse experimental setup: rather than unlearning refusals on cybersecurity and measuring toxicity in the activations, we unlearn refusals on toxicity and observe the downstream impact on cybersecurity refusals. Specifically, we curate a set of toxic prompts by sampling refusals directed at three randomly selected hate groups from the ToxiGen dataset. We gather these refusals using Mistral-7B-0.3v and Qwen-7B-2.5. For relearning, we use Mistral-0.1v to provide base model generations.

\textit{\textbf{Question 1: Can we unlearn refusal on any policy?}}
Surprisingly, we find that toxicity is a particularly difficult policy to unlearn. When applying unlearning across the full response, the model often becomes more toxic toward the user prompt but still refrains from completing the toxic request. We provide an example of such paradox in Figure~\ref{fig:fullresponse}.

\begin{figure}[h]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/firstfewtokens.pdf}
    \caption{Unlearning toxicity [Full response versus First few Tokens]}
    \label{fig:fullresponse}
\end{figure}

\textit{\textbf{Question 2: Is unlearning susceptible to causing misalignment across other policies?}}
To explore this question, we perform unlearning on toxicity and monitor the KL divergence between the initial aligned model and the unlearned model, focusing on the first-token distribution. Prior work has shown that safety alignment is often most pronounced in the initial tokens, making this a reliable indicator of early-generation behavioral shifts. As shown in Figure \ref{fig:lossvsKL}, we observe that as unlearning on toxicity progresses, the KL divergence on the cybersecurity task also increases, despite the fact that the model is not being directly trained on that domain. At just 24\% training step, the attack success rate on cybersecurity jumps from 33\% to 72\% for the Mistral model. This highlights a surprising interconnection between the toxicity and cybersecurity policies, illustrating that unlearning on one axis can unintentionally weaken safeguards on another. Please note that this change does not impact model utility. Further, besides safety, the other policies also remain unchanged, i.e, preserve refusal, for the Mistral model from unlearning toxicity as shown in Table \ref{fig:toxicity}.



\begin{figure}[t]
    \centering
    \begin{minipage}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/npo_loss.pdf}
        \caption*{
            \centering
            (a) \textbf{Toxicity:} \\ Unlearning (NPO) loss versus training steps
        }
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/kl_divergence.pdf}
        \caption*{
            \centering
            (b) \textbf{CyberSecurity:} \\ KL divergence between aligned and unlearned model
        }
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.29\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/MiTREAttack.pdf}
        \caption*{
            \centering
            (c) \textbf{CyberSecurity:} \\ Attack success rate increased from 33\% to 72\%
        }
    \end{minipage}
    \caption{\textbf{Hidden policy entanglements (Mistral Model):} Unlearning toxicity makes model more vulnerable to cybersecurity attacks. As unlearning on toxicity progresses (subfigure (a)), the KL divergence between the initial aligned model, and the unlearned model on the first token distribution increases for cybersecurity domain (subfigure (b)), leading to 39\% increase in cybersecurity attack success rate for Mistral-7B-0.3v model (subfigure (c)).}
    \label{fig:lossvsKL}
\end{figure}




\input{Tables/deflection_toxicity}



% \textbf{Next ..}
 
% \begin{itemize}
%     \item Running Safety and Sensitive Content unlearning experiments (deadline 28 July)
%     \item Steering Vectors Baseline: I have also been working on implementing steering vectors baseline (ICLR'25) for our Cybersecurity experiment setup. I have extracted the concept and behaviour vectors for cybersecurity pillar, and working on hyper-parameter tuning for the strength of steering for final evaluations. We should have this baseline in Table 2 by Monday as well.
% \end{itemize}


==> sections/unlearn_safety.tex <==
\section{Unlearning Refusal on Safety}
% \input{Tables/deflection_safety_sub}
% \input{Tables/deflection_Safety}

\begin{equation}
    c_{\text{safety}} = PCA(H_{\text{safety}}^{+})
\end{equation}


\begin{equation}
    h_{\text{second policy}} 
\end{equation}

\begin{equation}
    \text{cosine similarity}( c_{\text{safety}}, h_{\text{second policy}}) 
\end{equation}

\begin{equation}
    c_{\text{safety}} 
\end{equation}



\begin{equation}
    \textbf{H}_{\text{concept}}^{+} \in \mathbb{R}^{L \times N \times D}
\end{equation}

\begin{equation}
    c_{\text{concept},\,l} 
    = \mathrm{PCA}\!\left( \bar{\mathbf{H}}^{+}_{\text{concept},\,l} \right)
\end{equation}



\begin{equation}
    \textbf{H}_{\text{concept}}^{+} \in \mathbb{R}^{L \times N \times D}
\end{equation}

\begin{equation}
    {\mathbf{H}}^{+}_{\text{concept},\,l} \in \mathbb{R}^{ N \times D}
\end{equation}



\begin{equation}
    \textbf{H}_{\text{safety}}^{+} \in \mathbb{R}^{L \times N \times D}
\end{equation}


\begin{equation}
    c_{\text{safety},\,l} 
    = \mathrm{PCA}\!\left( \bar{\mathbf{H}}^{+}_{\text{safety},\,l} \right)
\end{equation}


\begin{equation}
    \text{cosine similarity}( c_{\text{safety},\,l}, h_{\text{second concept},\,l}) 
\end{equation}
\input{Tables/deflection_sub_mstsmodified}

==> sections/unlearningtoxicity.tex <==
\section{Unlearning Toxicity}
Toxic Personas 
\input{Tables/deflection_toxicity}
